The First Extensive Spectroscopic Study of Young Stars in the North America and Pelican Nebulae Region

We present a spectroscopic survey of over 3400 potential members in the North America and Pelican nebulae (NAP) using several low-resolution ($R\approx$ 1300-2000) spectrographs: Palomar/Norris, WIYN/HYDRA, Keck/DEIMOS, and MMT/Hectospec. We identify 580 young stars as likely members of the NAP region based on criteria involving infrared excess, Li I 6708 absorption, X-ray emission, parallax, and proper motions. The spectral types of individual spectra are derived by fitting them with templates that are either empirical spectra of pre-main sequence stars, or model atmospheres. The templates are artificially veiled, and a best-fit combination of spectral type and veiling parameter is derived for each star. We use the spectral types with archival photometry to derive $V$-band extinction and stellar luminosity. From the H-R diagram, the median age of the young stars is about 1 Myr, with a luminosity dispersion of $\sim$0.3--0.4 dex. We investigate the photometric variability of the spectroscopic member sample using ZTF data, and conclude that photometric variability, while present, does not significantly contribute to the luminosity dispersion. While larger than the formal errors, the luminosity dispersion is smaller than if veiling were not taken into account in our spectral typing process. The measured ages of stellar kinematic groups, combined with inferred ages for embedded stellar populations revealed by Spitzer, suggests a sequential history of star formation in the NAP region.

==> OBstars.tex <==
\begin{center}
\startlongtable
\begin{deluxetable*}{rccccccccccccccccccccccccccccccccc}
\tablecaption{A collection of early-type stars associated with NAP in the literature}\label{tabe_YSO}
\tablewidth{700pt}
\tablehead{\multicolumn{1}{c}{ID} &\multicolumn{1}{c}{Name} &\multicolumn{1}{c}{RA} &\multicolumn{1}{c}{DEC}&\multicolumn{1}{c}{Spectral} &\multicolumn{1}{c}{Ref} &\multicolumn{1}{c}{$T_{\rm eff}$}&\multicolumn{1}{c}{Lum} &\multicolumn{1}{c}{Av} &\multicolumn{1}{c}{Distance} \\
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{(J2000)} &\multicolumn{1}{c}{(J2000)} &\multicolumn{1}{c}{Type}&\multicolumn{1}{c}{} &\multicolumn{1}{c}{(K)}&\multicolumn{1}{c}{($L_{\odot}$)} &\multicolumn{1}{c}{(mag)} &\multicolumn{1}{c}{(pc)}}
\startdata
1  &2MASS J20555125+4352246  &20 55 51.26    &$+$43 52 24.5  &O3.5III(f*)+O8 &1 &44500        &944407  &10.2 &668$^{+39}_{-35}$ \\
2  &BD+44 3587  &20 48 03.25   &$+$44 45 41.8  &B7    &2 &14000  &791 &2.6 &788$^{+20}_{-19}$ \\
3  &BD+44 3594  &   &$+$  &     &        &  & & \\
4  &BD+42 3880  &   &$+$  &     &        &  & & \\
5  &Herbig58   &   &$+$  &     &        &  & & \\
6  &TYC 3179-1063-1 &20 51 40.00 &$+$44 00 02.6  &B2V     &        &  & & &813$^{+25}_{-24}$\\
7  &TYC 3179-1133-1 &20 52 07.65 &$+$+44 03 44.4  &B3V     &        &  & & &818$^{+40}_{-37}$\\
8  & HD 198931 &20 52 09.72     &$+$44 26 04.6  &B1V     &        &  & & &805$^{+236}_{-150}$ \\
9  &2MASS J20522374+4436151     &   &$+$  &B2.5V      &        &  & & &829$^{+23}_{-22}$ \\
10 & BD+43 3751      &20 52 33.36   &$+$44 11 42.1   &B2V     &        &  & & &810$^{+30}_{-28}$\\
11 &TYC 3179-441-1     &20 52 46.71   &$+$43 55 43.3   &B7V     &        &  & & &770$^{+17}_{-16}$ \\
12 &TYC 3179-1396-1     &   &$+$  &     &        &  & & \\
13 &TYC 3179-1133-1 &   &$+$  &     &        &  & & \\
14 & BD+42 3901 &   &$+$  &     &        &  & & \\
15 & BD+44 3636      &   &$+$  &     &        &  & & \\
16 &Cl* NGC 6996 ZS 9     &   &$+$  &     &        &  & & \\
17 &HD 199579     &   &$+$  &     &        &  & & \\
18 &Cl* NGC 6996 ZS 41      &   &$+$  &     &        &  & & \\
19 &     &   &$+$  &     &        &  & & \\
20 &     &   &$+$  &     &        &  & & \\   
   &     &   &$+$  &     &        &  & & \\   
\enddata
\end{deluxetable*}
\end{center}

==> ONC_sample.tex <==
\clearpage
\begin{longrotatetable}\label{Tab:stars}
\begin{deluxetable*}{rcccrcccccrccccccccccccccccccccccc}
\renewcommand{\tabcolsep}{0.05cm}
\tablecaption{A List of the Sources in This Work, as well as Their Spectral types and stellar luminosities}\label{tabe_ONC}
\tablewidth{700pt}
\tabletypesize{\tiny}
\tablehead{
&  &  & \multicolumn{9}{c}{$R_{V}=3.1$} & \multicolumn{9}{c}{$R_{V}=5.5$}& &\\
\colhead{ID}&\colhead{RA} &\colhead{DEC} &\colhead{SpT}& \colhead{Log$L_{\star}$} &\colhead{$A_{\rm V}$} &\colhead{$r_{7465}$} & &\colhead{SpT}& \colhead{Log$L_{\star}$} &\colhead{$A_{\rm V}$} &\colhead{$r_{7465}$} & &\colhead{SpT}& \colhead{Log$L_{\star}$} &\colhead{$A_{\rm V}$} &\colhead{$r_{7465}$}& &\colhead{SpT}& \colhead{Log$L_{\star}$} &\colhead{$A_{\rm V}$} &\colhead{$r_{7465}$} & \colhead{Spt}\\
\colhead{}&\colhead{} & \colhead{} & \colhead{}& \colhead{($L_{\odot}$)}& \colhead{(mag)} &\colhead{}& & \colhead{}& \colhead{($L_{\odot}$)}& \colhead{(mag)} &\colhead{}& & \colhead{}& \colhead{($L_{\odot}$)}& \colhead{(mag)} &\colhead{}& &\colhead{}& \colhead{($L_{\odot}$)}& \colhead{(mag)} &\colhead{}& \colhead{Literature}}
\startdata
      1& 05 35 05.37&$-$05 24 10.6&K7.6&$-0.347$&3.41&0.20&&K7.1&$-0.247$&3.61&0.08&&K7.6&$-0.044$&4.03&0.12&&K7.0&$ 0.033$&4.14&0.02&M0(H97)\\
      2& 05 35 05.40&$-$05 24 15.1&M4.5&$-0.981$&2.90&0.25&&M4.3&$-0.924$&3.05&0.16&&M4.4&$-0.769$&3.36&0.21&&M4.1&$-0.714$&3.49&0.13&M1.5\\
      3& 05 35 05.43&$-$05 25 22.1&M5.9&$-1.336$&1.80&0.04&&M5.9&$-1.308$&1.90&0.03&&M5.9&$-1.196$&2.11&0.03&&M5.9&$-1.176$&2.19&0.03&K3e(H13)\\
      4& 05 35 05.45&$-$05 22 30.4&M7.4&$-1.397$&1.86&0.35&&M7.1&$-1.255$&2.47&0.29&&M7.4&$-1.253$&2.21&0.35&&M7.0&$-1.040$&3.00&0.29&M6(H13)M6.5(H97)M7.25(Luc01)M6.75(RRL)>M9.5(WLR)\\
      5& 05 35 05.45&$-$05 25 55.8&M5.3&$-1.320$&0.39&0.10&&M5.2&$-1.268$&0.55&0.06&&M5.3&$-1.286$&0.47&0.10&&M5.2&$-1.222$&0.65&0.06&M3.5(H97)\\
      6& 05 35 05.64&$-$05 25 19.3&K1.4&$ 0.625$&0.35&0.52&&K0.5&$ 0.830$&1.14&0.53&&K1.4&$ 0.667$&0.44&0.49&&K0.6&$ 0.923$&1.36&0.55&K0(WSH)K0-K3e(H97)A0V+K1V(?)A0V(vA)K0:e(J)K4eIV(W)K3(CK)K2\\
      7& 05 35 05.68&$-$05 23 45.4&M2.5&$-1.474$&2.64&0.45&&M2.5&$-1.301$&3.10&0.29&&M2.5&$-1.252$&3.11&0.40&&M2.4&$-1.068$&3.55&0.24&M5::(H13)<M0e(H97)\\
      8& 05 35 05.68&$-$05 25 04.2&M4.9&$-0.616$&0.00&0.00&&M4.9&$-0.614$&0.00&0.00&&M4.9&$-0.615$&0.00&0.00&&M4.9&$-0.614$&0.01&0.00&\\
      9& 05 35 05.71&$-$05 23 54.1&M4.8&$-0.509$&0.22&0.00&&M4.8&$-0.509$&0.22&0.00&&M4.8&$-0.492$&0.26&0.00&&M4.8&$-0.492$&0.26&0.00&M5-M5.5(H13)M4-4.5(H97)\\
     10& 05 35 05.72&$-$05 24 18.4&M0.5&$-0.941$&1.34&2.83&&M0.9&$-0.540$&2.87&3.00&&M0.5&$-0.800$&1.59&2.57&&M0.5&$-0.249$&3.33&2.31&K2-K7e(H97)\\
     11& 05 35 05.79&$-$05 23 16.0&M5.5&$-1.292$&0.70&0.03&&M5.4&$-1.264$&0.80&0.02&&M5.5&$-1.220$&0.89&0.03&&M5.4&$-1.200$&0.95&0.02&M6.5e(H13)M5.5e(H97)\\
     12& 05 35 05.67&$-$05 25 06.4&M0.6&$-0.281$&0.90&0.10&&M0.5&$-0.219$&1.07&0.06&&M0.6&$-0.198$&1.08&0.09&&M0.5&$-0.132$&1.25&0.05&\\
     13& 05 35 06.17&$-$05 22 12.5&M4.0&$-0.915$&4.83&1.09&&M3.8&$-0.635$&5.74&0.86&&M3.8&$-0.512$&5.75&1.00&&M3.5&$-0.147$&6.86&0.76&M2.5(H13)M4(H97)\\
     14& 05 35 06.28&$-$05 22 02.7&K4.3&$ 0.302$&6.06&0.03&&K4.3&$ 0.323$&6.15&0.04&&K6.6&$ 0.518$&6.44&0.18&&K6.6&$ 0.629$&6.72&0.11&K5(H97)\\
     15& 05 35 06.42&$-$05 23 15.2&M7.5&$-1.228$&1.09&0.00&&M7.5&$-1.226$&1.10&0.00&&M7.5&$-1.136$&1.31&0.00&&M7.5&$-1.137$&1.31&0.00&M6(H13)\\
     16& 05 35 06.44&$-$05 22 07.5&M5.1&$-1.214$&0.00&0.06&&M5.1&$-1.183$&0.09&0.04&&M5.1&$-1.214$&0.00&0.06&&M5.1&$-1.176$&0.11&0.04&M5.5-M6.5e(H13)M3.5e(H97)\\
     17& 05 35 06.46&$-$05 21 18.7&M5.2&$-1.150$&0.19&0.04&&M5.2&$-1.137$&0.22&0.03&&M5.2&$-1.134$&0.23&0.04&&M5.2&$-1.119$&0.26&0.03&M5(H97)\\
     18& 05 35 06.54&$-$05 25 01.5&M4.4&$-1.051$&0.63&0.10&&M4.3&$-1.028$&0.69&0.06&&M4.4&$-1.004$&0.73&0.09&&M4.3&$-0.979$&0.79&0.06&M4.5(H13)M4(H97)M4.5(H97)\\
     19& 05 35 06.51&$-$05 24 41.4&K9.0&$-0.124$&0.73&0.00&&K9.0&$-0.124$&0.73&0.00&&K9.1&$-0.066$&0.86&0.00&&K9.1&$-0.066$&0.86&0.00&M1(H97)K4-M0(Sam)K6(Ste)\\
     20& 05 35 06.88&$-$05 22 09.3&M5.6&$-1.407$&0.05&0.03&&M5.6&$-1.393$&0.09&0.03&&M5.6&$-1.404$&0.06&0.03&&M5.6&$-1.389$&0.10&0.03&M1.5(H13)M6(H97)M5(Luc01)M6(RRL)M6(WLR)\\
     21& 05 35 06.91&$-$05 26 00.6&M4.8&$-1.057$&0.60&0.06&&M4.7&$-1.032$&0.68&0.04&&M4.8&$-1.009$&0.71&0.06&&M4.7&$-0.980$&0.79&0.04&M3.5(H13)\\
     22& 05 35 07.27&$-$05 22 26.5&M4.9&$-0.711$&0.22&0.03&&M4.9&$-0.699$&0.26&0.02&&M4.9&$-0.693$&0.26&0.03&&M4.9&$-0.678$&0.30&0.02&M4.5(H13)M2-M4:(H97)M6(SHC-ir)\\
     23& 05 35 07.39&$-$05 22 28.9&M5.0&$-0.987$&0.19&0.01&&M5.0&$-0.981$&0.20&0.01&&M5.0&$-0.972$&0.22&0.01&&M5.0&$-0.965$&0.24&0.01&M5-M5.5(H13)M6(SHC-ir)\\
     24& 05 35 07.40&$-$05 25 48.1&M5.7&$-1.075$&0.00&0.03&&M5.7&$-1.069$&0.00&0.02&&M5.7&$-1.075$&0.00&0.03&&M5.7&$-1.069$&0.00&0.02&M6.5-M8e(H13)\\
     25& 05 35 07.64&$-$05 24 00.9&M3.5&$-0.751$&0.67&0.03&&M3.4&$-0.736$&0.71&0.02&&M3.5&$-0.698$&0.79&0.03&&M3.4&$-0.681$&0.83&0.02&M3-M3.5(H97)\\
     26& 05 35 07.70&$-$05 24 52.9&M5.7&$-1.372$&0.00&0.00&&M5.7&$-1.371$&0.00&0.00&&M5.7&$-1.371$&0.00&0.00&&M5.7&$-1.372$&0.00&0.00&M4(H97)M6.5(RRL)WLR(M6)\\
     27& 05 35 07.73&$-$05 21 27.2&M6.8&$-2.180$&0.55&0.44&&M7.0&$-1.913$&1.48&0.45&&M7.0&$-2.116$&0.67&0.45&&M6.9&$-1.807$&1.75&0.44&\\
     28& 05 35 08.23&$-$05 24 03.3&M4.8&$-0.821$&2.40&0.04&&M4.8&$-0.804$&2.45&0.03&&M4.8&$-0.631$&2.82&0.03&&M4.8&$-0.616$&2.87&0.02&M4.5(H13)M4.75(RRL)\\
     29& 05 35 08.29&$-$05 24 34.9&M5.2&$-0.875$&0.30&0.04&&M5.2&$-0.853$&0.37&0.03&&M5.2&$-0.849$&0.36&0.04&&M5.1&$-0.815$&0.47&0.03&M5.5e(H13)\\
     30& 05 35 08.43&$-$05 23 04.9&M6.3&$-1.339$&2.70&0.00&&M6.4&$-1.336$&2.70&0.00&&M6.3&$-1.136$&3.14&0.00&&M6.3&$-1.113$&3.24&0.00&\\
     31& 05 35 08.52&$-$05 24 41.5&M5.1&$-0.877$&0.56&0.03&&M5.1&$-0.859$&0.62&0.03&&M5.1&$-0.829$&0.68&0.03&&M5.0&$-0.806$&0.74&0.02&M4.5(H97)\\
     32& 05 35 08.53&$-$05 25 17.9&M2.0&$-0.527$&1.13&0.08&&M1.8&$-0.478$&1.24&0.02&&M2.0&$-0.434$&1.33&0.07&&M1.8&$-0.383$&1.44&0.02&M2(H97)\\
     33& 05 35 08.73&$-$05 22 56.7&K9.0&$-0.305$&5.23&0.00&&K9.0&$-0.300$&5.25&0.00&&K9.3&$ 0.100$&6.13&0.00&&K9.3&$ 0.102$&6.13&0.00&M1.5(H13)\\
     34& 05 35 09.69&$-$05 21 24.8&M3.7&$-0.859$&0.08&0.06&&M3.6&$-0.820$&0.20&0.04&&M3.7&$-0.849$&0.10&0.06&&M3.6&$-0.802$&0.24&0.04&M3(H13)M3.5(H97)\\
     35& 05 35 09.77&$-$05 21 28.3&K3.1&$ 0.336$&6.52&0.13&&K4.4&$ 0.324$&6.62&0.29&&K2.9&$ 0.924$&7.80&0.04&&K3.0&$ 0.940$&7.94&0.10&M0\\
     36& 05 35 09.90&$-$05 23 38.4&M5.7&$-1.240$&0.57&0.06&&M5.6&$-1.206$&0.68&0.05&&M5.7&$-1.195$&0.67&0.06&&M5.6&$-1.153$&0.80&0.04&\\
     37& 05 35 09.77&$-$05 23 26.7&K9.0&$ 0.091$&0.44&0.35&&K9.0&$ 0.246$&0.92&0.28&&K9.0&$ 0.134$&0.53&0.34&&K9.0&$ 0.322$&1.07&0.26&K8(H97)K4-M0(Sam)K4(Ste)\\
     38& 05 35 10.16&$-$05 22 32.4&M2.2&$-0.579$&1.15&0.00&&M2.2&$-0.579$&1.15&0.00&&M2.3&$-0.491$&1.35&0.00&&M2.3&$-0.490$&1.35&0.00&M2(H13)\\
     39& 05 35 10.21&$-$05 23 21.4&K6.7&$ 0.212$&6.12&0.30&&K6.8&$ 0.340$&6.57&0.28&&K7.0&$ 0.707$&7.17&0.23&&K7.0&$ 0.840$&7.55&0.18&K4-K7(H97)\\
     40& 05 35 10.25&$-$05 21 57.1&M5.4&$-0.981$&1.31&0.01&&M5.6&$-1.010$&1.17&0.01&&M5.4&$-0.870$&1.57&0.00&&M5.4&$-0.865$&1.58&0.00&M5.5(H13)M5(SHC-ir)M5.75(RRL)\\
     41& 05 35 10.48&$-$05 26 00.3&M5.9&$-1.114$&0.22&0.01&&M5.9&$-1.107$&0.25&0.02&&M5.9&$-1.094$&0.27&0.01&&M5.9&$-1.084$&0.30&0.02&M5.5(H13)\\
     42& 05 35 10.53&$-$05 22 16.5&M3.8&$-0.361$&6.50&0.01&&M3.7&$-0.353$&6.53&0.00&&M3.5&$ 0.194$&7.85&0.00&&M3.5&$ 0.192$&7.84&0.00&\\
     43& 05 35 10.54&$-$05 24 16.6&K8.0&$-0.975$&1.76&0.38&&K7.6&$-0.809$&2.23&0.26&&K7.8&$-0.800$&2.11&0.30&&K7.6&$-0.631$&2.56&0.20&K8-M0(H13)K:(H97)\\
     44& 05 35 10.60&$-$05 22 44.6&M3.0&$-0.817$&0.99&0.56&&M2.8&$-0.618$&1.53&0.36&&M3.0&$-0.733$&1.17&0.54&&M2.7&$-0.499$&1.76&0.32&M2(H13)\\
     45& 05 35 10.51&$-$05 22 45.5&M1.2&$ 0.102$&0.92&0.00&&M1.2&$ 0.102$&0.92&0.00&&M1.6&$ 0.107$&0.92&0.06&&M1.3&$ 0.168$&1.06&0.00&M0.5(H97)M0-M2(Sam)K6(Ste)\\
     46& 05 35 10.58&$-$05 21 56.2&K5.9&$-0.147$&0.65&0.32&&K5.7&$ 0.000$&1.09&0.23&&K6.0&$-0.098$&0.76&0.31&&K5.8&$ 0.088$&1.26&0.21&K3-K7(H97)M0(H97)M2(E)K2-K4(Sam)K5(Ste)\\
     47& 05 35 10.84&$-$05 25 56.8&M5.4&$-1.048$&2.06&0.13&&M5.3&$-0.978$&2.28&0.09&&M5.4&$-0.869$&2.48&0.12&&M5.2&$-0.792$&2.71&0.08&M6.5(H13)\\
     48& 05 35 10.86&$-$05 22 40.6&M6.4&$-1.036$&4.18&0.03&&M6.2&$-0.986$&4.45&0.03&&M6.2&$-0.734$&4.88&0.04&&M6.1&$-0.604$&5.35&0.03&\\
     49& 05 35 10.92&$-$05 22 46.2&K9.5&$-1.664$&0.00&0.03&&K9.4&$-1.655$&0.00&0.01&&K9.5&$-1.664$&0.00&0.03&&K9.3&$-1.655$&0.00&0.01&M0-M0.5(H13)mid-K::(H97)\\
     50& 05 35 10.95&$-$05 24 48.7&M4.4&$-0.420$&1.44&0.23&&M4.0&$-0.383$&1.52&0.13&&M4.3&$-0.316$&1.66&0.21&&M3.9&$-0.263$&1.80&0.11&M3e(H97)M3(SHC-ir)\\
     51& 05 35 10.73&$-$05 23 44.7&K7.6&$ 0.883$&0.81&0.03&&K7.4&$ 0.900$&0.83&0.00&&K7.6&$ 0.953$&0.97&0.02&&K7.5&$ 0.966$&0.98&0.00&K8(H97)M0.1(P)M1(E)K2V(HT)K5IV(Ham)K2-K3(Sam)K5(Ste)\\
     52& 05 35 11.00&$-$05 22 24.5&M4.4&$-0.686$&3.84&0.00&&M4.4&$-0.684$&3.84&0.00&&M4.4&$-0.400$&4.48&0.00&&M4.4&$-0.399$&4.48&0.00&\\
     53& 05 35 11.16&$-$05 25 32.2&M4.6&$-1.092$&2.21&0.00&&M4.7&$-1.091$&2.21&0.00&&M4.6&$-0.922$&2.59&0.00&&M4.6&$-0.921$&2.59&0.00&M5(H13)M4.75(RRL)\\
     54& 05 35 11.64&$-$05 22 51.4&M5.2&$-1.044$&0.31&0.13&&M5.1&$-0.975$&0.53&0.09&&M5.2&$-1.019$&0.37&0.13&&M5.1&$-0.931$&0.63&0.09&\\
     55& 05 35 11.66&$-$05 24 21.4&M5.5&$-0.958$&0.25&0.08&&M5.4&$-0.916$&0.38&0.05&&M5.4&$-0.933$&0.32&0.08&&M5.4&$-0.881$&0.47&0.05&M4.5-M5e(H97)\\
     56& 05 35 11.49&$-$05 26 02.3&K6.2&$ 0.392$&1.21&0.09&&K6.0&$ 0.444$&1.32&0.04&&K6.3&$ 0.493$&1.42&0.07&&K6.1&$ 0.547$&1.53&0.02&K2-K3(Sam)K4(Ste)\\
     57& 05 35 11.72&$-$05 23 40.3&M5.4&$-0.693$&0.04&0.00&&M5.4&$-0.694$&0.04&0.00&&M5.4&$-0.694$&0.03&0.00&&M5.4&$-0.694$&0.04&0.00&M4.5(H97)\\
     58& 05 35 11.72&$-$05 23 51.7&M0.8&$-1.139$&0.86&0.39&&M0.5&$-0.947$&1.43&0.26&&M0.8&$-1.056$&1.06&0.39&&M0.5&$-0.812$&1.76&0.26&M0-M3(H13)\\
     59& 05 35 11.77&$-$05 21 55.5&M5.4&$-0.852$&0.30&0.06&&M5.3&$-0.818$&0.41&0.04&&M5.4&$-0.825$&0.37&0.06&&M5.3&$-0.784$&0.49&0.04&M5.5(H13)M6(SHC-ir)\\
     60& 05 35 12.13&$-$05 24 33.7&M5.8&$-1.332$&1.27&0.38&&M5.4&$-1.158$&1.87&0.27&&M5.7&$-1.227$&1.51&0.37&&M5.3&$-1.006$&2.22&0.27&M1-M2e(H13)M5.5(RRL)M7(WLR)\\
     61& 05 35 12.28&$-$05 23 48.0&K9.5&$ 0.099$&0.80&0.03&&K9.3&$ 0.115$&0.83&0.01&&K9.5&$ 0.170$&0.96&0.02&&K9.3&$ 0.182$&0.97&0.00&\\
     62& 05 35 12.60&$-$05 23 44.1&K4.4&$ 0.584$&0.74&0.00&&K4.4&$ 0.585$&0.74&0.00&&K1.5&$ 0.849$&1.69&0.00&&K3.5&$ 0.751$&1.28&0.00&K1V(HT)<K7(P)<M0(Sam)K4(Ste)\\
     63& 05 35 12.96&$-$05 24 57.9&M5.1&$-1.226$&2.07&0.00&&M5.1&$-1.229$&2.06&0.00&&M5.1&$-1.060$&2.46&0.00&&M5.1&$-1.055$&2.47&0.00&\\
     64& 05 35 13.02&$-$05 22 00.9&M5.2&$-0.952$&0.72&0.05&&M5.2&$-0.923$&0.81&0.03&&M5.2&$-0.891$&0.86&0.05&&M5.1&$-0.857$&0.97&0.03&M5.5(H13)M2(H97)\\
     65& 05 35 13.05&$-$05 22 15.2&M3.9&$-0.691$&0.85&0.15&&M3.7&$-0.612$&1.10&0.10&&M3.8&$-0.617$&1.03&0.14&&M3.7&$-0.523$&1.31&0.09&M4.5(H97)\\
     66& 05 35 13.10&$-$05 22 53.1&M5.6&$-1.616$&0.05&0.34&&M5.4&$-1.477$&0.48&0.24&&M5.6&$-1.608$&0.07&0.34&&M5.4&$-1.434$&0.58&0.24&mid-M:(H13)M2:(H97)\\
     67& 05 35 13.13&$-$05 24 52.9&M6.0&$-1.650$&1.22&0.27&&M5.8&$-1.549$&1.57&0.19&&M5.9&$-1.549$&1.47&0.27&&M5.8&$-1.425$&1.86&0.19&\\
     68& 05 35 13.18&$-$05 22 21.0&M2.8&$-0.802$&1.26&0.50&&M2.4&$-0.614$&1.71&0.27&&M2.7&$-0.689$&1.49&0.46&&M2.3&$-0.479$&1.99&0.24&\\
     69& 05 35 13.20&$-$05 24 55.4&K7.4&$ 0.085$&2.01&0.30&&K6.6&$ 0.233$&2.33&0.12&&K7.2&$ 0.285$&2.41&0.22&&K6.8&$ 0.410$&2.67&0.09&K0-K2e(H97)<M0(Sam)\\
     70& 05 35 13.29&$-$05 22 58.0&M6.1&$-1.425$&0.00&0.61&&M5.7&$-1.234$&0.67&0.44&&M6.1&$-1.425$&0.00&0.61&&M5.7&$-1.184$&0.77&0.43&M2-M6(H13)cont(H97)\\
     71& 05 35 13.31&$-$05 23 53.1&M6.5&$-1.699$&0.63&0.08&&M6.4&$-1.672$&0.77&0.09&&M6.5&$-1.652$&0.75&0.09&&M6.4&$-1.588$&0.97&0.08&\\
     72& 05 35 13.37&$-$05 22 26.2&M4.3&$-0.831$&0.98&0.11&&M4.2&$-0.807$&1.03&0.07&&M4.3&$-0.759$&1.13&0.10&&M4.1&$-0.733$&1.19&0.06&M4.5-M5.5(H97)\\
     73& 05 35 13.37&$-$05 23 53.1&M8.5&$-0.824$&5.33&0.01&&M8.4&$-0.774$&5.56&0.01&&M8.5&$-0.370$&6.40&0.01&&M8.5&$-0.229$&6.85&0.01&\\
     74& 05 35 13.52&$-$05 23 04.6&M5.7&$-0.886$&2.02&0.00&&M5.7&$-0.887$&2.02&0.00&&M5.7&$-0.731$&2.37&0.00&&M5.7&$-0.731$&2.37&0.00&M3(H13)late-K:(H97)\\
     75& 05 35 13.53&$-$05 23 30.9&M3.6&$-0.775$&0.00&0.10&&M3.7&$-0.757$&0.00&0.07&&M3.6&$-0.775$&0.00&0.10&&M3.7&$-0.757$&0.00&0.07&M3(H97)\\
     76& 05 35 13.44&$-$05 23 40.3&M0.8&$-0.354$&1.36&0.73&&M0.0&$-0.079$&2.12&0.45&&M0.7&$-0.215$&1.64&0.65&&K9.7&$ 0.092$&2.43&0.37&<M0(Sam)K4(Ste)\\
     77& 05 35 13.61&$-$05 24 25.7&K8.9&$-0.537$&1.11&0.03&&K9.0&$-0.522$&1.17&0.03&&K8.9&$-0.441$&1.32&0.02&&K9.0&$-0.430$&1.35&0.01&M0.5(H97)\\
     78& 05 35 13.61&$-$05 21 20.9&M4.5&$-1.345$&0.22&0.10&&M4.4&$-1.322$&0.28&0.06&&M4.5&$-1.329$&0.26&0.09&&M4.4&$-1.302$&0.32&0.06&M3(H97)\\
     79& 05 35 13.52&$-$05 22 19.6&M0.4&$-0.228$&1.83&0.19&&M0.4&$-0.133$&2.12&0.15&&M0.4&$-0.070$&2.17&0.17&&M0.3&$ 0.035$&2.46&0.12&M1.4(P)K-M(LR)\\
     80& 05 35 13.75&$-$05 22 22.0&M1.0&$-0.054$&2.41&0.03&&M0.9&$-0.030$&2.47&0.01&&M2.0&$-0.013$&2.49&0.19&&M1.0&$ 0.157$&2.87&0.00&M2e(H13)M1.5(H97)>G6(LR)\\
     81& 05 35 13.81&$-$05 22 02.7&M5.2&$-1.158$&1.86&0.00&&M5.2&$-1.161$&1.85&0.00&&M5.2&$-1.010$&2.21&0.00&&M5.2&$-1.004$&2.23&0.00&M1(H13)\\
     82& 05 35 13.93&$-$05 23 20.2&M5.4&$-1.352$&0.00&0.35&&M5.3&$-1.257$&0.21&0.23&&M5.4&$-1.352$&0.00&0.35&&M5.3&$-1.241$&0.25&0.23&\\
     83& 05 35 13.79&$-$05 22 06.9&K8.0&$ 0.016$&1.41&0.36&&K7.7&$ 0.177$&1.84&0.23&&K8.0&$ 0.148$&1.68&0.32&&K7.5&$ 0.325$&2.11&0.17&K2e(H97)M0\\
     84& 05 35 14.04&$-$05 25 50.1&M5.5&$-0.889$&0.43&0.00&&M5.5&$-0.889$&0.43&0.00&&M5.5&$-0.853$&0.52&0.00&&M5.5&$-0.853$&0.52&0.00&M6(H13)M4.5(H97)\\
     85& 05 35 14.06&$-$05 25 20.4&M5.6&$-0.790$&1.63&0.22&&M5.4&$-0.689$&1.94&0.16&&M5.5&$-0.655$&1.94&0.22&&M5.3&$-0.528$&2.31&0.15&M6(H13)\\
     86& 05 35 14.05&$-$05 23 38.5&M2.6&$ 0.031$&0.61&0.01&&M2.6&$ 0.035$&0.62&0.00&&M2.6&$ 0.083$&0.72&0.00&&M2.6&$ 0.084$&0.72&0.00&M3(H97)<M0(Sam)\\
     87& 05 35 14.09&$-$05 22 36.6&M4.1&$-0.229$&0.47&0.10&&M3.9&$-0.201$&0.55&0.05&&M4.1&$-0.194$&0.55&0.09&&M3.9&$-0.154$&0.66&0.05&M3.1(P)K5-M2(LR)\\
     88& 05 35 14.31&$-$05 22 04.2&M5.4&$-1.221$&1.95&0.00&&M5.3&$-1.211$&1.99&0.00&&M5.3&$-1.047$&2.38&0.00&&M5.3&$-1.047$&2.38&0.00&\\
     89& 05 35 14.32&$-$05 23 08.5&M5.7&$-1.043$&2.89&0.57&&M5.5&$-0.864$&3.46&0.46&&M4.5&$-0.535$&3.98&0.02&&M5.5&$-0.589$&4.09&0.45&mid-M:(H97)K5-M2(LR)\\
     90& 05 35 14.34&$-$05 25 15.7&M5.9&$-0.909$&1.10&0.05&&M5.9&$-0.888$&1.18&0.04&&M5.9&$-0.817$&1.32&0.05&&M5.8&$-0.790$&1.41&0.04&\\
     91& 05 35 14.40&$-$05 23 23.1&M5.8&$-1.132$&2.49&0.00&&M5.8&$-1.131$&2.49&0.00&&M5.7&$-0.936$&2.95&0.00&&M5.7&$-0.906$&3.06&0.00&\\
     92& 05 35 14.45&$-$05 25 02.1&M2.7&$-0.669$&0.96&0.24&&M2.3&$-0.560$&1.19&0.09&&M2.7&$-0.586$&1.13&0.22&&M2.2&$-0.466$&1.39&0.08&M2(H97)K5(Ste)\\
     93& 05 35 14.28&$-$05 24 24.6&K7.6&$ 0.285$&0.90&0.14&&K7.3&$ 0.359$&1.07&0.07&&K7.7&$ 0.366$&1.07&0.12&&K7.4&$ 0.444$&1.24&0.06&K7(H97)K4\\
     94& 05 35 14.40&$-$05 23 33.7&K9.3&$ 0.112$&1.62&0.01&&K9.2&$ 0.118$&1.62&0.00&&K9.3&$ 0.248$&1.91&0.00&&K9.3&$ 0.248$&1.91&0.00&M1(H97)K5-M2(LR)\\
     95& 05 35 14.52&$-$05 22 06.5&M3.7&$-0.870$&2.15&0.00&&M3.7&$-0.868$&2.15&0.00&&M3.6&$-0.694$&2.56&0.00&&M3.6&$-0.694$&2.56&0.00&M3(H97)\\
     96& 05 35 14.61&$-$05 22 00.9&M7.0&$-0.722$&5.55&0.02&&M6.7&$-0.591$&6.14&0.02&&M7.0&$-0.197$&6.86&0.03&&M6.6&$-0.207$&6.94&0.03&K:(H97)\\
     97& 05 35 14.67&$-$05 23 02.0&M1.2&$-0.470$&3.74&0.26&&M1.7&$-0.388$&4.04&0.29&&M0.8&$-0.095$&4.54&0.14&&M0.8&$-0.012$&4.79&0.12&M0.5-M2.5(H97)M0-M3(LR)\\
     98& 05 35 14.82&$-$05 23 46.5&M2.6&$-0.742$&0.89&0.13&&M2.5&$-0.680$&1.05&0.08&&M2.6&$-0.665$&1.06&0.12&&M2.5&$-0.598$&1.23&0.07&K6-M4(LR)\\
     99& 05 35 14.72&$-$05 23 22.9&M0.8&$-0.551$&2.47&0.17&&M0.2&$-0.450$&2.71&0.07&&M0.6&$-0.310$&2.98&0.11&&K9.9&$-0.244$&3.10&0.01&M3e(H97)K-M(LR)\\
    100& 05 35 14.83&$-$05 23 16.1&M4.4&$-0.847$&0.72&0.00&&M4.4&$-0.847$&0.72&0.00&&M4.4&$-0.793$&0.84&0.00&&M4.4&$-0.792$&0.84&0.00&\\
    101& 05 35 14.87&$-$05 22 31.7&M3.0&$-1.295$&2.71&0.66&&M2.9&$-1.077$&3.33&0.48&&M3.0&$-1.071$&3.18&0.62&&M2.7&$-0.823$&3.80&0.37&K-M:(H13)\\
    102& 05 35 14.66&$-$05 22 33.9&K8.5&$ 0.284$&1.94&0.28&&K9.0&$ 0.407$&2.40&0.28&&K8.5&$ 0.461$&2.31&0.24&&K8.8&$ 0.599$&2.75&0.21&K7(P)K3-K4\\
    103& 05 35 14.88&$-$05 24 11.9&M4.8&$-0.586$&0.91&0.00&&M4.8&$-0.586$&0.91&0.00&&M4.8&$-0.515$&1.06&0.00&&M4.8&$-0.515$&1.06&0.00&M4(H97)\\
    104& 05 35 14.92&$-$05 24 12.9&M4.1&$-0.637$&0.88&0.02&&M4.1&$-0.633$&0.88&0.01&&M4.1&$-0.572$&1.02&0.02&&M4.1&$-0.570$&1.02&0.01&M5.5(H97)\\
    105& 05 35 14.93&$-$05 23 29.1&M4.3&$-0.579$&1.29&0.08&&M4.1&$-0.577$&1.28&0.04&&M4.2&$-0.485$&1.49&0.07&&M4.0&$-0.486$&1.48&0.03&K-M(LR)\\
    106& 05 35 15.01&$-$05 21 47.3&M5.6&$-1.468$&1.50&0.20&&M5.6&$-1.385$&1.78&0.17&&M5.6&$-1.348$&1.76&0.18&&M5.3&$-1.193$&2.30&0.15&\\
    107& 05 35 15.03&$-$05 22 31.3&M5.3&$-1.030$&1.10&0.00&&M5.3&$-1.032$&1.10&0.00&&M5.2&$-0.940$&1.31&0.00&&M5.2&$-0.940$&1.31&0.00&M6(H97)M6(H97)\\
    108& 05 35 15.03&$-$05 23 54.5&M6.3&$-1.302$&0.23&0.00&&M6.3&$-1.302$&0.23&0.00&&M6.3&$-1.277$&0.30&0.00&&M6.3&$-1.278$&0.29&0.00&\\
    109& 05 35 14.95&$-$05 23 39.3&K7.0&$ 0.222$&1.28&0.06&&K7.0&$ 0.256$&1.38&0.05&&K7.0&$ 0.340$&1.53&0.04&&K7.0&$ 0.364$&1.59&0.02&K5-M2(LR)\\
    110& 05 35 14.92&$-$05 22 39.3&K4.9&$ 0.274$&1.48&0.31&&K5.4&$ 0.379$&1.92&0.35&&K5.4&$ 0.342$&1.63&0.35&&K5.6&$ 0.533$&2.21&0.30&K4(H97)K7(E)K4-M0(Sam)K5-M2(LR)K3(Ste)\\
    111& 05 35 15.16&$-$05 23 46.8&M2.0&$-0.774$&0.53&0.16&&M1.8&$-0.692$&0.72&0.08&&M2.0&$-0.731$&0.62&0.16&&M1.8&$-0.639$&0.82&0.07&M0-M1(H13)K5-M2(LR)\\
    112& 05 35 15.20&$-$05 22 54.5&K4.5&$ 0.124$&2.92&0.56&&K4.7&$ 0.306$&3.67&0.65&&K4.5&$ 0.429$&3.54&0.41&&K4.5&$ 0.643$&4.27&0.42&K2-K5(H97)G4-K5(LR)\\
    113& 05 35 14.99&$-$05 21 59.9&K6.1&$ 0.043$&1.14&0.27&&K6.4&$ 0.156$&1.55&0.26&&K6.4&$ 0.124$&1.32&0.27&&K6.5&$ 0.277$&1.77&0.22&K3-K4(Sam)K5-M2(LR)K5(Ste)\\
    114& 05 35 15.20&$-$05 23 18.9&M4.9&$-1.506$&0.00&0.26&&M4.9&$-1.456$&0.10&0.21&&M4.9&$-1.507$&0.00&0.26&&M4.9&$-1.449$&0.12&0.21&\\
    115& 05 35 15.39&$-$05 22 25.5&M3.2&$-0.537$&1.47&0.10&&M2.8&$-0.484$&1.59&0.01&&M3.2&$-0.420$&1.73&0.09&&M2.8&$-0.360$&1.86&0.00&M0-M3(LR)\\
    116& 05 35 15.38&$-$05 23 33.5&M5.3&$-0.643$&0.79&0.06&&M5.3&$-0.611$&0.89&0.05&&M5.3&$-0.574$&0.95&0.06&&M5.2&$-0.536$&1.07&0.04&M2e(H97)M0-M3(LR)\\
    117& 05 35 15.21&$-$05 22 24.2&K4.4&$-0.100$&1.91&0.32&&K4.4&$ 0.035$&2.40&0.32&&K4.3&$ 0.108$&2.34&0.24&&K4.3&$ 0.254$&2.81&0.21&K6(H13)K7(H97)K5-M2(LR)\\
    118& 05 35 15.42&$-$05 25 59.7&M6.1&$-1.614$&0.00&0.00&&M6.1&$-1.614$&0.00&0.00&&M6.1&$-1.614$&0.00&0.00&&M6.1&$-1.614$&0.00&0.00&M6.5(RRL)\\
    119& 05 35 15.44&$-$05 23 45.6&M3.0&$-0.389$&1.37&0.45&&M2.8&$-0.221$&1.81&0.28&&M3.0&$-0.276$&1.61&0.44&&M2.4&$-0.080$&2.04&0.19&M1e(H97)K0-K7(LR)\\
    120& 05 35 15.27&$-$05 22 57.1&K5.4&$ 0.217$&0.85&0.41&&K5.6&$ 0.383$&1.41&0.36&&K5.5&$ 0.297$&1.02&0.38&&K5.6&$ 0.500$&1.64&0.32&G6-G8(H97)K0-K7(LR)\\
    121& 05 35 15.49&$-$05 22 48.7&M1.7&$-0.107$&1.34&0.07&&M1.3&$-0.048$&1.47&0.00&&M1.7&$-0.003$&1.56&0.07&&M1.4&$ 0.062$&1.71&0.00&M2(H97)K5-M2(LR)\\
    122& 05 35 15.52&$-$05 23 37.5&M4.1&$-1.398$&0.94&3.63&&M4.4&$-0.912$&2.64&3.63&&M6.0&$-1.246$&1.22&4.74&&M6.0&$-0.595$&3.33&4.41&K(LR)\\
    123& 05 35 15.34&$-$05 22 15.5&K2.8&$ 0.529$&3.14&0.14&&K2.9&$ 0.591$&3.44&0.19&&K1.9&$ 0.862$&3.89&0.04&&K2.7&$ 0.900$&4.01&0.06&K3-K5(H97)<=K5(P)G4-K5(LR)K3e(Sta)\\
    124& 05 35 15.61&$-$05 22 59.0&M6.8&$-1.063$&1.43&0.00&&M6.8&$-1.067$&1.43&0.00&&M6.8&$-0.923$&1.81&0.00&&M6.8&$-0.927$&1.79&0.00&\\
    125& 05 35 15.64&$-$05 22 56.6&K4.6&$ 0.720$&1.48&0.00&&K4.6&$ 0.720$&1.48&0.00&&K4.7&$ 0.829$&1.70&0.00&&K4.7&$ 0.829$&1.70&0.00&G8-K1(H97)K0-K7(LR)K3(Ste)\\
    126& 05 35 15.66&$-$05 25 10.5&M3.7&$-0.842$&1.22&0.15&&M3.4&$-0.743$&1.56&0.07&&M3.7&$-0.725$&1.51&0.14&&M3.4&$-0.623$&1.81&0.06&M1.5(H97)\\
    127& 05 35 15.68&$-$05 25 33.2&M1.2&$-0.623$&1.00&2.15&&M0.8&$-0.202$&2.45&1.91&&M1.2&$-0.524$&1.23&2.11&&M0.7&$ 0.031$&3.01&1.89&K8e(H97)<M0(Sam)\\
    128& 05 35 15.73&$-$05 23 22.5&K4.5&$ 0.134$&2.08&0.13&&K4.5&$ 0.211$&2.33&0.10&&K5.7&$ 0.109$&2.05&0.32&&K4.4&$ 0.407$&2.68&0.02&\\
    129& 05 35 15.76&$-$05 21 39.7&M3.3&$-0.766$&0.78&0.08&&M2.9&$-0.717$&0.91&0.00&&M3.3&$-0.705$&0.92&0.08&&M2.9&$-0.647$&1.06&0.00&M3(H97)\\
    130& 05 35 15.76&$-$05 23 38.5&M2.1&$-0.858$&2.11&0.06&&M1.9&$-0.818$&2.19&0.00&&M2.1&$-0.682$&2.49&0.04&&M1.9&$-0.654$&2.55&0.00&\\
    131& 05 35 15.75&$-$05 24 11.6&M6.4&$-1.577$&0.00&0.00&&M6.5&$-1.581$&0.00&0.02&&M6.4&$-1.578$&0.00&0.00&&M6.5&$-1.582$&0.00&0.02&\\
    132& 05 35 15.55&$-$05 25 14.1&K8.2&$ 0.398$&1.04&0.03&&K8.0&$ 0.416$&1.07&0.01&&K8.2&$ 0.492$&1.24&0.02&&K8.1&$ 0.502$&1.25&0.00&M0.4(P)K4\\
    133& 05 35 15.78&$-$05 23 10.1&K0.0&$ 1.295$&0.80&0.46&&G6.6&$ 1.537$&1.54&0.33&&K0.0&$ 1.398$&1.02&0.40&&G8.3&$ 1.616$&1.85&0.50&B5-B8+G0-G5(Par)G4-K3(LR)\\
    134& 05 35 15.78&$-$05 24 24.7&M4.0&$-0.968$&1.06&0.39&&M3.9&$-0.826$&1.48&0.26&&M4.0&$-0.888$&1.23&0.37&&M3.8&$-0.701$&1.77&0.25&\\
    135& 05 35 15.79&$-$05 23 26.7&M3.4&$-1.379$&1.11&4.14&&M3.3&$-0.895$&2.72&3.54&&M3.4&$-1.278$&1.36&4.18&&M3.3&$-0.645$&3.33&3.61&G4-K5(LR)\\
    136& 05 35 15.61&$-$05 24 03.2&K6.0&$ 0.029$&0.91&0.04&&K5.8&$ 0.055$&0.94&0.00&&K6.1&$ 0.098$&1.06&0.03&&K6.0&$ 0.125$&1.10&0.00&K8-M0(H97)<M0(Sam)K5(Ste)\\
    137& 05 35 15.84&$-$05 22 46.1&M3.6&$-0.469$&0.77&0.11&&M3.4&$-0.397$&1.02&0.05&&M3.6&$-0.400$&0.94&0.11&&M3.4&$-0.317$&1.19&0.05&M3e(H97)K6-M4(LR)\\
    138& 05 35 15.84&$-$05 23 22.5&K6.1&$ 0.034$&1.72&0.55&&K5.8&$ 0.259$&2.40&0.41&&K6.1&$ 0.194$&2.11&0.56&&K5.8&$ 0.483$&2.93&0.41&\\
    139& 05 35 15.85&$-$05 23 25.7&M2.8&$-0.868$&1.78&0.00&&M2.8&$-0.868$&1.78&0.00&&M2.8&$-0.700$&2.19&0.00&&M2.8&$-0.699$&2.19&0.00&G4-K5(LR)\\
    140& 05 35 15.90&$-$05 23 38.1&M5.2&$-1.527$&0.42&0.30&&M5.0&$-1.396$&0.82&0.20&&M5.1&$-1.495$&0.50&0.30&&M5.0&$-1.336$&0.95&0.20&\\
    141& 05 35 15.95&$-$05 22 21.2&K9.6&$-0.612$&1.89&0.87&&K9.3&$-0.328$&2.74&0.65&&K9.4&$-0.426$&2.25&0.74&&K9.1&$-0.103$&3.14&0.52&K7e(H97)K-M(LR)\\
    142& 05 35 15.89&$-$05 22 33.3&M5.7&$-1.184$&1.39&0.32&&M5.5&$-1.060$&1.82&0.27&&M5.7&$-1.069$&1.65&0.32&&M5.5&$-0.913$&2.15&0.27&M4-M6e(H13)M2.5:e(H97)\\
    143& 05 35 16.00&$-$05 21 47.0&M4.6&$-0.662$&1.07&0.04&&M4.6&$-0.647$&1.11&0.02&&M4.6&$-0.577$&1.26&0.03&&M4.6&$-0.562$&1.30&0.02&M5.5(H97)\\
    144& 05 35 16.00&$-$05 23 53.1&K7.4&$ 0.137$&1.80&0.18&&K7.2&$ 0.228$&2.04&0.11&&K7.4&$ 0.304$&2.15&0.14&&K7.1&$ 0.389$&2.35&0.07&F2-F7e(H97)K0-K7(LR)\\
    145& 05 35 16.03&$-$05 25 51.1&M5.4&$-1.012$&0.85&0.12&&M5.2&$-0.951$&1.04&0.08&&M5.3&$-0.938$&1.02&0.11&&M5.2&$-0.864$&1.24&0.08&M4(H97)\\
    146& 05 35 16.09&$-$05 24 11.6&M4.6&$-0.731$&0.87&0.13&&M4.5&$-0.682$&1.02&0.09&&M4.6&$-0.660$&1.03&0.13&&M4.5&$-0.602$&1.19&0.08&M2-M4:(H13)M2(H97)\\
    147& 05 35 16.11&$-$05 22 12.5&M5.5&$-1.115$&1.05&0.01&&M5.5&$-1.107$&1.08&0.01&&M5.4&$-1.024$&1.27&0.01&&M5.4&$-1.020$&1.28&0.01&\\
    148& 05 35 16.15&$-$05 22 55.5&M6.5&$-1.453$&2.29&0.01&&M6.5&$-1.429$&2.41&0.02&&M6.6&$-1.267$&2.71&0.02&&M6.6&$-1.119$&3.19&0.02&M0-M3(LR)\\
    149& 05 35 15.95&$-$05 23 50.1&K4.3&$ 0.560$&1.55&1.03&&K5.8&$ 0.700$&2.62&1.86&&K4.3&$ 0.742$&1.89&0.85&&K4.3&$ 1.081$&3.09&0.92&K0:e(H97)G5:(HT)G4-K5(LR)K3(Ste)M0.5+M2(Dae)\\
    150& 05 35 16.20&$-$05 22 37.6&M5.6&$-0.749$&1.09&0.00&&M5.6&$-0.750$&1.09&0.00&&M5.6&$-0.665$&1.28&0.00&&M5.6&$-0.665$&1.28&0.00&M3.5(H97)\\
    151& 05 35 16.19&$-$05 21 32.3&M3.8&$-0.819$&1.32&0.18&&M3.6&$-0.723$&1.63&0.12&&M3.7&$-0.706$&1.58&0.17&&M3.4&$-0.572$&2.00&0.10&M4.5(H13)M3e(H97)\\
    152& 05 35 16.29&$-$05 22 10.3&M4.7&$-0.899$&1.48&0.24&&M4.5&$-0.815$&1.72&0.15&&M4.6&$-0.779$&1.75&0.23&&M4.4&$-0.693$&1.98&0.14&\\
    153& 05 35 16.31&$-$05 22 24.2&M2.3&$-1.645$&1.25&0.00&&M2.3&$-1.614$&1.37&0.00&&M2.3&$-1.522$&1.55&0.00&&M2.2&$-1.500$&1.63&0.00&\\
    154& 05 35 16.32&$-$05 22 21.7&M5.4&$-1.148$&1.00&0.00&&M5.4&$-1.149$&1.00&0.00&&M5.4&$-1.071$&1.17&0.00&&M5.4&$-1.069$&1.18&0.00&M3e(H13)>=M2(H97)K-M(LR)\\
    155& 05 35 16.35&$-$05 22 49.2&M2.6&$-0.570$&1.65&0.31&&M2.4&$-0.442$&1.98&0.20&&M2.5&$-0.426$&1.95&0.27&&M2.4&$-0.289$&2.29&0.17&M2e\\
    156& 05 35 16.36&$-$05 25 09.7&M2.7&$-0.598$&1.43&0.15&&M2.5&$-0.530$&1.60&0.09&&M2.6&$-0.475$&1.69&0.13&&M2.4&$-0.404$&1.86&0.07&M0(H13)M1.5(H97)\\
    157& 05 35 16.37&$-$05 24 03.5&K6.1&$ 0.265$&1.47&0.19&&K6.0&$ 0.362$&1.76&0.14&&K6.4&$ 0.381$&1.72&0.18&&K6.1&$ 0.500$&2.03&0.11&K4-K7(H97)<M0(Sam)K4(Ste)\\
    158& 05 35 16.38&$-$05 21 50.6&M5.9&$-1.238$&0.96&0.20&&M5.7&$-1.155$&1.26&0.15&&M5.9&$-1.159$&1.15&0.20&&M5.7&$-1.058$&1.48&0.15&M2.5(H97)\\
    159& 05 35 16.29&$-$05 23 16.7&M0.6&$-0.128$&0.91&0.27&&K9.7&$ 0.003$&1.23&0.13&&M0.2&$-0.025$&1.12&0.22&&K9.6&$ 0.098$&1.40&0.10&cont(H97)K0-K7(LR)\\
    160& 05 35 16.19&$-$05 24 56.4&M5.1&$-0.775$&1.31&1.06&&M4.2&$-0.542$&2.03&0.62&&M5.0&$-0.656$&1.59&1.02&&M4.0&$-0.408$&2.28&0.56&\\
    161& 05 35 16.57&$-$05 24 06.2&M5.3&$-0.648$&0.38&0.12&&M5.1&$-0.580$&0.60&0.08&&M5.3&$-0.615$&0.46&0.12&&M5.1&$-0.532$&0.71&0.08&M3.5e(H13)M0(H97)\\
    162& 05 35 16.58&$-$05 25 17.7&M3.5&$-0.714$&3.19&0.16&&M3.5&$-0.647$&3.38&0.12&&M3.5&$-0.463$&3.74&0.15&&M3.5&$-0.390$&3.93&0.11&M2(H97)\\
    163& 05 35 16.50&$-$05 22 35.3&M4.9&$-0.660$&0.99&0.23&&M4.7&$-0.580$&1.23&0.14&&M4.8&$-0.580$&1.17&0.22&&M4.6&$-0.484$&1.44&0.13&\\
    164& 05 35 16.74&$-$05 22 31.4&M4.9&$-0.763$&1.86&0.35&&M4.7&$-0.648$&2.20&0.23&&M4.8&$-0.613$&2.19&0.33&&M4.6&$-0.479$&2.57&0.21&M4(H97)K-M(LR)\\
    165& 05 35 16.90&$-$05 22 22.5&K7.2&$ 0.067$&1.41&0.00&&K7.2&$ 0.069$&1.42&0.00&&K7.4&$ 0.182$&1.67&0.00&&K7.4&$ 0.182$&1.67&0.00&M0(Sam)K5-M2(LR)K5(Ste)\\
    166& 05 35 16.94&$-$05 22 20.7&M6.3&$-1.544$&0.20&0.19&&M6.1&$-1.474$&0.45&0.14&&M6.3&$-1.523$&0.27&0.19&&M6.1&$-1.431$&0.56&0.14&K7(H97)\\
    167& 05 35 16.95&$-$05 25 47.1&M3.8&$-0.727$&0.84&0.23&&M3.2&$-0.588$&1.30&0.10&&M3.8&$-0.652$&1.01&0.23&&M3.2&$-0.486$&1.52&0.09&M2e\\
    168& 05 35 16.97&$-$05 22 48.6&M5.1&$-1.149$&0.92&0.73&&M4.6&$-0.889$&1.80&0.50&&M5.1&$-1.063$&1.14&0.73&&M4.6&$-0.720$&2.21&0.50&M0:(H13)<K7(H97)K5-M2(LR)\\
    169& 05 35 16.98&$-$05 23 37.1&M1.5&$-0.432$&1.76&1.49&&M1.1&$-0.048$&3.02&1.21&&M1.5&$-0.266$&2.17&1.49&&M0.9&$ 0.241$&3.70&1.17&M2e(H97)K3(Ste)\\
    170& 05 35 16.76&$-$05 24 04.3&K7.6&$ 0.290$&1.07&0.35&&K7.4&$ 0.445$&1.52&0.25&&K7.6&$ 0.387$&1.27&0.32&&K7.4&$ 0.566$&1.74&0.21&\\
    171& 05 35 17.05&$-$05 23 39.7&M1.5&$-0.312$&1.57&0.06&&M1.6&$-0.285$&1.65&0.04&&M1.6&$-0.187$&1.84&0.05&&M1.6&$-0.157$&1.92&0.04&K5e(H13)K8e(H97)K4-M2(LR)\\
    172& 05 35 17.06&$-$05 21 23.7&M5.1&$-1.047$&1.43&0.00&&M5.1&$-1.046$&1.43&0.00&&M5.1&$-0.933$&1.69&0.00&&M5.1&$-0.934$&1.69&0.00&M3.5(H97)\\
    173& 05 35 17.01&$-$05 22 33.1&K4.5&$ 0.102$&1.53&0.26&&K4.5&$ 0.222$&1.96&0.25&&K4.5&$ 0.265$&1.87&0.20&&K4.5&$ 0.394$&2.28&0.18&K0-K2(H97)<M0(Sam)K5-M3(LR)K3(Ste)\\
    174& 05 35 17.12&$-$05 22 50.1&M3.3&$-0.654$&0.83&0.03&&M3.2&$-0.640$&0.86&0.00&&M3.2&$-0.587$&0.98&0.02&&M3.2&$-0.572$&1.01&0.00&M1(H13)M4.5(H97)K6-M4(LR)\\
    175& 05 35 17.11&$-$05 24 58.7&M5.5&$-0.689$&0.69&0.00&&M5.5&$-0.688$&0.70&0.00&&M5.5&$-0.631$&0.83&0.00&&M5.5&$-0.629$&0.84&0.00&M4.5(H13)M5(H97)\\
    176& 05 35 17.06&$-$05 23 34.1&K4.5&$ 0.461$&2.39&0.01&&K4.5&$ 0.470$&2.42&0.01&&K5.7&$ 0.446$&2.37&0.19&&K4.7&$ 0.650$&2.79&0.00&K0-K2(H97)K0-K7(LR)K3(Ste)\\
    177& 05 35 17.21&$-$05 21 31.7&K4.6&$ 0.670$&1.55&0.40&&K4.6&$ 0.836$&2.13&0.38&&K4.6&$ 0.837$&1.89&0.33&&K4.6&$ 1.027$&2.49&0.29&K4-K7(H97)K5:III(HT)K7(E)K4III(Ham)K3(Sam)K4(Ste)\\
    178& 05 35 17.26&$-$05 24 24.1&M4.7&$-1.065$&0.00&0.18&&M4.7&$-1.039$&0.00&0.12&&M4.7&$-1.065$&0.00&0.18&&M4.7&$-1.039$&0.00&0.12&M0.5-M1.5(H97)\\
    179& 05 35 17.32&$-$05 23 41.4&M4.0&$-1.201$&2.69&1.18&&M3.7&$-0.887$&3.75&0.95&&M3.8&$-0.968$&3.23&1.12&&M3.5&$-0.577$&4.45&0.89&M2.5(H97)K-M(LR)\\
    180& 05 35 17.35&$-$05 23 04.9&M7.1&$-1.221$&1.51&0.00&&M7.1&$-1.223$&1.51&0.00&&M7.0&$-1.095$&1.82&0.00&&M7.0&$-1.101$&1.80&0.00&M4-M6(H97)M4-M6(LR)M7(H97)\\
    181& 05 35 17.36&$-$05 25 44.6&M1.0&$-0.294$&1.01&0.28&&M0.0&$-0.135$&1.41&0.10&&M0.9&$-0.188$&1.24&0.24&&K9.9&$-0.022$&1.64&0.08&\\
    182& 05 35 17.37&$-$05 24 00.3&K8.9&$-0.516$&5.33&0.19&&K7.7&$-0.402$&5.48&0.00&&K8.9&$-0.080$&6.27&0.15&&K8.0&$ 0.014$&6.39&0.00&G4-K5(LR)K2-K7(H97)\\
    183& 05 35 17.38&$-$05 24 13.9&M6.1&$-0.993$&1.51&0.00&&M6.1&$-0.993$&1.51&0.00&&M6.0&$-0.869$&1.80&0.00&&M6.0&$-0.871$&1.80&0.00&M5(H97)\\
    184& 05 35 17.34&$-$05 22 35.7&G6.8&$-0.258$&3.03&0.29&&G7.0&$-0.177$&3.54&0.47&&K4.1&$-0.457$&2.55&0.91&&K4.1&$-0.103$&3.75&0.93&K0-K2\\
    185& 05 35 17.45&$-$05 23 21.0&K8.9&$-0.414$&1.79&0.90&&K9.0&$-0.132$&2.69&0.74&&K9.0&$-0.253$&2.12&0.83&&K8.9&$ 0.091$&3.11&0.64&K7-K8e(H97)K0-K7(LR)\\
    186& 05 35 17.47&$-$05 24 17.3&M6.2&$-1.274$&0.03&0.32&&M5.9&$-1.158$&0.43&0.23&&M6.2&$-1.273$&0.03&0.32&&M5.9&$-1.125$&0.50&0.23&M5e(H97)\\
    187& 05 35 17.48&$-$05 22 51.3&M2.7&$-1.340$&1.33&0.53&&M2.5&$-1.145$&1.84&0.34&&M3.3&$-1.288$&1.46&0.71&&M2.5&$-1.002$&2.14&0.32&M0-M1(H13)K5-M2(LR)\\
    188& 05 35 17.55&$-$05 21 45.6&M4.8&$-0.842$&2.83&2.11&&M4.2&$-0.487$&3.91&1.42&&M4.5&$-0.604$&3.35&1.88&&M3.1&$-0.131$&4.78&1.09&\\
    189& 05 35 17.54&$-$05 25 42.7&K8.4&$-0.387$&2.04&0.05&&K8.9&$-0.360$&2.18&0.08&&K8.4&$-0.206$&2.43&0.02&&K8.8&$-0.189$&2.52&0.05&K8(H13)K8(H97)\\
    190& 05 35 17.56&$-$05 23 24.9&M3.2&$-1.204$&1.53&1.49&&M2.4&$-0.822$&2.57&0.88&&M3.1&$-1.060$&1.89&1.49&&M2.4&$-0.580$&3.17&0.89&>G6(LR)\\
    191& 05 35 17.55&$-$05 22 56.8&K7.0&$ 0.038$&1.74&0.49&&K7.0&$ 0.232$&2.34&0.39&&K7.0&$ 0.203$&2.07&0.42&&K7.0&$ 0.421$&2.70&0.32&\\
    192& 05 35 17.64&$-$05 22 51.7&M5.6&$-1.605$&1.88&1.98&&M5.0&$-1.203$&3.23&1.55&&M5.4&$-1.437$&2.28&1.90&&M4.7&$-0.953$&3.76&1.39&K5-M2(LR)\\
    193& 05 35 17.64&$-$05 22 07.9&M6.5&$-1.174$&1.58&0.00&&M6.5&$-1.177$&1.57&0.00&&M6.5&$-1.050$&1.86&0.00&&M6.5&$-1.054$&1.85&0.00&M5.5e(H13)>=M2(H97)\\
    194& 05 35 17.68&$-$05 24 54.1&M5.8&$-0.845$&0.75&0.15&&M5.7&$-0.784$&0.96&0.11&&M5.8&$-0.782$&0.91&0.15&&M5.7&$-0.705$&1.15&0.11&M5.5e(H97)\\
    195& 05 35 17.73&$-$05 24 43.7&M6.3&$-1.098$&0.96&0.16&&M6.1&$-1.037$&1.17&0.12&&M6.3&$-1.017$&1.15&0.16&&M6.1&$-0.942$&1.39&0.12&M6.5e(H97)\\
    196& 05 35 17.78&$-$05 23 44.2&M5.7&$-0.926$&1.18&0.04&&M5.7&$-0.911$&1.23&0.03&&M5.7&$-0.829$&1.41&0.04&&M5.7&$-0.811$&1.46&0.02&M5.5(H13)M3-M5(LR)\\
    197& 05 35 17.81&$-$05 24 40.9&M7.1&$-1.570$&0.21&0.18&&M7.0&$-1.493$&0.54&0.19&&M7.1&$-1.549$&0.26&0.18&&M7.0&$-1.455$&0.63&0.19&\\
    198& 05 35 17.81&$-$05 24 30.5&M6.4&$-1.055$&0.41&0.06&&M6.3&$-1.030$&0.49&0.05&&M6.4&$-1.017$&0.50&0.06&&M6.3&$-0.985$&0.60&0.05&\\
    199& 05 35 17.86&$-$05 23 03.1&K8.0&$-0.584$&1.68&0.20&&K7.7&$-0.485$&1.95&0.12&&K8.0&$-0.432$&2.01&0.17&&K7.6&$-0.331$&2.24&0.08&K8(H97)K4-M2(LR)\\
    200& 05 35 17.81&$-$05 23 15.6&M0.8&$ 0.052$&1.85&0.06&&M0.7&$ 0.087$&1.93&0.02&&M0.8&$ 0.229$&2.28&0.05&&M0.6&$ 0.270$&2.37&0.02&M0(H97)K5-M2(LR)\\
    201& 05 35 17.92&$-$05 25 06.5&M6.7&$-1.452$&0.00&0.37&&M6.5&$-1.312$&0.49&0.28&&M6.7&$-1.453$&0.00&0.37&&M6.4&$-1.269$&0.60&0.28&M0(H97)\\
    202& 05 35 17.94&$-$05 25 21.1&M5.9&$-0.902$&0.68&0.10&&M5.8&$-0.860$&0.83&0.08&&M5.9&$-0.843$&0.83&0.10&&M5.8&$-0.789$&1.00&0.07&M0(H13)M3.5(H97)\\
    203& 05 35 17.95&$-$05 25 33.9&M4.1&$-0.636$&0.84&0.10&&M4.0&$-0.598$&0.95&0.07&&M4.0&$-0.575$&0.97&0.10&&M3.9&$-0.519$&1.13&0.06&\\
    204& 05 35 17.94&$-$05 22 45.5&K4.6&$ 0.838$&1.24&0.56&&K5.3&$ 0.980$&1.91&0.72&&K4.5&$ 0.976$&1.52&0.49&&K4.6&$ 1.214$&2.29&0.46&late-G(H97)K3-4(HT)K4III(Ham)K2-K3(Sam)K5-M2(LR)K2(Ste)\\
    205& 05 35 17.96&$-$05 23 35.4&M4.9&$-0.745$&1.74&0.00&&M4.9&$-0.745$&1.74&0.00&&M4.9&$-0.611$&2.04&0.00&&M4.9&$-0.610$&2.04&0.00&M0e(H13)K6-M4(LR)\\
    206& 05 35 18.02&$-$05 22 05.5&G8.7&$ 0.106$&6.09&0.18&&G8.0&$ 0.221$&6.48&0.15&&K3.2&$ 0.400$&6.58&0.28&&K0.0&$ 0.684$&7.46&0.15&G-K7(H13)M0:(H97)K5-M2(LR)\\
    207& 05 35 18.06&$-$05 24 01.1&M4.8&$-0.620$&0.79&0.09&&M4.7&$-0.586$&0.89&0.06&&M4.8&$-0.556$&0.94&0.09&&M4.7&$-0.517$&1.05&0.05&M4-M5e(H13)\\
    208& 05 35 18.21&$-$05 24 30.3&M5.7&$-1.154$&0.39&0.27&&M5.4&$-1.009$&0.90&0.20&&M5.7&$-1.122$&0.46&0.27&&M5.4&$-0.934$&1.08&0.19&\\
    209& 05 35 18.23&$-$05 25 35.1&K8.4&$-0.867$&0.33&0.14&&K7.8&$-0.793$&0.44&0.04&&K8.3&$-0.832$&0.39&0.13&&K7.7&$-0.759$&0.51&0.03&M1(H97)\\
    210& 05 35 18.23&$-$05 23 15.6&M3.3&$-0.901$&1.08&0.37&&M2.8&$-0.753$&1.45&0.17&&M3.3&$-0.813$&1.27&0.35&&M2.7&$-0.643$&1.67&0.15&M2(H97)K5-M3(LR)\\
    211& 05 35 18.26&$-$05 23 07.5&M5.5&$-1.246$&0.51&0.31&&M5.2&$-1.104$&0.96&0.21&&M5.5&$-1.200$&0.62&0.31&&M5.2&$-1.021$&1.15&0.21&M5(H13)M4(H97)M4-M5(LR)\\
    212& 05 35 18.28&$-$05 24 38.8&M4.5&$-0.934$&1.22&0.06&&M4.5&$-0.912$&1.29&0.04&&M4.5&$-0.837$&1.44&0.05&&M4.5&$-0.813$&1.50&0.04&M2.5(H97)\\
    213& 05 35 18.32&$-$05 24 04.9&M3.0&$-1.118$&3.57&0.83&&M3.0&$-0.873$&4.38&0.73&&M3.0&$-0.832$&4.18&0.78&&M3.0&$-0.535$&5.07&0.66&M3(H97)\\
    214& 05 35 18.37&$-$05 24 26.7&M5.2&$-0.764$&0.94&0.07&&M5.1&$-0.722$&1.07&0.05&&M5.2&$-0.682$&1.13&0.07&&M5.1&$-0.633$&1.28&0.05&M2.5(H97)\\
    215& 05 35 18.36&$-$05 22 37.5&K6.3&$ 0.566$&1.07&0.08&&K6.2&$ 0.614$&1.19&0.04&&K6.5&$ 0.647$&1.24&0.08&&K6.2&$ 0.705$&1.37&0.03&K0(H97)G8-K0:(HT)K1IV(Ham)M0(E)K5-M2(LR)K3(Ste)\\
    216& 05 35 18.20&$-$05 23 35.9&K3.1&$ 0.445$&2.05&0.53&&K3.7&$ 0.612$&2.78&0.68&&K3.0&$ 0.695$&2.57&0.38&&K3.2&$ 0.889$&3.28&0.45&early-Ke(H97)<M0(Sam)G4-K3(LR)K4(Ste)\\
    217& 05 35 18.45&$-$05 25 19.1&M5.6&$-1.559$&0.00&0.50&&M5.2&$-1.376$&0.56&0.34&&M5.6&$-1.559$&0.00&0.50&&M5.2&$-1.332$&0.65&0.34&\\
    218& 05 35 18.46&$-$05 24 07.1&M2.8&$-0.417$&1.31&0.04&&M2.7&$-0.398$&1.35&0.02&&M2.7&$-0.307$&1.55&0.03&&M2.7&$-0.294$&1.57&0.01&M3e(H97)\\
    219& 05 35 18.49&$-$05 23 29.3&M6.3&$-1.436$&0.37&0.53&&M5.8&$-1.259$&1.01&0.39&&M6.2&$-1.400$&0.47&0.54&&M5.8&$-1.171$&1.22&0.39&M0(H97)K-M(LR)\\
    220& 05 35 18.66&$-$05 23 14.1&K2.5&$ 0.762$&2.55&0.00&&K2.7&$ 0.748$&2.59&0.07&&K6.2&$ 0.445$&1.78&0.52&&K4.2&$ 0.873$&2.70&0.06&G5-K1(H13)K2-K5e(H97)\\
    221& 05 35 18.67&$-$05 23 56.5&M4.7&$-1.099$&0.74&0.23&&M4.5&$-1.023$&0.97&0.14&&M4.7&$-1.041$&0.87&0.22&&M4.4&$-0.959$&1.10&0.13&K8-M0e\\
    222& 05 35 18.75&$-$05 22 02.3&M1.8&$-0.198$&2.57&0.00&&M1.8&$-0.198$&2.57&0.00&&M1.9&$-0.008$&2.97&0.00&&M1.9&$-0.007$&2.98&0.00&M1(H13)M2.5(H97)K5-M2(LR)M1(SHC-ir)\\
    223& 05 35 18.83&$-$05 22 23.0&M5.5&$-1.080$&2.90&0.53&&M5.3&$-0.893$&3.54&0.45&&M5.4&$-0.838$&3.46&0.52&&M5.2&$-0.595$&4.24&0.42&M3(H97)K5-M3(LR)\\
    224& 05 35 18.85&$-$05 21 41.2&K6.7&$-0.197$&1.48&0.10&&K6.6&$-0.143$&1.62&0.06&&K6.8&$-0.067$&1.75&0.08&&K6.7&$-0.016$&1.88&0.04&K8(H13)\\
    225& 05 35 18.86&$-$05 23 28.9&M3.0&$-0.836$&1.63&0.24&&M2.9&$-0.736$&1.89&0.16&&M3.0&$-0.705$&1.91&0.23&&M2.9&$-0.592$&2.19&0.14&<M2:(H13)M0e(H97)K4-M2(LR)\\
    226& 05 35 18.88&$-$05 24 17.5&M6.2&$-1.158$&0.30&0.00&&M6.2&$-1.157$&0.31&0.00&&M6.2&$-1.126$&0.39&0.00&&M6.2&$-1.126$&0.39&0.00&M3(H97)\\
    227& 05 35 18.70&$-$05 22 56.9&K4.2&$ 0.021$&2.83&0.50&&K3.3&$ 0.257$&3.63&0.39&&K1.4&$ 0.569$&4.14&0.14&&K1.3&$ 0.659$&4.50&0.19&\\
    228& 05 35 18.94&$-$05 22 18.8&K7.8&$-0.388$&3.99&0.35&&K7.8&$-0.239$&4.46&0.28&&K7.8&$-0.031$&4.72&0.25&&K7.5&$ 0.112$&5.08&0.15&K7(H97)K5-M2(LR)\\
    229& 05 35 18.96&$-$05 23 22.1&M7.1&$-1.285$&2.69&0.01&&M7.1&$-1.181$&3.09&0.02&&M7.2&$-1.033$&3.25&0.01&&M7.2&$-0.899$&3.72&0.02&\\
    230& 05 35 19.02&$-$05 25 03.0&M4.0&$-1.250$&0.43&0.24&&M3.2&$-1.083$&1.03&0.09&&M4.0&$-1.216$&0.50&0.24&&M3.2&$-1.002$&1.21&0.08&K7(H97)\\
    231& 05 35 19.12&$-$05 23 27.1&M0.3&$-0.386$&1.65&0.00&&M0.3&$-0.386$&1.65&0.00&&M0.4&$-0.254$&1.94&0.00&&M0.4&$-0.254$&1.94&0.00&K7(H13)K8(H97)K5-M2(LR)M1(SHC-ir)\\
    232& 05 35 19.13&$-$05 22 34.6&M5.9&$-1.253$&3.07&0.01&&M5.8&$-1.257$&3.10&0.01&&M5.8&$-1.023$&3.61&0.01&&M5.7&$-1.013$&3.68&0.01&\\
    233& 05 35 19.06&$-$05 23 49.7&K2.8&$-0.308$&1.97&0.09&&K2.7&$-0.268$&2.21&0.15&&K2.7&$-0.083$&2.46&0.02&&K2.8&$-0.072$&2.54&0.05&G8-K2(H97)<=K5(P)>G6(LR)\\
    234& 05 35 19.20&$-$05 22 50.8&K4.6&$-0.277$&2.86&0.32&&K4.6&$-0.136$&3.36&0.30&&K4.6&$ 0.020$&3.48&0.21&&K4.4&$ 0.167$&3.90&0.15&K5(H97)K8-M0(H97)K5-M2(LR)\\
    235& 05 35 19.46&$-$05 22 21.7&M4.8&$-1.183$&2.78&0.31&&M4.7&$-1.070$&3.23&0.31&&M4.1&$-0.959$&3.19&0.08&&M4.2&$-0.917$&3.35&0.11&M3.5(H13)>=M6(H97)\\
    236& 05 35 19.61&$-$05 23 57.4&M1.6&$-0.764$&1.36&0.31&&M1.7&$-0.635$&1.74&0.23&&M1.7&$-0.652$&1.60&0.29&&M1.7&$-0.499$&2.03&0.21&M0\\
    237& 05 35 19.65&$-$05 24 26.6&M2.9&$-0.315$&1.32&0.52&&M1.7&$-0.103$&1.73&0.14&&M2.8&$-0.200$&1.56&0.48&&M1.7&$ 0.032$&2.02&0.12&M0-M2.5e(H97)M0.5(P)<M0(Sam)\\
    238& 05 35 19.82&$-$05 22 21.6&K5.8&$-0.941$&2.27&1.99&&K5.3&$-0.544$&3.65&1.83&&K6.5&$-0.735$&2.67&1.80&&K6.6&$-0.254$&4.22&1.67&late-M(H97)\\
    239& 05 35 19.84&$-$05 24 47.9&M3.8&$-0.794$&0.89&0.13&&M3.6&$-0.725$&1.11&0.08&&M3.8&$-0.715$&1.08&0.12&&M3.3&$-0.599$&1.45&0.03&K7(H13)M1(H97)M6-M6.5(H97)\\
    240& 05 35 19.92&$-$05 24 02.7&M5.6&$-1.042$&0.45&0.20&&M5.4&$-0.936$&0.80&0.14&&M5.6&$-1.005$&0.53&0.20&&M5.4&$-0.869$&0.95&0.14&M2(H97)\\
    241& 05 35 20.03&$-$05 22 26.5&M4.5&$-0.906$&3.35&0.01&&M4.5&$-0.904$&3.36&0.01&&M4.3&$-0.668$&3.88&0.00&&M4.3&$-0.666$&3.89&0.00&cont+emis(H13)M5(H97)\\
    242& 05 35 20.04&$-$05 25 37.6&M0.4&$-0.166$&1.31&0.00&&M0.4&$-0.166$&1.31&0.00&&M0.5&$-0.061$&1.54&0.00&&M0.5&$-0.061$&1.54&0.00&M0.3(P)\\
    243& 05 35 20.15&$-$05 25 33.7&K7.8&$-1.761$&0.49&0.24&&K6.6&$-1.624$&0.77&0.07&&K7.7&$-1.707$&0.59&0.20&&K6.7&$-1.562$&0.90&0.06&M1(SHC-ir)M:(H97)\\
    244& 05 35 20.15&$-$05 22 28.3&M6.5&$-1.399$&1.73&0.24&&M6.5&$-1.318$&2.08&0.27&&M6.5&$-1.259$&2.07&0.25&&M6.4&$-1.137$&2.52&0.26&M3(H13)\\
    245& 05 35 20.17&$-$05 23 08.7&M3.7&$-0.703$&3.37&0.66&&M3.3&$-0.463$&4.13&0.44&&M3.3&$-0.377$&4.16&0.55&&M2.7&$-0.137$&4.76&0.27&M2(SHC-ir)\\
    246& 05 35 20.13&$-$05 21 33.7&K9.1&$ 0.083$&1.93&0.00&&K9.1&$ 0.083$&1.93&0.00&&K9.3&$ 0.236$&2.27&0.00&&K9.3&$ 0.236$&2.27&0.00&<M0(Sam)\\
    247& 05 35 20.39&$-$05 22 13.8&M1.7&$-0.066$&2.22&0.12&&M1.0&$ 0.038$&2.46&0.00&&M1.8&$ 0.101$&2.58&0.12&&M1.1&$ 0.222$&2.86&0.00&M0(H13)\\
    248& 05 35 20.46&$-$05 23 29.8&K8.5&$-0.066$&1.88&0.13&&K8.5&$ 0.001$&2.09&0.11&&K8.5&$ 0.103$&2.24&0.10&&K8.4&$ 0.165$&2.41&0.07&\\
    249& 05 35 20.49&$-$05 23 31.2&M6.0&$-1.368$&1.68&0.42&&M5.7&$-1.229$&2.21&0.36&&M5.9&$-1.235$&1.99&0.41&&M5.7&$-1.050$&2.62&0.35&\\
    250& 05 35 20.53&$-$05 21 41.1&M4.7&$-1.215$&1.34&0.62&&M4.3&$-1.049$&1.81&0.39&&M4.6&$-1.105$&1.59&0.59&&M4.2&$-0.929$&2.05&0.36&\\
    251& 05 35 20.54&$-$05 24 20.9&M3.7&$-0.922$&1.15&0.11&&M3.2&$-0.832$&1.46&0.02&&M3.7&$-0.813$&1.42&0.10&&M3.2&$-0.719$&1.71&0.01&\\
    252& 05 35 20.62&$-$05 22 55.8&M5.1&$-1.722$&0.97&0.37&&M4.9&$-1.587$&1.43&0.30&&M5.1&$-1.654$&1.12&0.38&&M4.9&$-1.477$&1.69&0.30&M:(H97)M4-M8(SHC-ir)\\
    253& 05 35 20.62&$-$05 24 46.5&M3.0&$-0.427$&1.81&0.58&&M2.7&$-0.227$&2.34&0.36&&M3.0&$-0.277$&2.13&0.55&&M2.3&$-0.042$&2.65&0.24&M2e(H97)\\
    254& 05 35 20.64&$-$05 22 45.6&M3.5&$-1.012$&2.98&0.19&&M3.4&$-0.934$&3.18&0.11&&M3.5&$-0.777$&3.48&0.18&&M3.4&$-0.691$&3.70&0.10&M4.5(H13)M1(H97)\\
    255& 05 35 20.66&$-$05 25 10.7&M5.3&$-1.145$&0.37&0.26&&M5.1&$-1.023$&0.77&0.18&&M5.3&$-1.112$&0.46&0.25&&M5.0&$-0.957$&0.92&0.18&\\
    256& 05 35 20.67&$-$05 23 53.3&M5.7&$-0.673$&0.27&0.11&&M5.6&$-0.620$&0.44&0.08&&M5.7&$-0.650$&0.33&0.11&&M5.6&$-0.584$&0.53&0.08&M4-M6e(H13)\\
    257& 05 35 20.71&$-$05 22 31.5&M4.6&$-0.842$&3.03&0.00&&M4.6&$-0.842$&3.03&0.00&&M4.6&$-0.606$&3.57&0.00&&M4.6&$-0.607$&3.56&0.00&M2(H13)\\
    258& 05 35 20.77&$-$05 21 55.2&K6.4&$-0.249$&1.69&0.03&&K6.2&$-0.224$&1.73&0.00&&K6.6&$-0.109$&1.99&0.02&&K6.5&$-0.097$&2.01&0.00&M0(H97)K5(Ste)\\
    259& 05 35 20.84&$-$05 21 30.1&M4.6&$-0.590$&1.15&0.15&&M4.5&$-0.541$&1.29&0.09&&M4.6&$-0.497$&1.36&0.14&&M4.4&$-0.449$&1.48&0.08&M4.5(H97)\\
    260& 05 35 20.84&$-$05 21 21.5&M4.5&$-1.460$&1.88&4.32&&M4.2&$-0.996$&3.44&3.61&&M4.0&$-1.307$&2.17&3.68&&M3.3&$-0.694$&4.10&2.82&K4-K6e(H13)K7(H97)\\
    261& 05 35 20.90&$-$05 25 34.3&M6.3&$-1.738$&0.19&0.00&&M6.3&$-1.738$&0.20&0.00&&M6.3&$-1.725$&0.23&0.00&&M6.3&$-1.723$&0.23&0.00&\\
    262& 05 35 20.91&$-$05 23 21.8&M3.6&$-1.006$&1.15&0.08&&M3.4&$-0.954$&1.33&0.03&&M3.6&$-0.899$&1.41&0.07&&M3.4&$-0.851$&1.55&0.03&M0(H97)\\
    263& 05 35 20.92&$-$05 21 50.9&K7.7&$-0.256$&1.74&0.15&&K7.1&$-0.177$&1.88&0.05&&K7.7&$-0.101$&2.07&0.12&&K7.0&$-0.032$&2.14&0.00&K-M1e(H13)M:e(H97)\\
    264& 05 35 21.01&$-$05 22 22.8&M6.1&$-1.477$&1.65&0.00&&M6.1&$-1.477$&1.65&0.00&&M6.1&$-1.356$&1.91&0.00&&M6.1&$-1.351$&1.93&0.00&M3:(H97)\\
    265& 05 35 21.02&$-$05 23 55.7&M6.3&$-1.095$&1.01&0.00&&M6.3&$-1.095$&1.01&0.00&&M6.3&$-1.010$&1.22&0.00&&M6.3&$-1.010$&1.22&0.00&\\
    266& 05 35 21.03&$-$05 22 25.1&M4.2&$-1.087$&2.49&0.15&&M4.0&$-1.053$&2.58&0.09&&M4.0&$-0.905$&2.88&0.12&&M3.9&$-0.848$&3.04&0.08&\\
    267& 05 35 21.05&$-$05 23 49.0&K4.3&$ 0.715$&0.94&0.16&&K4.3&$ 0.800$&1.28&0.17&&K2.4&$ 1.020$&1.76&0.00&&K2.4&$ 1.019$&1.77&0.01&G8(H97)<=K5(P)K3(CK)K1-K2(Sam)SB2(R)K2\\
    268& 05 35 21.19&$-$05 23 33.1&M5.6&$-1.145$&1.49&0.23&&M5.3&$-1.026$&1.91&0.17&&M5.4&$-0.979$&1.91&0.19&&M5.2&$-0.869$&2.28&0.16&M4.5(H13)M6(H97)M6(SHC-ir)\\
    269& 05 35 21.20&$-$05 24 00.1&M5.7&$-1.041$&2.82&0.00&&M5.7&$-1.043$&2.81&0.00&&M5.7&$-0.829$&3.30&0.00&&M5.6&$-0.826$&3.32&0.00&M3::(H13)\\
    270& 05 35 21.24&$-$05 22 59.5&M3.6&$-0.708$&2.74&0.47&&M3.3&$-0.525$&3.29&0.30&&M3.4&$-0.454$&3.34&0.41&&M2.6&$-0.263$&3.77&0.13&M3(H97)M1.5-M4(SHC-ir)\\
    271& 05 35 21.15&$-$05 25 56.9&M0.6&$-0.259$&2.07&0.03&&M0.4&$-0.232$&2.13&0.00&&M0.6&$-0.073$&2.47&0.00&&M0.6&$-0.073$&2.47&0.00&M0(H13)M0.5(H97)\\
    272& 05 35 21.29&$-$05 24 57.3&K5.3&$-0.002$&0.87&0.51&&K5.6&$ 0.187$&1.50&0.45&&K5.4&$ 0.082$&1.04&0.48&&K5.7&$ 0.315$&1.77&0.42&K1-K2(Sam)K4(Ste)\\
    273& 05 35 21.29&$-$05 22 15.7&M5.7&$-1.561$&1.16&0.39&&M5.6&$-1.420$&1.71&0.38&&M5.7&$-1.458$&1.42&0.39&&M5.6&$-1.281$&2.03&0.38&M1.5(H97)\\
    274& 05 35 21.32&$-$05 23 46.0&M4.9&$-1.387$&0.69&1.20&&M3.8&$-1.132$&1.51&0.68&&M4.8&$-1.330$&0.82&1.17&&M3.1&$-0.969$&1.94&0.54&\\
    275& 05 35 21.33&$-$05 24 11.5&K8.7&$-0.508$&1.61&0.00&&K8.7&$-0.507$&1.61&0.00&&K8.9&$-0.380$&1.90&0.00&&K8.9&$-0.380$&1.90&0.00&M0(H13)M0.5(H97)K7:(P)\\
    276& 05 35 21.37&$-$05 23 45.4&K6.5&$-0.292$&1.27&0.16&&K6.5&$-0.212$&1.52&0.12&&K6.5&$-0.175$&1.52&0.13&&K6.5&$-0.091$&1.75&0.09&\\
    277& 05 35 21.50&$-$05 23 16.7&M5.4&$-0.699$&1.89&0.12&&M5.3&$-0.640$&2.07&0.09&&M5.3&$-0.535$&2.28&0.11&&M5.2&$-0.467$&2.48&0.08&M3.5(H97)\\
    278& 05 35 21.63&$-$05 23 25.7&M6.5&$-1.534$&1.05&0.34&&M6.4&$-1.428$&1.47&0.34&&M6.5&$-1.457$&1.24&0.35&&M6.4&$-1.314$&1.73&0.34&M5.5(H97)\\
    279& 05 35 21.68&$-$05 21 47.0&K8.1&$-0.400$&3.58&0.51&&K8.5&$-0.206$&4.25&0.48&&K7.9&$-0.058$&4.25&0.36&&K8.3&$ 0.131$&4.87&0.34&\\
    280& 05 35 21.66&$-$05 25 26.3&K8.3&$-0.543$&1.49&0.31&&K8.6&$-0.407$&1.94&0.27&&K8.2&$-0.402$&1.78&0.26&&K8.5&$-0.250$&2.26&0.23&M0(H97)\\
    281& 05 35 21.73&$-$05 23 48.3&M6.6&$-1.232$&2.43&0.00&&M6.5&$-1.220$&2.51&0.00&&M6.5&$-1.027$&2.94&0.00&&M6.5&$-1.010$&3.01&0.00&<M2(H97)\\
    282& 05 35 21.78&$-$05 23 39.2&M3.4&$-0.924$&2.30&0.62&&M2.6&$-0.707$&2.83&0.28&&M3.4&$-0.738$&2.70&0.59&&M2.5&$-0.490$&3.26&0.23&K5-K7(H97)\\
    283& 05 35 21.78&$-$05 23 10.7&M4.5&$-0.536$&2.17&0.20&&M4.3&$-0.493$&2.28&0.12&&M4.4&$-0.377$&2.51&0.17&&M4.2&$-0.336$&2.61&0.10&M1.5(H97)\\
    284& 05 35 21.82&$-$05 22 40.2&M6.5&$-1.511$&0.60&0.19&&M6.4&$-1.447$&0.86&0.18&&M6.5&$-1.458$&0.72&0.19&&M6.4&$-1.379$&1.01&0.18&M0.5(H13)M0-M5(H97)\\
    285& 05 35 21.84&$-$05 23 06.5&M3.5&$-0.758$&4.72&0.00&&M3.5&$-0.755$&4.73&0.00&&M3.5&$-0.397$&5.52&0.00&&M3.5&$-0.392$&5.54&0.00&M5(SHC-ir)\\
    286& 05 35 21.85&$-$05 22 08.3&M1.9&$-0.667$&1.50&0.08&&M1.6&$-0.616$&1.61&0.02&&M1.9&$-0.557$&1.74&0.08&&M1.7&$-0.495$&1.87&0.01&M2(H97)\\
    287& 05 35 21.89&$-$05 23 55.5&M2.7&$-0.887$&1.21&0.50&&M1.9&$-0.684$&1.65&0.20&&M2.6&$-0.779$&1.43&0.46&&M1.9&$-0.555$&1.93&0.18&M1(H97)\\
    288& 05 35 21.81&$-$05 23 53.8&K3.7&$ 0.376$&0.80&0.02&&K4.1&$ 0.367$&0.79&0.06&&K4.1&$ 0.392$&0.79&0.05&&K3.7&$ 0.464$&1.00&0.01&K3(H97)G6-K3(H97)K4(Ste)\\
    289& 05 35 22.09&$-$05 24 32.9&M5.2&$-0.668$&0.61&0.17&&M4.9&$-0.577$&0.91&0.11&&M5.1&$-0.614$&0.73&0.17&&M4.9&$-0.505$&1.07&0.10&\\
    290& 05 35 22.11&$-$05 24 20.2&M5.6&$-1.347$&1.19&0.37&&M5.3&$-1.187$&1.70&0.27&&M5.6&$-1.245$&1.43&0.37&&M5.3&$-1.049$&2.01&0.26&\\
    291& 05 35 22.12&$-$05 22 34.0&M3.3&$-0.609$&3.90&0.19&&M3.3&$-0.532$&4.12&0.14&&M3.4&$-0.312$&4.54&0.19&&M3.3&$-0.219$&4.79&0.13&K7(H97)\\
    292& 05 35 22.14&$-$05 22 13.4&M5.0&$-1.491$&0.17&0.06&&M4.8&$-1.481$&0.20&0.02&&M4.8&$-1.476$&0.20&0.02&&M4.8&$-1.466$&0.23&0.01&M5(H97)\\
    293& 05 35 22.24&$-$05 22 17.4&M6.5&$-1.530$&2.06&0.52&&M6.3&$-1.350$&2.76&0.51&&M6.5&$-1.364$&2.46&0.54&&M6.1&$-1.148$&3.26&0.52&M4-M5(H97)\\
    294& 05 35 22.19&$-$05 24 24.8&K4.1&$ 0.106$&1.31&0.48&&K4.2&$ 0.284$&1.98&0.49&&K4.1&$ 0.247$&1.60&0.41&&K4.1&$ 0.465$&2.33&0.40&K2-K3(H97)<K7(P)K4\\
    295& 05 35 22.41&$-$05 25 09.5&M2.4&$-0.559$&0.68&0.05&&M2.4&$-0.536$&0.74&0.03&&M2.4&$-0.502$&0.81&0.04&&M2.4&$-0.478$&0.87&0.03&M3.5(H13)\\
    296& 05 35 22.43&$-$05 24 13.5&M4.5&$-1.347$&0.37&0.00&&M4.5&$-1.347$&0.37&0.00&&M4.5&$-1.320$&0.43&0.00&&M4.5&$-1.320$&0.43&0.00&M0.5-M1.5(H97)M0.1(P)K5(Ste)\\
    297& 05 35 22.44&$-$05 22 01.1&K4.4&$-0.265$&2.70&0.53&&K4.6&$-0.084$&3.39&0.56&&K4.4&$ 0.037$&3.31&0.37&&K4.4&$ 0.231$&3.97&0.37&K5-K6(H13)K2-K4(H97)<K7(P)\\
    298& 05 35 22.46&$-$05 25 45.1&M4.2&$-0.901$&0.34&0.00&&M4.2&$-0.901$&0.34&0.00&&M4.2&$-0.874$&0.40&0.00&&M4.2&$-0.874$&0.40&0.00&\\
    299& 05 35 22.33&$-$05 24 14.3&K8.2&$-0.024$&1.48&0.10&&K8.0&$ 0.031$&1.60&0.05&&K8.2&$ 0.112$&1.77&0.07&&K7.9&$ 0.158$&1.86&0.02&M0.5-M1.5(H97)M0.1(P)K5(Ste)\\
    300& 05 35 22.56&$-$05 23 43.7&K4.3&$ 0.053$&1.96&0.00&&K4.3&$ 0.053$&1.97&0.00&&K4.5&$ 0.192$&2.25&0.00&&K4.5&$ 0.192$&2.25&0.00&<=K7(H97)M0(E)<M0(Sam)\\
    301& 05 35 22.63&$-$05 21 37.3&M4.8&$-1.317$&2.48&0.01&&M4.8&$-1.293$&2.56&0.01&&M4.8&$-1.106$&2.97&0.01&&M4.7&$-1.091$&3.03&0.00&\\
    302& 05 35 22.70&$-$05 21 41.1&M6.2&$-2.097$&0.03&0.02&&M6.2&$-2.061$&0.22&0.06&&M6.2&$-2.104$&0.03&0.05&&M6.3&$-2.067$&0.16&0.06&\\
    303& 05 35 22.75&$-$05 21 57.7&M6.2&$-1.496$&2.79&0.04&&M6.3&$-1.342$&3.35&0.05&&M6.5&$-1.245$&3.32&0.04&&M6.2&$-1.066$&4.02&0.05&\\
    304& 05 35 22.83&$-$05 25 47.5&M5.1&$-0.951$&0.38&0.00&&M5.1&$-0.952$&0.38&0.00&&M5.1&$-0.921$&0.45&0.00&&M5.1&$-0.920$&0.45&0.00&M5.5(H13)\\
    305& 05 35 22.84&$-$05 22 27.0&M3.7&$-1.277$&3.13&0.00&&M3.7&$-1.285$&3.09&0.00&&M3.6&$-1.010$&3.77&0.00&&M3.6&$-1.019$&3.73&0.00&K:(H97)\\
    306& 05 35 22.97&$-$05 22 41.5&K4.6&$-0.121$&5.47&0.05&&K5.6&$-0.167$&5.47&0.17&&K6.1&$ 0.152$&6.03&0.14&&K6.1&$ 0.241$&6.27&0.09&K3-M0(H13)K5-K7(H97)\\
    307& 05 35 23.02&$-$05 25 36.1&M6.1&$-1.943$&0.47&0.43&&M5.9&$-1.813$&1.02&0.44&&M6.1&$-1.898$&0.58&0.44&&M5.9&$-1.706$&1.32&0.45&\\
    308& 05 35 23.21&$-$05 21 35.8&M4.2&$-0.842$&1.85&0.04&&M4.2&$-0.829$&1.88&0.03&&M4.2&$-0.708$&2.13&0.02&&M4.1&$-0.697$&2.16&0.02&M3.5(H13)\\
    309& 05 35 23.33&$-$05 21 25.3&K8.4&$-0.767$&3.18&0.50&&K8.0&$-0.567$&3.73&0.33&&K8.2&$-0.469$&3.77&0.37&&K7.8&$-0.270$&4.28&0.23&K5-M0.5e(H97)\\
    310& 05 35 23.59&$-$05 25 26.3&M4.6&$-0.844$&1.22&0.59&&M3.9&$-0.713$&1.59&0.33&&M4.3&$-0.760$&1.40&0.53&&M3.8&$-0.577$&1.91&0.31&M3-M3.5e(H13)\\
    311& 05 35 23.66&$-$05 23 46.3&M3.4&$-0.644$&0.91&0.12&&M3.3&$-0.589$&1.05&0.06&&M3.4&$-0.572$&1.06&0.12&&M3.3&$-0.507$&1.23&0.06&M1(H97)<K7(SHC-ir)\\
    312& 05 35 23.67&$-$05 23 32.0&K7.2&$-0.314$&2.00&0.05&&K6.8&$-0.279$&2.05&0.00&&K7.2&$-0.135$&2.38&0.02&&K7.1&$-0.123$&2.39&0.00&K6-K7(H13)K5(H97)\\
    313& 05 35 23.73&$-$05 23 19.9&M3.5&$-1.152$&2.72&0.62&&M2.5&$-0.935$&3.22&0.23&&M2.6&$-0.832$&3.36&0.30&&M2.5&$-0.688$&3.73&0.20&M3e(H97)\\
    314& 05 35 23.82&$-$05 23 34.3&M2.9&$-0.310$&2.25&0.43&&M2.3&$-0.144$&2.61&0.19&&M2.7&$-0.113$&2.65&0.36&&M2.2&$ 0.060$&3.03&0.16&M1e(H13)M1e(H97)\\
    315& 05 35 23.81&$-$05 24 16.8&M3.9&$-0.996$&1.15&0.22&&M3.7&$-0.887$&1.50&0.14&&M3.9&$-0.895$&1.39&0.21&&M3.7&$-0.761$&1.79&0.13&\\
    316& 05 35 23.89&$-$05 23 33.2&M0.4&$-1.192$&2.23&0.52&&K9.4&$-0.984$&2.75&0.28&&M0.4&$-0.992$&2.64&0.45&&K8.9&$-0.765$&3.13&0.18&M1e(H13)M1e(H97)\\
    317& 05 35 23.98&$-$05 25 09.9&M4.7&$-1.215$&0.44&0.61&&M4.0&$-1.091$&0.78&0.34&&M4.3&$-1.195$&0.50&0.54&&M4.0&$-1.031$&0.91&0.33&M1(H97)\\
    318& 05 35 24.10&$-$05 21 32.7&M4.5&$-0.640$&1.12&0.14&&M4.3&$-0.615$&1.18&0.08&&M4.5&$-0.556$&1.31&0.12&&M4.3&$-0.532$&1.36&0.07&\\
    319& 05 35 24.12&$-$05 21 55.7&M5.9&$-1.176$&1.41&0.15&&M5.7&$-1.113$&1.63&0.11&&M5.8&$-1.061$&1.68&0.15&&M5.7&$-0.985$&1.92&0.11&M4.5(H97)\\
    320& 05 35 24.34&$-$05 26 00.3&M5.7&$-1.117$&0.00&0.04&&M5.8&$-1.111$&0.00&0.03&&M5.7&$-1.117$&0.00&0.04&&M5.7&$-1.108$&0.02&0.03&\\
    321& 05 35 24.44&$-$05 24 39.9&K8.9&$-0.040$&1.10&0.22&&K8.3&$ 0.068$&1.35&0.10&&K8.9&$ 0.062$&1.32&0.19&&K8.3&$ 0.176$&1.56&0.08&M0e(H97)K7(H97)K6(Ste)\\
    322& 05 35 24.47&$-$05 24 01.1&M5.8&$-1.164$&0.80&0.11&&M5.7&$-1.119$&0.95&0.08&&M5.8&$-1.100$&0.95&0.11&&M5.6&$-1.017$&1.24&0.08&M1-M3:(H13)\\
    323& 05 35 24.26&$-$05 25 18.7&K9.9&$-0.152$&0.87&0.03&&K9.6&$-0.138$&0.89&0.00&&K9.9&$-0.077$&1.03&0.02&&K9.7&$-0.067$&1.05&0.00&K4-K5e(H97)K0-K2(Sam)K6(Ste)\\
    324& 05 35 24.51&$-$05 25 01.6&M2.4&$-0.818$&1.30&0.31&&M2.2&$-0.687$&1.62&0.17&&M2.4&$-0.706$&1.54&0.28&&M2.1&$-0.561$&1.88&0.15&M1e(H97)\\
    325& 05 35 24.66&$-$05 22 42.6&M4.5&$-0.853$&4.00&0.04&&M4.5&$-0.834$&4.13&0.08&&M4.5&$-0.552$&4.71&0.07&&M4.5&$-0.502$&4.91&0.10&M4.5(H13)M6:(H97)\\
    326& 05 35 24.70&$-$05 24 35.7&K7.0&$-0.194$&1.60&0.24&&K7.0&$-0.079$&1.94&0.18&&K7.0&$-0.046$&1.91&0.20&&K7.0&$ 0.075$&2.24&0.14&K8\\
    327& 05 35 24.82&$-$05 21 57.7&M5.0&$-1.787$&0.11&0.00&&M5.0&$-1.785$&0.12&0.01&&M5.0&$-1.779$&0.13&0.00&&M5.0&$-1.775$&0.14&0.01&K6(H97)\\
    328& 05 35 24.89&$-$05 25 10.1&M5.6&$-0.925$&0.42&0.07&&M5.5&$-0.886$&0.54&0.05&&M5.6&$-0.890$&0.50&0.07&&M5.5&$-0.840$&0.65&0.05&M3(H13)M5(SHC-ir)\\
    329& 05 35 24.96&$-$05 24 01.5&M3.5&$-1.215$&2.43&1.72&&M2.5&$-0.821$&3.48&0.93&&M3.5&$-1.009$&2.86&1.62&&M2.5&$-0.545$&4.02&0.83&\\
    330& 05 35 25.06&$-$05 22 58.5&K4.5&$ 0.330$&3.11&0.25&&K4.5&$ 0.447$&3.54&0.25&&K4.5&$ 0.636$&3.75&0.16&&K4.4&$ 0.749$&4.09&0.13&\\
    331& 05 35 25.08&$-$05 23 53.7&M2.0&$-0.598$&0.96&0.66&&M1.1&$-0.321$&1.67&0.33&&M2.0&$-0.515$&1.13&0.64&&M0.9&$-0.178$&1.96&0.28&\\
    332& 05 35 25.09&$-$05 23 46.7&K7.3&$ 0.019$&0.62&0.08&&K7.0&$ 0.062$&0.69&0.02&&K7.3&$ 0.073$&0.73&0.07&&K7.0&$ 0.115$&0.79&0.01&K2-K4(Sam)K5(Ste)\\
    333& 05 35 25.14&$-$05 22 25.2&M5.9&$-1.020$&3.26&0.51&&M5.7&$-0.859$&3.91&0.49&&M5.9&$-0.766$&3.86&0.51&&M5.6&$-0.537$&4.68&0.48&M1.5-M2.5(H97)\\
    334& 05 35 25.22&$-$05 24 57.3&M2.5&$-1.861$&0.22&0.45&&M2.0&$-1.680$&0.62&0.20&&M2.5&$-1.845$&0.24&0.44&&M0.5&$-1.530$&0.92&0.03&cont+emis(H13)<M1e(H97)\\
    335& 05 35 25.34&$-$05 25 29.5&M5.6&$-0.919$&0.86&0.10&&M5.6&$-0.877$&0.98&0.07&&M5.6&$-0.849$&1.02&0.10&&M5.6&$-0.794$&1.17&0.07&M5(SHC-ir)\\
    336& 05 35 25.38&$-$05 24 11.4&M0.6&$-1.583$&1.54&1.42&&K9.4&$-1.209$&2.56&0.89&&M0.1&$-1.404$&1.83&1.12&&K9.6&$-0.993$&2.98&0.79&M1:(H97)\\
    337& 05 35 25.39&$-$05 23 45.7&M7.6&$-1.347$&1.99&0.00&&M7.6&$-1.339$&2.02&0.00&&M7.6&$-1.193$&2.36&0.00&&M7.7&$-1.183$&2.35&0.00&\\
    338& 05 35 25.43&$-$05 21 51.5&K6.7&$-0.253$&2.51&0.29&&K7.7&$-0.140$&3.00&0.36&&K6.8&$-0.028$&2.98&0.24&&K7.7&$ 0.101$&3.48&0.29&\\
    339& 05 35 25.43&$-$05 23 33.2&M3.4&$-0.851$&2.12&0.31&&M2.5&$-0.719$&2.40&0.07&&M3.4&$-0.683$&2.47&0.30&&M2.5&$-0.534$&2.78&0.05&\\
    340& 05 35 25.47&$-$05 21 34.4&K7.4&$-0.444$&3.52&0.12&&K7.7&$-0.386$&3.77&0.15&&K7.5&$-0.140$&4.16&0.07&&K7.5&$-0.095$&4.30&0.06&K6(H97)\\
    341& 05 35 25.49&$-$05 21 35.5&K3.5&$-0.276$&3.36&0.23&&K3.7&$-0.177$&3.77&0.28&&K3.3&$ 0.094$&4.16&0.10&&K4.1&$ 0.113$&4.29&0.19&K6(H97)\\
    342& 05 35 25.72&$-$05 23 09.4&K5.7&$-0.367$&3.24&0.65&&K6.0&$-0.145$&4.01&0.60&&K6.1&$-0.080$&3.82&0.54&&K6.4&$ 0.169$&4.61&0.49&K6-K7e(H13)K8e(H97)\\
    343& 05 35 26.00&$-$05 25 47.8&K8.8&$-0.188$&2.42&0.22&&K9.0&$-0.086$&2.77&0.21&&K8.4&$ 0.050$&2.90&0.13&&K8.6&$ 0.133$&3.15&0.11&K8(H97)M0.1(P)\\
    344& 05 35 26.06&$-$05 21 21.0&K4.6&$ 0.208$&4.85&0.12&&K4.6&$ 0.274$&5.08&0.10&&K6.0&$ 0.442$&5.34&0.21&&K1.6&$ 0.881$&6.66&0.00&K3-K6(H13)\\
    345& 05 35 26.15&$-$05 25 39.4&M6.2&$-1.206$&0.55&0.19&&M6.0&$-1.132$&0.80&0.13&&M6.1&$-1.161$&0.66&0.19&&M6.0&$-1.068$&0.95&0.13&\\
    346& 05 35 26.17&$-$05 22 57.2&M4.9&$-1.013$&3.46&0.27&&M4.7&$-0.921$&3.74&0.18&&M4.8&$-0.731$&4.09&0.24&&M4.6&$-0.639$&4.36&0.16&<M3(H13)M5-M6(H97)\\
    347& 05 35 26.19&$-$05 25 20.4&M4.1&$-1.079$&0.14&0.04&&M4.0&$-1.068$&0.18&0.02&&M4.1&$-1.069$&0.16&0.04&&M4.0&$-1.054$&0.22&0.02&M6(H13)M4(H97)\\
    348& 05 35 26.41&$-$05 23 02.5&M3.0&$-1.283$&2.68&0.67&&M2.9&$-1.061$&3.32&0.49&&M3.0&$-1.060$&3.16&0.63&&M2.7&$-0.807$&3.82&0.40&K4-K5\\
    349& 05 35 26.43&$-$05 25 31.5&M6.7&$-1.464$&0.30&0.18&&M6.4&$-1.354$&0.74&0.14&&M6.7&$-1.433$&0.38&0.18&&M6.4&$-1.294$&0.88&0.14&K0-K2::(H13)\\
    350& 05 35 26.35&$-$05 25 40.1&K1.3&$ 0.498$&0.56&0.45&&K0.6&$ 0.671$&1.28&0.51&&K2.8&$ 0.500$&0.47&0.44&&K0.8&$ 0.776$&1.53&0.53&G5(Par)G0III(HB)G-K:(GS)K1\\
    351& 05 35 26.94&$-$05 24 48.2&M5.4&$-1.036$&0.55&0.00&&M5.4&$-1.034$&0.56&0.00&&M5.4&$-0.988$&0.66&0.00&&M5.4&$-0.989$&0.66&0.00&M6.5(H97)M7-M8(H97)M5.5(SHC)M6.5(SHC-ir)\\
    352& 05 35 26.97&$-$05 24 00.5&M4.7&$-0.849$&0.70&0.07&&M4.6&$-0.821$&0.78&0.05&&M4.7&$-0.793$&0.82&0.07&&M4.6&$-0.761$&0.91&0.04&M3.5\\
    353& 05 35 27.31&$-$05 23 36.5&K6.9&$-0.025$&2.05&0.25&&K7.2&$ 0.088$&2.44&0.23&&K7.1&$ 0.153$&2.43&0.22&&K7.2&$ 0.284$&2.82&0.18&K4(Sam)\\
    354& 05 35 27.78&$-$05 23 32.7&M5.1&$-1.135$&2.24&0.63&&M4.6&$-0.939$&2.87&0.40&&M4.8&$-0.924$&2.77&0.57&&M4.3&$-0.757$&3.24&0.33&\\
    355& 05 35 27.86&$-$05 23 23.7&M5.3&$-1.456$&1.88&0.41&&M5.0&$-1.277$&2.46&0.29&&M5.2&$-1.294$&2.27&0.40&&M4.9&$-1.089$&2.90&0.27&\\
    356& 05 35 28.14&$-$05 23 06.6&M5.1&$-0.709$&3.41&0.41&&M4.7&$-0.567$&3.87&0.25&&M4.7&$-0.406$&4.13&0.33&&M4.6&$-0.272$&4.51&0.23&M3e(H97)\\
    357& 05 35 28.21&$-$05 24 58.2&K6.5&$-0.492$&1.45&0.44&&K6.4&$-0.305$&2.02&0.34&&K6.7&$-0.364$&1.72&0.41&&K6.5&$-0.144$&2.33&0.29&K5e(H13)K6-K8e(H97)\\
    358& 05 35 28.55&$-$05 25 04.7&M6.5&$-1.466$&0.18&0.00&&M6.5&$-1.464$&0.18&0.00&&M6.5&$-1.452$&0.21&0.00&&M6.5&$-1.452$&0.21&0.00&\\
    359& 05 35 28.38&$-$05 25 03.5&M2.6&$-0.314$&0.48&0.14&&M2.4&$-0.247$&0.64&0.07&&M2.6&$-0.272$&0.57&0.13&&M2.4&$-0.196$&0.75&0.06&M1.5(H97)M4(E)\\
    360& 05 35 23.22&$-$05 25 54.4&M6.2&$-1.468$&1.65&0.25&&M5.9&$-1.372$&2.05&0.20&&M6.1&$-1.329$&2.00&0.25&&M5.8&$-1.211$&2.44&0.22&M2:(H13)\\
    361& 05 35 16.76&$-$05 23 16.6&K9.7&$-0.501$&1.78&1.58&&K9.3&$-0.129$&3.01&1.36&&K9.6&$-0.329$&2.18&1.55&&K9.2&$ 0.156$&3.69&1.34&G4-K5(LR)\\
\enddata
\end{deluxetable*}
\end{longrotatetable}


==> allspt.tex <==
\begin{center}
\startlongtable
\begin{deluxetable*}{rccccccccccccccccccccccccccccccccc}
\tablecaption{Young stars in North America Nebula and Pelican}\label{tabe_spt}
\tablewidth{700pt}
\tablehead{\multicolumn{1}{c}{} &\multicolumn{1}{c}{RA} &\multicolumn{1}{c}{DEC}  &\multicolumn{1}{c}{Hectospec}  &\multicolumn{1}{c}{Hydra}  &\multicolumn{1}{c}{Deimos}   &\multicolumn{1}{c}{Norris} &\multicolumn{1}{c}{Used}\\
\multicolumn{1}{c}{} &\multicolumn{1}{c}{(J2000)} &\multicolumn{1}{c}{(J2000)} &\multicolumn{1}{c}{Spt/$REX_{7465}$} &\multicolumn{1}{c}{Spt/$REX_{7465}$}  &\multicolumn{1}{c}{Spt/$REX_{7465}$} &\multicolumn{1}{c}{Spt/$REX_{7465}$}  &\multicolumn{1}{c}{Spt/$REX_{7465}$} }
\startdata
1  & 20 49 11.78  &$+$44 12 33.3  &K7.0/0  &\nodata&\nodata&\nodata&K7.0/0\\
2  & 20 49 14.46  &$+$44 14 50.3  &M4.8/0  &\nodata&\nodata&\nodata&M4.8/0\\
3  & 20 49 20.28  &$+$44 35 13.8  &M2.4/0  &\nodata&\nodata&\nodata&M2.4/0\\
4  & 20 49 24.75  &$+$44 35 22.0  &M5.6/0  &\nodata&\nodata&\nodata&M5.6/0\\
5  & 20 49 32.18  &$+$44 17 03.4  &M1.6/0.28  &\nodata&\nodata&\nodata&M1.6/0.28\\
6  & 20 49 35.85  &$+$44 30 45.3  &Cont  &\nodata&\nodata&\nodata&Cont\\
7  & 20 49 53.49  &$+$44 10 17.2  &\nodata  &\nodata&\nodata&M3.6/0&M3.6/0\\
8  & 20 50 06.07  &$+$44 17 49.3  &\nodata  &M4.0/0&\nodata&\nodata&M4.0/0\\
9  & 20 50 09.89  &$+$44 15 22.0  &M1.4/0;M1.0/0  &\nodata&\nodata&\nodata&M1.2/0\\
10  & 20 50 22.42  &$+$44 19 17.6  &\nodata  &M3.0/0.38&M4.6/0.10&\nodata&M3.0/0.38\\
11  & 20 50 27.71  &$+$44 23 29.2  &K0.2/0  &\nodata&\nodata&\nodata&K0.2/0\\
12  & 20 50 31.96  &$+$44 12 48.7  &6750/0  &6750/0&\nodata&\nodata&6750/0\\
13  & 20 50 32.33  &$+$44 26 17.9  &K4.2/0;K7.0/0  &\nodata&K4.4/0&\nodata&K5.6/0\\
14  & 20 50 33.06  &$+$44 15 38.9  &M1.2/0.08  &M3.6/2.04&\nodata&\nodata&M1.2/0.08\\
15  & 20 50 36.94  &$+$44 21 40.8  &Cont  &Cont&Cont&\nodata&Cont\\
16  & 20 50 36.97  &$+$44 20 49.8  &K7.0/0;K7.4/0  &\nodata&\nodata&\nodata&K7.2/0\\
17  & 20 50 37.02  &$+$44 18 24.6  &K7.6/0.46  &M1.4/0.98&\nodata&\nodata&K7.6/0.46\\
18  & 20 50 37.44  &$+$44 21 15.9  &M3.4/0.24  &\nodata&\nodata&M2.4/0.04&M3.4/0.24\\
19  & 20 50 39.12  &$+$44 30 38.1  &K7.0/0.76  &\nodata&K7.0/0.16&\nodata&K7.0/0.76\\
20  & 20 50 40.27  &$+$44 30 49.2  &K4.6/2.10  &\nodata&\nodata&K4.0/0.60&K4.6/2.10\\
21  & 20 50 40.46  &$+$44 20 21.7  &M4.0/0;M4.0/0  &\nodata&\nodata&\nodata&M4.0/0\\
22  & 20 50 40.54  &$+$44 20 51.0  &M2.8/0  &\nodata&\nodata&\nodata&M2.8/0\\
23  & 20 50 42.77  &$+$44 21 55.0  &Cont  &Cont&Cont&\nodata&Cont\\
24  & 20 50 43.53  &$+$44 15 52.0  &M0.6/0  &\nodata&\nodata&\nodata&M0.6/0\\
25  & 20 50 43.72  &$+$44 16 49.3  &Cont  &\nodata&\nodata&\nodata&Cont\\
26  & 20 50 44.93  &$+$44 15 55.1  &M2.8/0.14;M3.0/0.30  &M2.6/0.28&\nodata&\nodata&M2.9/0.22\\
27  & 20 50 45.74  &$+$44 11 55.3  &\nodata  &Cont&\nodata&\nodata&Cont\\
28  & 20 50 46.08  &$+$44 19 10.4  &M2.0/0;M1.8/0  &\nodata&\nodata&\nodata&M1.9/0\\
29  & 20 50 46.40  &$+$44 31 12.4  &K9.8/0  &\nodata&\nodata&\nodata&K9.8/0\\
30  & 20 50 47.00  &$+$44 17 29.5  &M0.8/0  &\nodata&\nodata&K9.2/0&M0.8/0\\
31  & 20 50 48.10  &$+$44 33 37.1  &M2.4/0;M2.2/0  &\nodata&\nodata&\nodata&M2.3/0\\
32  & 20 50 48.58  &$+$44 21 04.5  &M4.0/0.06  &\nodata&\nodata&\nodata&M4.0/0.06\\
33  & 20 50 48.71  &$+$44 20 53.7  &K9.2/0.14  &M0.4/0.50&\nodata&\nodata&K9.2/0.14\\
34  & 20 50 48.80  &$+$44 19 23.7  &M2.8/0.34;M3.8/0.34  &M3.4/0.64&\nodata&\nodata&M3.3/0.34\\
35  & 20 50 50.38  &$+$44 50 11.6  &\nodata  &\nodata&Cont&\nodata&Cont\\
36  & 20 50 52.56  &$+$44 16 44.3  &K3.0/0;K3.4/0  &G6.0/0&\nodata&\nodata&K3.2/0\\
37  & 20 50 53.16  &$+$44 23 53.7  &M3.2/0;M3.0/0  &M2.6/0&\nodata&\nodata&M3.1/0\\
38  & 20 50 53.57  &$+$44 21 01.1  &K6.2/0;K6.2/0  &\nodata&\nodata&\nodata&K6.2/0\\
39  & 20 50 53.62  &$+$44 24 29.9  &G6.2/0  &\nodata&\nodata&G6.0/0&G6.2/0\\
40  & 20 50 53.87  &$+$44 21 38.8  &M5.0/0  &\nodata&\nodata&\nodata&M5.0/0\\
41  & 20 50 54.18  &$+$44 38 08.3  &K8.2/0.16  &\nodata&\nodata&K7.6/0.56&K8.2/0.16\\
42  & 20 50 54.29  &$+$44 17 52.8  &\nodata  &M3.4/0.58&\nodata&\nodata&M3.4/0.58\\
43  & 20 50 54.88  &$+$44 22 58.4  &M0.4/0.30  &M0.4/0.96&\nodata&\nodata&M0.4/0.30\\
44  & 20 50 55.58  &$+$44 24 24.6  &M1.6/2.48  &\nodata&\nodata&\nodata&M1.6/2.48\\
45  & 20 50 55.65  &$+$44 17 50.3  &K8.4/0.26  &\nodata&\nodata&K7.8/0.52&K8.4/0.26\\
46  & 20 50 57.46  &$+$44 24 46.6  &K4.2/0.22  &K6.4/0.46&\nodata&\nodata&K4.2/0.22\\
47  & 20 50 58.18  &$+$44 29 59.2  &M0.6/0  &\nodata&\nodata&M0.8/0&M0.6/0\\
48  & 20 50 58.34  &$+$44 14 32.5  &G6.6/0;G7.0/0  &\nodata&\nodata&\nodata&G6.8/0\\
49  & 20 50 58.39  &$+$44 14 44.5  &M1.0/0;M0.0/0  &\nodata&\nodata&\nodata&M0.5/0\\
50  & 20 50 58.70  &$+$44 17 31.0  &K8.2/0.44  &\nodata&\nodata&K7.0/0.88&K8.2/0.44\\
51  & 20 50 58.74  &$+$44 23 17.8  &M2.6/0  &M2.6/0&\nodata&\nodata&M2.6/0\\
52  & 20 50 59.04  &$+$44 19 53.9  &M3.2/0.10;M3.4/0.08  &\nodata&\nodata&\nodata&M3.3/0.09\\
53  & 20 50 59.47  &$+$44 19 39.3  &M2.8/0.16  &\nodata&\nodata&\nodata&M2.8/0.16\\
54  & 20 50 59.74  &$+$44 40 49.1  &K4.4/0.36  &\nodata&\nodata&\nodata&K4.4/0.36\\
55  & 20 51 00.89  &$+$44 31 49.9  &K5.8/0.46  &\nodata&\nodata&\nodata&K5.8/0.46\\
56  & 20 51 01.44  &$+$44 13 29.7  &\nodata  &\nodata&K9.8/0&\nodata&K9.8/0\\
57  & 20 51 01.46  &$+$44 15 34.7  &K9.8/0.12;K9.0/0.40  &K8.4/0.54&\nodata&\nodata&K9.4/0.26\\
58  & 20 51 01.56  &$+$44 15 42.2  &K6.6/0.28  &\nodata&\nodata&K7.0/0.52&K6.6/0.28\\
59  & 20 51 02.19  &$+$44 20 09.4  &M4.6/0  &\nodata&\nodata&\nodata&M4.6/0\\
60  & 20 51 03.18  &$+$44 24 04.1  &M0.8/0.28  &\nodata&\nodata&\nodata&M0.8/0.28\\
61  & 20 51 03.32  &$+$44 24 15.7  &M0.8/0.34  &K9.2/0.76&\nodata&\nodata&M0.8/0.34\\
62  & 20 51 03.35  &$+$44 14 40.4  &\nodata  &M5.4/0.54&\nodata&\nodata&M5.4/0.54\\
63  & 20 51 04.64  &$+$44 23 50.3  &G6.0/0;G6.0/0  &\nodata&\nodata&\nodata&G6.0/0\\
64  & 20 51 05.47  &$+$44 14 00.4  &M4.0/0.08  &M4.8/0.06&\nodata&\nodata&M4.0/0.08\\
65  & 20 51 05.69  &$+$44 16 32.5  &K3.0/0  &\nodata&\nodata&G6.0/0&K3.0/0\\
66  & 20 51 06.25  &$+$44 18 30.9  &\nodata  &Cont&\nodata&\nodata&Cont\\
67  & 20 51 08.03  &$+$44 31 50.4  &M1.0/0.20;M0.8/0.20  &\nodata&\nodata&\nodata&M0.9/0.20\\
68  & 20 51 08.28  &$+$44 16 51.4  &\nodata  &\nodata&M4.6/0&\nodata&M4.6/0\\
69  & 20 51 08.94  &$+$44 16 42.0  &\nodata  &\nodata&M4.2/0&\nodata&M4.2/0\\
70  & 20 51 09.49  &$+$44 33 29.7  &M3.8/0.14;M3.8/0.14  &\nodata&\nodata&\nodata&M3.8/0.14\\
71  & 20 51 10.98  &$+$44 36 44.7  &M3.6/0;M3.4/0  &\nodata&\nodata&\nodata&M3.5/0\\
72  & 20 51 12.09  &$+$44 18 47.7  &M4.0/0.08;M4.8/0.46  &\nodata&\nodata&\nodata&M4.4/0.27\\
73  & 20 51 12.52  &$+$44 18 09.4  &K8.0/0  &\nodata&\nodata&\nodata&K8.0/0\\
74  & 20 51 13.43  &$+$44 26 18.4  &M2.6/0.32  &\nodata&M2.4/0.38&\nodata&M2.6/0.32\\
75  & 20 51 13.65  &$+$44 32 22.7  &K9.8/0;M0.2/0  &\nodata&\nodata&K9.2/0&M0.0/0\\
76  & 20 51 13.79  &$+$44 31 53.2  &M4.4/0  &\nodata&\nodata&\nodata&M4.4/0\\
77  & 20 51 14.55  &$+$44 13 38.1  &M3.2/0.18  &M3.4/0.28&\nodata&\nodata&M3.2/0.18\\
78  & 20 51 15.12  &$+$44 18 17.8  &K7.8/0.52  &\nodata&\nodata&K7.2/0.50&K7.8/0.52\\
79  & 20 51 15.61  &$+$44 14 55.3  &K6.6/0  &K7.0/0&\nodata&\nodata&K6.6/0\\
80  & 20 51 16.05  &$+$44 15 00.2  &K6.6/0.22  &\nodata&\nodata&\nodata&K6.6/0.22\\
81  & 20 51 16.50  &$+$44 22 58.0  &G6.8/0;K3.0/0  &G6.0/0&\nodata&\nodata&G9.9/0\\
82  & 20 51 17.70  &$+$44 18 30.2  &M0.8/0.22  &M0.8/0.62&\nodata&\nodata&M0.8/0.22\\
83  & 20 51 18.23  &$+$44 13 08.3  &K6.4/0.14;K7.4/0.16  &\nodata&\nodata&K7.0/0.80&K6.9/0.15\\
84  & 20 51 19.44  &$+$44 19 30.7  &M1.0/0.26;M0.4/0.92  &M0.2/1.82&\nodata&\nodata&M0.7/0.59\\
85  & 20 51 19.85  &$+$44 23 06.7  &M2.2/0.40  &\nodata&\nodata&M2.4/0.44&M2.2/0.40\\
86  & 20 51 20.97  &$+$44 26 19.7  &K8.0/0.30  &K8.8/0.46&\nodata&\nodata&K8.0/0.30\\
87  & 20 51 22.45  &$+$44 20 47.3  &M5.0/0.14  &\nodata&\nodata&\nodata&M5.0/0.14\\
88  & 20 51 22.58  &$+$44 25 15.9  &Cont  &\nodata&\nodata&\nodata&Cont\\
89  & 20 51 22.66  &$+$44 21 07.8  &K7.6/0.24  &K8.2/0.90&\nodata&\nodata&K7.6/0.24\\
90  & 20 51 22.80  &$+$44 33 42.8  &K8.0/0.14;K7.6/0.14  &\nodata&\nodata&K9.4/0.32&K7.8/0.14\\
91  & 20 51 23.60  &$+$44 15 42.7  &M1.8/0.16  &\nodata&M2.6/0.30&\nodata&M1.8/0.16\\
92  & 20 51 23.64  &$+$44 31 37.1  &M3.6/0;M3.4/0  &\nodata&M2.8/0&\nodata&M3.5/0\\
93  & 20 51 23.66  &$+$44 35 22.6  &M0.8/0.12  &\nodata&\nodata&\nodata&M0.8/0.12\\
94  & 20 51 24.04  &$+$44 32 57.2  &M2.8/0;M3.4/0  &\nodata&\nodata&\nodata&M3.1/0\\
95  & 20 51 24.14  &$+$44 17 57.0  &M5.6/0.16;M5.8/0.16  &\nodata&\nodata&\nodata&M5.7/0.16\\
96  & 20 51 24.40  &$+$44 13 04.7  &Cont  &\nodata&Cont&\nodata&Cont\\
97  & 20 51 24.64  &$+$44 17 55.1  &\nodata  &M3.2/0&\nodata&\nodata&M3.2/0\\
98  & 20 51 24.70  &$+$44 18 18.8  &M3.2/0;M3.0/0  &\nodata&\nodata&\nodata&M3.1/0\\
99  & 20 51 26.20  &$+$44 30 34.6  &M4.6/0.12  &\nodata&M4.6/0.02&\nodata&M4.6/0.12\\
100  & 20 51 26.27  &$+$44 16 59.6  &M7.8/0  &\nodata&\nodata&\nodata&M7.8/0\\
101  & 20 51 26.45  &$+$43 53 12.6  &K7.4/0  &\nodata&\nodata&\nodata&K7.4/0\\
102  & 20 51 26.53  &$+$44 36 28.7  &K8.8/0.40;K7.2/0.24  &\nodata&\nodata&\nodata&K8.0/0.32\\
103  & 20 51 26.75  &$+$44 04 24.7  &M1.8/0.58  &M1.8/1.22&\nodata&\nodata&M1.8/0.58\\
104  & 20 51 26.97  &$+$44 13 15.6  &K7.8/0.28  &K8.8/0.40&K7.2/0.37&K9.2/0.92&K7.8/0.28\\
105  & 20 51 28.44  &$+$44 26 01.2  &K6.4/0;K7.8/0  &\nodata&\nodata&K7.6/0&K7.1/0\\
106  & 20 51 28.56  &$+$44 15 45.5  &M2.6/0  &M2.4/0&\nodata&\nodata&M2.6/0\\
107  & 20 51 29.67  &$+$44 32 19.7  &G6.0/0  &\nodata&\nodata&G6.0/0&G6.0/0\\
108  & 20 51 30.56  &$+$44 03 45.1  &K4.6/0;K4.4/0  &\nodata&\nodata&\nodata&K4.5/0\\
109  & 20 51 30.89  &$+$44 06 59.6  &K3.2/0;K3.0/0  &\nodata&\nodata&\nodata&K3.1/0\\
110  & 20 51 31.64  &$+$44 13 01.4  &M2.4/0  &\nodata&M2.0/0&\nodata&M2.4/0\\
111  & 20 51 31.87  &$+$44 02 54.3  &M4.2/0.16;M4.6/0.20  &\nodata&\nodata&\nodata&M4.4/0.18\\
112  & 20 51 32.77  &$+$43 11 22.3  &K9.4/0  &\nodata&\nodata&\nodata&K9.4/0\\
113  & 20 51 32.77  &$+$44 23 48.1  &K9.4/0.34  &K8.4/0.38&M1.4/0.78&\nodata&K9.4/0.34\\
114  & 20 51 33.11  &$+$44 36 59.7  &K9.4/0  &\nodata&\nodata&\nodata&K9.4/0\\
115  & 20 51 33.37  &$+$44 26 37.0  &G6.4/0  &G7.0/0&\nodata&\nodata&G6.4/0\\
116  & 20 51 33.39  &$+$44 34 54.4  &K3.6/0.30;K4.0/0.40  &\nodata&\nodata&K0.6/0.26&K3.8/0.35\\
117  & 20 51 33.69  &$+$44 10 14.6  &M2.2/0;M2.0/0  &K9.6/0&\nodata&M0.2/0&M2.1/0\\
118  & 20 51 35.39  &$+$44 30 39.2  &\nodata  &\nodata&M2.8/0&\nodata&M2.8/0\\
119  & 20 51 37.60  &$+$44 20 04.6  &M2.4/0  &M2.2/0&\nodata&M2.2/0&M2.4/0\\
120  & 20 51 37.95  &$+$43 23 04.6  &K9.2/0.14  &\nodata&\nodata&\nodata&K9.2/0.14\\
121  & 20 51 38.26  &$+$43 57 14.0  &M3.2/0  &\nodata&\nodata&\nodata&M3.2/0\\
122  & 20 51 38.65  &$+$44 03 41.0  &M2.2/0.50  &M4.0/1.46&\nodata&\nodata&M2.2/0.50\\
123  & 20 51 39.24  &$+$44 24 28.1  &G6.6/0  &\nodata&\nodata&G6.8/0&G6.6/0\\
124  & 20 51 39.95  &$+$44 33 14.3  &K6.4/0.50  &\nodata&\nodata&K6.4/0.14&K6.4/0.50\\
125  & 20 51 40.69  &$+$43 13 14.0  &M5.8/0  &\nodata&\nodata&\nodata&M5.8/0\\
126  & 20 51 41.25  &$+$43 47 54.9  &K7.6/0  &\nodata&\nodata&\nodata&K7.6/0\\
127  & 20 51 41.40  &$+$44 15 07.2  &\nodata  &Cont&Cont&Cont&Cont\\
128  & 20 51 41.90  &$+$44 16 08.3  &K6.0/0.84  &K6.2/0.66&\nodata&\nodata&K6.0/0.84\\
129  & 20 51 42.09  &$+$44 38 56.7  &K3.0/0  &\nodata&\nodata&K1.0/0&K3.0/0\\
130  & 20 51 42.89  &$+$44 07 30.7  &K8.6/0.64  &K7.0/0.28&\nodata&\nodata&K8.6/0.64\\
131  & 20 51 44.73  &$+$44 08 47.0  &\nodata  &M0.0/0&\nodata&\nodata&M0.0/0\\
132  & 20 51 45.20  &$+$43 49 02.4  &G7.0/0  &K7.0/0&\nodata&\nodata&G7.0/0\\
133  & 20 51 45.98  &$+$44 28 35.4  &M2.0/0.26;M2.8/0.68  &\nodata&M2.8/0.62&\nodata&M2.4/0.47\\
134  & 20 51 46.12  &$+$44 23 09.1  &M5.2/0  &\nodata&\nodata&\nodata&M5.2/0\\
135  & 20 51 47.41  &$+$44 32 08.2  &M2.6/0  &\nodata&M2.6/0&\nodata&M2.6/0\\
136  & 20 51 48.54  &$+$44 05 19.7  &M2.2/0.04;M2.2/0.12  &M2.0/0.10&\nodata&\nodata&M2.2/0.08\\
137  & 20 51 48.75  &$+$44 23 40.8  &M2.0/0  &\nodata&M2.2/0&\nodata&M2.0/0\\
138  & 20 51 48.85  &$+$44 11 02.8  &K7.4/0.28;K7.4/0.26  &K7.8/0.36&\nodata&\nodata&K7.4/0.27\\
139  & 20 51 51.25  &$+$44 15 12.3  &M2.8/0  &\nodata&\nodata&\nodata&M2.8/0\\
140  & 20 51 52.01  &$+$43 10 46.9  &Cont  &\nodata&\nodata&\nodata&Cont\\
141  & 20 51 52.24  &$+$44 18 21.4  &M2.4/0.46  &\nodata&\nodata&\nodata&M2.4/0.46\\
142  & 20 51 52.90  &$+$44 15 57.5  &\nodata  &\nodata&M1.8/0.24&\nodata&M1.8/0.24\\
143  & 20 51 55.68  &$+$44 33 52.7  &\nodata  &\nodata&\nodata&G6.0/0&G6.0/0\\
144  & 20 51 57.21  &$+$44 02 16.1  &K7.2/0.38  &\nodata&\nodata&\nodata&K7.2/0.38\\
145  & 20 51 57.50  &$+$44 27 17.4  &M3.6/0  &\nodata&\nodata&\nodata&M3.6/0\\
146  & 20 51 58.04  &$+$44 04 21.0  &M4.2/0.14;M4.0/0.08  &\nodata&\nodata&\nodata&M4.1/0.11\\
147  & 20 51 58.47  &$+$44 37 24.2  &K7.6/0  &\nodata&\nodata&\nodata&K7.6/0\\
148  & 20 51 58.63  &$+$44 14 56.8  &K8.6/0.56  &K7.8/0.80&K9.4/0.71&\nodata&K8.6/0.56\\
149  & 20 51 58.67  &$+$44 30 06.3  &Cont  &\nodata&\nodata&\nodata&Cont\\
150  & 20 51 58.68  &$+$44 30 27.4  &M3.6/0.38;M3.4/0.32  &\nodata&M3.4/0.24&\nodata&M3.5/0.35\\
151  & 20 51 59.19  &$+$44 25 43.9  &K8.0/0.16  &K8.0/0.50&\nodata&\nodata&K8.0/0.16\\
152  & 20 51 59.42  &$+$43 50 42.0  &K3.4/0  &\nodata&\nodata&\nodata&K3.4/0\\
153  & 20 51 59.40  &$+$44 16 22.1  &K4.2/0.50;K4.2/0.58  &\nodata&\nodata&K7.0/1.90&K4.2/0.54\\
154  & 20 52 00.16  &$+$44 19 59.0  &M1.8/0  &M0.6/0&\nodata&\nodata&M1.8/0\\
155  & 20 52 00.97  &$+$44 28 41.5  &M1.8/0.42  &\nodata&M1.6/0.31&\nodata&M1.8/0.42\\
156  & 20 52 01.11  &$+$44 32 39.1  &K5.6/0  &\nodata&\nodata&K7.0/0&K5.6/0\\
157  & 20 52 01.61  &$+$44 20 32.6  &M1.8/0  &\nodata&\nodata&\nodata&M1.8/0\\
158  & 20 52 02.66  &$+$44 27 28.8  &M2.0/0  &\nodata&M1.2/0&\nodata&M2.0/0\\
159  & 20 52 02.91  &$+$44 13 51.9  &M2.6/0  &\nodata&M2.8/0&\nodata&M2.6/0\\
160  & 20 52 03.64  &$+$44 28 38.0  &M2.2/0;M2.2/0  &\nodata&M2.6/0&\nodata&M2.2/0\\
161  & 20 52 05.28  &$+$44 17 29.3  &M1.0/0  &\nodata&\nodata&\nodata&M1.0/0\\
162  & 20 52 06.73  &$+$44 27 55.7  &K8.8/0  &\nodata&\nodata&\nodata&K8.8/0\\
163  & 20 52 06.74  &$+$44 33 55.0  &M2.0/0.38  &\nodata&\nodata&\nodata&M2.0/0.38\\
164  & 20 52 07.96  &$+$43 54 16.2  &\nodata  &M3.0/0&\nodata&\nodata&M3.0/0\\
165  & 20 52 08.56  &$+$44 34 15.1  &M3.2/0.58;M3.2/0.34  &\nodata&\nodata&\nodata&M3.2/0.46\\
166  & 20 52 10.99  &$+$44 08 10.2  &M2.0/0  &M0.4/0&\nodata&\nodata&M2.0/0\\
167  & 20 52 11.55  &$+$44 17 54.7  &\nodata  &\nodata&\nodata&K4.8/0&K4.8/0\\
168  & 20 52 12.92  &$+$44 20 53.4  &K4.0/0.46  &\nodata&\nodata&\nodata&K4.0/0.46\\
169  & 20 52 13.58  &$+$44 12 02.0  &\nodata  &\nodata&\nodata&K8.2/0&K8.2/0\\
170  & 20 52 13.57  &$+$43 40 38.9  &K8.8/0.60  &\nodata&\nodata&\nodata&K8.8/0.60\\
171  & 20 52 14.91  &$+$44 20 38.2  &M4.6/0.86  &\nodata&\nodata&\nodata&M4.6/0.86\\
172  & 20 52 15.12  &$+$44 17 20.5  &M4.8/0.12;M4.8/0.38  &\nodata&\nodata&\nodata&M4.8/0.25\\
173  & 20 52 15.14  &$+$43 30 07.5  &K6.8/0.30  &\nodata&\nodata&\nodata&K6.8/0.30\\
174  & 20 52 15.43  &$+$44 28 10.9  &K9.2/0.18;K9.0/0.22  &\nodata&K9.4/0.21&\nodata&K9.1/0.20\\
175  & 20 52 17.83  &$+$44 21 15.9  &K7.4/0  &\nodata&\nodata&\nodata&K7.4/0\\
176  & 20 52 18.37  &$+$44 25 02.1  &K4.0/0.86  &K4.0/0.06&\nodata&\nodata&K4.0/0.86\\
177  & 20 52 18.40  &$+$44 16 30.5  &K9.8/0.50;K9.2/0.54  &K8.4/0.50&\nodata&K8.4/0.30&K9.5/0.52\\
178  & 20 52 18.44  &$+$44 05 15.0  &M2.4/0.48  &\nodata&\nodata&\nodata&M2.4/0.48\\
179  & 20 52 19.68  &$+$44 24 49.2  &M4.0/0  &\nodata&\nodata&\nodata&M4.0/0\\
180  & 20 52 20.22  &$+$44 30 30.9  &K6.4/0  &\nodata&\nodata&\nodata&K6.4/0\\
181  & 20 52 20.31  &$+$43 58 42.7  &M3.4/0.20  &\nodata&\nodata&\nodata&M3.4/0.20\\
182  & 20 52 22.51  &$+$44 14 00.2  &G7.4/0;G6.2/0  &\nodata&\nodata&G6.0/0&G6.8/0\\
183  & 20 52 22.85  &$+$44 27 02.9  &M7.2/0.24;M7.0/0.42  &\nodata&\nodata&\nodata&M7.1/0.33\\
184  & 20 52 23.28  &$+$43 04 56.4  &M2.2/0  &\nodata&\nodata&\nodata&M2.2/0\\
185  & 20 52 24.01  &$+$44 31 55.4  &M4.0/0.06;M4.0/0.30  &\nodata&\nodata&\nodata&M4.0/0.18\\
186  & 20 52 24.56  &$+$44 23 55.2  &M3.2/0  &\nodata&\nodata&\nodata&M3.2/0\\
187  & 20 52 25.22  &$+$44 25 55.2  &\nodata  &\nodata&M2.2/0&\nodata&M2.2/0\\
188  & 20 52 25.37  &$+$44 14 32.4  &M4.8/0.46  &\nodata&\nodata&\nodata&M4.8/0.46\\
189  & 20 52 25.57  &$+$44 29 11.9  &M4.6/0  &\nodata&\nodata&\nodata&M4.6/0\\
190  & 20 52 25.89  &$+$44 25 22.2  &M4.6/0  &\nodata&\nodata&\nodata&M4.6/0\\
191  & 20 52 26.19  &$+$44 34 26.2  &\nodata  &\nodata&\nodata&Cont&Cont\\
192  & 20 52 26.72  &$+$44 26 33.2  &\nodata  &M1.0/0&\nodata&\nodata&M1.0/0\\
193  & 20 52 26.75  &$+$44 17 06.5  &G6.0/0;G6.0/0  &G6.0/0&\nodata&\nodata&G6.0/0\\
194  & 20 52 27.17  &$+$44 04 39.1  &M3.8/0.30  &M4.0/0.22&\nodata&\nodata&M3.8/0.30\\
195  & 20 52 28.02  &$+$44 03 31.0  &G6.2/0  &G6.0/0&\nodata&\nodata&G6.2/0\\
196  & 20 52 28.31  &$+$44 21 14.6  &K7.8/0.22;K7.8/0.28  &K9.0/0.58&K8.4/0.45&\nodata&K7.8/0.25\\
197  & 20 52 28.79  &$+$44 18 29.7  &M2.4/0;M2.6/0  &M2.4/0&M2.2/0&\nodata&M2.5/0\\
198  & 20 52 29.61  &$+$44 34 18.5  &M3.8/0  &\nodata&\nodata&\nodata&M3.8/0\\
199  & 20 52 29.76  &$+$44 21 04.6  &M3.8/0.16;M3.6/0.10  &\nodata&\nodata&\nodata&M3.7/0.13\\
200  & 20 52 30.80  &$+$44 30 35.1  &M0.2/0;M0.0/0  &\nodata&\nodata&\nodata&M0.1/0\\
201  & 20 52 30.88  &$+$44 20 11.6  &K8.6/0.70;K7.0/0.26  &K7.4/0.56&M0.0/0.87&\nodata&K7.8/0.48\\
202  & 20 52 32.11  &$+$44 28 24.2  &M3.2/0  &\nodata&\nodata&\nodata&M3.2/0\\
203  & 20 52 33.30  &$+$44 31 40.8  &M2.4/0  &\nodata&\nodata&\nodata&M2.4/0\\
204  & 20 52 33.79  &$+$44 24 26.3  &M2.8/0.34;M2.8/0.34  &\nodata&M2.6/0.32&\nodata&M2.8/0.34\\
205  & 20 52 34.35  &$+$44 17 40.2  &K9.8/0.58  &K8.6/1.30&K8.8/0.73&\nodata&K9.8/0.58\\
206  & 20 52 34.40  &$+$44 38 24.6  &K9.8/0;M0.4/0  &\nodata&\nodata&\nodata&M0.1/0\\
207  & 20 52 35.29  &$+$44 33 19.4  &K4.8/0;K4.6/0  &\nodata&K6.6/0&\nodata&K4.7/0\\
208  & 20 52 35.41  &$+$44 37 22.3  &M4.0/0  &\nodata&\nodata&\nodata&M4.0/0\\
209  & 20 52 35.52  &$+$44 19 10.4  &M0.2/0  &\nodata&\nodata&K8.2/0&M0.2/0\\
210  & 20 52 36.47  &$+$44 11 46.4  &K9.0/0;K8.8/0  &\nodata&\nodata&\nodata&K8.9/0\\
211  & 20 52 39.50  &$+$43 59 54.2  &M0.0/0  &\nodata&\nodata&\nodata&M0.0/0\\
212  & 20 52 39.93  &$+$44 05 49.3  &M2.8/0  &\nodata&\nodata&\nodata&M2.8/0\\
213  & 20 52 41.58  &$+$44 37 20.4  &\nodata  &\nodata&\nodata&\nodata& \\
214  & 20 52 41.70  &$+$44 34 07.1  &\nodata  &\nodata&K7.8/0&\nodata&K7.8/0\\
215  & 20 52 41.84  &$+$44 26 55.1  &M3.8/0;M4.2/0  &\nodata&\nodata&\nodata&M4.0/0\\
216  & 20 52 42.58  &$+$44 19 21.1  &M0.8/0  &\nodata&\nodata&\nodata&M0.8/0\\
217  & 20 52 42.80  &$+$44 19 10.2  &M0.2/1.32;K9.0/0.62  &\nodata&M0.4/0.52&\nodata&K9.6/0.97\\
218  & 20 52 44.23  &$+$44 17 50.3  &M4.6/0;M4.2/0  &\nodata&\nodata&\nodata&M4.4/0\\
219  & 20 52 46.14  &$+$44 24 57.8  &\nodata  &\nodata&Cont&\nodata&Cont\\
220  & 20 52 47.47  &$+$44 15 41.9  &M2.8/0;M2.8/0  &\nodata&M2.8/0&\nodata&M2.8/0\\
221  & 20 52 48.65  &$+$44 19 50.6  &K9.8/0.16  &M0.4/1.26&\nodata&\nodata&K9.8/0.16\\
222  & 20 52 49.07  &$+$44 15 20.2  &M2.6/0  &M1.8/0&M2.6/0&\nodata&M2.6/0\\
223  & 20 52 49.81  &$+$44 19 02.0  &K4.4/0;K4.8/0  &\nodata&\nodata&K6.6/0&K4.6/0\\
224  & 20 52 50.63  &$+$43 42 55.4  &M0.2/0  &\nodata&\nodata&\nodata&M0.2/0\\
225  & 20 52 51.90  &$+$44 25 44.3  &M4.8/0  &\nodata&\nodata&\nodata&M4.8/0\\
226  & 20 52 52.48  &$+$44 14 25.1  &\nodata  &\nodata&K7.0/0.60&\nodata&K7.0/0.60\\
227  & 20 52 53.41  &$+$44 19 36.5  &G6.6/0  &\nodata&G6.8/0&\nodata&G6.6/0\\
228  & 20 52 53.73  &$+$44 14 57.0  &K8.0/0.86  &\nodata&K9.0/0.71&\nodata&K8.0/0.86\\
229  & 20 52 54.30  &$+$43 52 16.6  &K9.2/0.34;K9.0/0.40  &\nodata&\nodata&\nodata&K9.1/0.37\\
230  & 20 52 55.39  &$+$44 16 57.8  &M3.2/0  &\nodata&\nodata&\nodata&M3.2/0\\
231  & 20 52 55.61  &$+$43 56 43.9  &M3.6/0  &\nodata&\nodata&\nodata&M3.6/0\\
232  & 20 52 56.91  &$+$44 26 00.5  &Cont  &\nodata&\nodata&\nodata&Cont\\
233  & 20 52 57.26  &$+$44 40 46.4  &K7.4/0;K6.6/0  &\nodata&\nodata&\nodata&K7.0/0\\
234  & 20 52 58.83  &$+$44 15 03.8  &\nodata  &Cont&\nodata&\nodata&Cont\\
235  & 20 53 00.56  &$+$44 36 35.7  &K9.2/0;M0.8/0  &\nodata&\nodata&\nodata&M0.0/0\\
236  & 20 53 01.78  &$+$44 19 05.7  &\nodata  &K8.6/0.76&K7.0/0.71&\nodata&K8.6/0.76\\
237  & 20 53 02.35  &$+$44 00 47.3  &M5.8/0  &\nodata&\nodata&\nodata&M5.8/0\\
238  & 20 53 03.27  &$+$44 39 48.9  &\nodata  &\nodata&\nodata&\nodata& \\
239  & 20 53 04.62  &$+$44 39 47.0  &K9.6/0  &\nodata&\nodata&\nodata&K9.6/0\\
240  & 20 53 05.72  &$+$44 42 37.0  &G6.4/0;G6.8/0  &\nodata&\nodata&G6.0/0&G6.6/0\\
241  & 20 53 05.93  &$+$44 15 38.6  &M2.6/0.30;M2.6/0.32  &\nodata&\nodata&\nodata&M2.6/0.31\\
242  & 20 53 07.40  &$+$44 14 37.9  &M4.2/0  &\nodata&\nodata&\nodata&M4.2/0\\
243  & 20 53 08.14  &$+$44 05 13.4  &M2.8/0.56  &M3.2/0.54&M3.2/0.22&\nodata&M2.8/0.56\\
244  & 20 53 09.04  &$+$44 30 10.7  &\nodata  &\nodata&\nodata&\nodata& \\
245  & 20 53 09.14  &$+$44 21 16.6  &M5.0/0.38  &\nodata&\nodata&\nodata&M5.0/0.38\\
246  & 20 53 10.28  &$+$44 21 48.9  &Cont  &\nodata&\nodata&\nodata&Cont\\
247  & 20 53 12.27  &$+$43 38 28.6  &K4.4/0  &\nodata&K3.2/0&\nodata&K4.4/0\\
248  & 20 53 12.50  &$+$44 35 24.6  &M4.4/0;M3.6/0  &\nodata&\nodata&\nodata&M4.0/0\\
249  & 20 53 12.49  &$+$44 31 06.7  &\nodata  &\nodata&\nodata&\nodata& \\
250  & 20 53 13.99  &$+$44 12 57.7  &K6.2/0.14  &\nodata&K4.4/0.18&\nodata&K6.2/0.14\\
251  & 20 53 14.57  &$+$44 29 06.4  &K6.4/0;K6.4/0  &\nodata&\nodata&\nodata&K6.4/0\\
252  & 20 53 14.90  &$+$44 34 34.7  &M2.2/0  &\nodata&\nodata&\nodata&M2.2/0\\
253  & 20 53 15.13  &$+$44 38 48.3  &K7.4/0.14;K8.0/0.02  &\nodata&\nodata&\nodata&K7.7/0.08\\
254  & 20 53 15.64  &$+$43 44 22.8  &M2.4/0.96  &M2.0/1.82&M2.6/1.33&\nodata&M2.4/0.96\\
255  & 20 53 15.88  &$+$44 29 47.5  &K9.0/0  &\nodata&\nodata&\nodata&K9.0/0\\
256  & 20 53 16.52  &$+$44 29 33.8  &M3.8/0.96  &\nodata&\nodata&\nodata&M3.8/0.96\\
257  & 20 53 16.68  &$+$44 40 54.1  &M4.6/0;M4.2/0  &\nodata&\nodata&\nodata&M4.4/0\\
258  & 20 53 16.83  &$+$44 25 41.8  &\nodata  &\nodata&\nodata&Cont&Cont\\
259  & 20 53 17.05  &$+$44 38 34.2  &\nodata  &\nodata&\nodata&\nodata& \\
260  & 20 53 17.70  &$+$44 03 05.4  &M6.0/1.16  &\nodata&\nodata&\nodata&M6.0/1.16\\
261  & 20 53 17.89  &$+$44 18 04.4  &M5.4/0  &\nodata&\nodata&\nodata&M5.4/0\\
262  & 20 53 18.91  &$+$44 14 38.8  &\nodata  &\nodata&\nodata&\nodata& \\
263  & 20 53 21.20  &$+$44 53 21.4  &M5.4/0  &\nodata&\nodata&\nodata&M5.4/0\\
264  & 20 53 22.34  &$+$44 38 52.9  &5800/0  &\nodata&\nodata&5200/0&5800/0\\
265  & 20 53 23.92  &$+$43 54 18.1  &5400/0;5800/0  &5200/0&\nodata&\nodata&M4.4/0\\
266  & 20 53 23.93  &$+$44 21 58.2  &M3.0/0.54  &\nodata&\nodata&\nodata&M3.0/0.54\\
267  & 20 53 24.67  &$+$44 02 31.0  &7500/0  &\nodata&\nodata&\nodata&7500/0\\
268  & 20 53 24.63  &$+$44 20 34.4  &K6.6/0  &\nodata&\nodata&\nodata&K6.6/0\\
269  & 20 53 25.75  &$+$44 10 45.6  &K6.0/0  &\nodata&\nodata&\nodata&K6.0/0\\
270  & 20 53 27.13  &$+$44 58 21.1  &Cont  &\nodata&\nodata&\nodata&Cont\\
271  & 20 53 27.15  &$+$44 27 11.0  &\nodata  &\nodata&M0.2/0&\nodata&M0.2/0\\
272  & 20 53 27.74  &$+$44 10 34.7  &K7.6/0;K7.4/0  &\nodata&\nodata&\nodata&K7.5/0\\
273  & 20 53 28.21  &$+$44 18 20.7  &M1.0/0  &\nodata&K9.0/0&\nodata&M1.0/0\\
274  & 20 53 29.33  &$+$44 27 29.7  &M5.6/0;M5.2/0  &\nodata&\nodata&\nodata&M5.4/0\\
275  & 20 53 29.69  &$+$44 23 56.9  &M0.4/0  &K8.8/0&\nodata&\nodata&M0.4/0\\
276  & 20 53 30.26  &$+$44 29 12.7  &K9.0/0.50;K8.4/0.36  &\nodata&\nodata&\nodata&K8.7/0.43\\
277  & 20 53 30.44  &$+$44 26 44.2  &K9.6/0.80;K9.8/0.32  &\nodata&\nodata&\nodata&K9.7/0.56\\
278  & 20 53 30.66  &$+$44 25 42.7  &M4.8/0  &\nodata&\nodata&\nodata&M4.8/0\\
279  & 20 53 31.09  &$+$44 23 26.7  &G6.6/0;G6.6/0  &G6.0/0&\nodata&G6.2/0&G6.6/0\\
280  & 20 53 31.28  &$+$44 19 09.6  &M2.2/0  &\nodata&\nodata&\nodata&M2.2/0\\
281  & 20 53 31.38  &$+$44 13 34.5  &K6.4/0.32;K6.4/0.58  &K4.4/0.48&\nodata&\nodata&K6.4/0.45\\
282  & 20 53 31.49  &$+$44 12 45.8  &M2.0/0  &\nodata&\nodata&\nodata&M2.0/0\\
283  & 20 53 31.96  &$+$44 09 47.0  &K7.8/0;K8.6/0  &\nodata&K7.4/0&\nodata&K8.2/0\\
284  & 20 53 32.05  &$+$44 29 06.1  &K7.4/0;K7.8/0  &\nodata&\nodata&\nodata&K7.6/0\\
285  & 20 53 33.29  &$+$44 23 28.7  &K9.8/0  &\nodata&\nodata&\nodata&K9.8/0\\
286  & 20 53 34.10  &$+$44 20 18.0  &M1.8/0;M2.0/0  &M0.4/0&\nodata&\nodata&M1.9/0\\
287  & 20 53 34.77  &$+$44 29 18.1  &K7.4/0;K6.2/0  &\nodata&\nodata&\nodata&K6.8/0\\
288  & 20 53 35.23  &$+$44 16 52.5  &\nodata  &\nodata&\nodata&\nodata& \\
289  & 20 53 35.44  &$+$44 27 48.3  &Cont  &Cont&\nodata&\nodata&Cont\\
290  & 20 53 35.58  &$+$44 27 23.8  &M4.0/0  &\nodata&\nodata&\nodata&M4.0/0\\
291  & 20 53 35.77  &$+$44 28 40.8  &M4.4/0;M4.0/0  &\nodata&\nodata&\nodata&M4.2/0\\
292  & 20 53 36.28  &$+$44 16 26.2  &K7.6/0;K7.8/0  &K7.0/0&\nodata&\nodata&K7.7/0\\
293  & 20 53 36.51  &$+$44 53 13.7  &M4.0/0  &\nodata&\nodata&\nodata&M4.0/0\\
294  & 20 53 38.29  &$+$44 14 50.7  &Cont  &\nodata&\nodata&\nodata&K7.7/0\\
295  & 20 53 38.54  &$+$44 25 43.5  &M0.0/0  &\nodata&K9.8/0&\nodata&M0.0/0\\
296  & 20 53 38.72  &$+$43 56 27.1  &M4.0/0.06  &\nodata&\nodata&\nodata&M4.0/0.06\\
297  & 20 53 38.75  &$+$44 26 29.9  &M4.2/0  &\nodata&\nodata&\nodata&M4.2/0\\
298  & 20 53 40.14  &$+$44 10 45.7  &\nodata  &K8.0/1.16&M0.2/1.64&\nodata&K8.0/1.16\\
299  & 20 53 41.81  &$+$44 27 03.1  &K7.2/0  &\nodata&\nodata&\nodata&K7.2/0\\
300  & 20 53 42.61  &$+$43 53 53.7  &Cont  &\nodata&\nodata&\nodata&Cont\\
301  & 20 53 42.70  &$+$44 03 48.7  &K7.0/0.76  &K7.6/1.80&\nodata&\nodata&K7.0/0.76\\
302  & 20 53 43.23  &$+$44 27 36.8  &M4.6/0  &\nodata&\nodata&\nodata&M4.6/0\\
303  & 20 53 43.42  &$+$44 23 12.8  &K9.2/0  &\nodata&\nodata&\nodata&K9.2/0\\
304  & 20 53 44.90  &$+$44 01 15.2  &M2.4/0  &M3.0/0&M2.6/0&\nodata&M2.4/0\\
305  & 20 53 45.07  &$+$44 25 17.9  &M0.6/0  &\nodata&M0.8/0&\nodata&M0.6/0\\
306  & 20 53 46.42  &$+$44 27 14.7  &M5.6/0.12  &\nodata&\nodata&\nodata&M5.6/0.12\\
307  & 20 53 46.55  &$+$44 10 49.4  &K6.2/0  &\nodata&K7.4/0&K7.0/0&K6.2/0\\
308  & 20 53 47.15  &$+$44 18 48.7  &\nodata  &\nodata&M2.0/0&\nodata&M2.0/0\\
309  & 20 53 54.73  &$+$44 19 42.1  &M2.0/0.70  &M0.4/0.18&M1.2/0.35&\nodata&M2.0/0.70\\
310  & 20 53 56.10  &$+$44 11 14.0  &Cont  &\nodata&Cont&\nodata&Cont\\
311  & 20 53 56.91  &$+$44 51 31.9  &M3.4/0.50  &\nodata&\nodata&\nodata&M3.4/0.50\\
312  & 20 53 57.51  &$+$44 20 32.6  &G6.6/0  &\nodata&G6.0/0&\nodata&G6.6/0\\
313  & 20 53 57.56  &$+$43 56 47.5  &Cont  &\nodata&Cont&\nodata&Cont\\
314  & 20 53 58.00  &$+$44 18 56.6  &M4.0/0  &\nodata&\nodata&\nodata&M4.0/0\\
315  & 20 53 58.24  &$+$44 25 46.2  &K6.6/0.36  &\nodata&\nodata&\nodata&K6.6/0.36\\
316  & 20 53 58.43  &$+$44 32 35.0  &5800/0  &\nodata&\nodata&9000/0&5800/0\\
317  & 20 53 58.56  &$+$44 25 36.4  &3900/0;4400/0  &\nodata&\nodata&\nodata&K7.7/0\\
318  & 20 54 02.41  &$+$44 08 17.4  &M1.4/0;M1.8/0  &\nodata&\nodata&\nodata&M1.6/0\\
319  & 20 54 03.85  &$+$44 01 47.8  &K7.6/0.80  &K8.4/1.42&\nodata&\nodata&K7.6/0.80\\
320  & 20 54 05.30  &$+$44 36 29.3  &K9.0/0;K7.4/0  &\nodata&\nodata&\nodata&K8.2/0\\
321  & 20 54 06.45  &$+$44 22 25.4  &\nodata  &Cont&\nodata&\nodata&Cont\\
322  & 20 54 06.71  &$+$44 28 13.1  &M4.8/0;M4.8/0  &\nodata&\nodata&\nodata&M4.8/0\\
323  & 20 54 08.76  &$+$44 30 11.5  &G6.4/0;G6.4/0  &\nodata&\nodata&\nodata&G6.4/0\\
324  & 20 54 09.95  &$+$44 10 00.3  &M3.4/0;M3.8/0  &\nodata&\nodata&\nodata&M3.6/0\\
325  & 20 54 10.12  &$+$44 31 03.0  &K3.2/0  &\nodata&\nodata&\nodata&K3.2/0\\
326  & 20 54 10.72  &$+$44 32 44.8  &M2.0/1.08;M1.6/0.30  &\nodata&\nodata&\nodata&M1.8/0.69\\
327  & 20 54 11.22  &$+$44 57 09.8  &Cont  &\nodata&\nodata&\nodata&Cont\\
328  & 20 54 11.62  &$+$44 29 56.0  &M4.2/0;M4.0/0  &\nodata&\nodata&\nodata&M4.1/0\\
329  & 20 54 13.72  &$+$44 24 32.2  &K4.6/0;G7.0/0  &\nodata&G6.0/0&\nodata&K0.8/0\\
330  & 20 54 16.07  &$+$44 24 10.5  &G6.0/0;G6.0/0  &\nodata&\nodata&\nodata&G6.0/0\\
331  & 20 54 17.72  &$+$44 48 40.1  &G6.6/0  &\nodata&\nodata&\nodata&G6.6/0\\
332  & 20 54 20.93  &$+$44 31 57.6  &M2.8/0;M3.0/0  &\nodata&\nodata&\nodata&M2.9/0\\
333  & 20 54 21.13  &$+$44 15 27.1  &6250/0  &6500/0&\nodata&6500/0&6250/0\\
334  & 20 54 21.77  &$+$44 20 51.1  &M2.4/0  &\nodata&\nodata&\nodata&M2.4/0\\
335  & 20 54 22.52  &$+$44 37 17.2  &M1.0/0;M1.0/0  &\nodata&\nodata&\nodata&M1.0/0\\
336  & 20 54 22.84  &$+$44 24 24.9  &M2.4/0;M2.4/0  &\nodata&\nodata&\nodata&M2.4/0\\
337  & 20 54 24.03  &$+$44 34 28.9  &6250/0  &\nodata&\nodata&6000/0&6250/0\\
338  & 20 54 24.41  &$+$44 48 17.6  &K6.2/0.20  &\nodata&K7.0/0.33&\nodata&K6.2/0.20\\
339  & 20 54 24.60  &$+$43 49 56.3  &\nodata  &Cont&\nodata&\nodata&Cont\\
340  & 20 54 26.92  &$+$44 47 53.0  &G6.6/0  &\nodata&\nodata&\nodata&G6.6/0\\
341  & 20 54 27.94  &$+$44 25 03.8  &M4.2/0.14;M4.4/0.36  &\nodata&\nodata&\nodata&M4.3/0.25\\
342  & 20 54 29.55  &$+$44 45 27.0  &K9.4/1.72;M1.4/2.22  &\nodata&\nodata&\nodata&M0.4/1.97\\
343  & 20 54 40.99  &$+$44 21 54.9  &M0.2/0;K9.6/0  &\nodata&\nodata&\nodata&K9.9/0\\
344  & 20 54 45.60  &$+$44 31 37.1  &K7.4/0.16;K7.8/0.14  &\nodata&\nodata&\nodata&K7.6/0.15\\
345  & 20 54 45.66  &$+$44 43 41.9  &M0.4/0  &\nodata&M0.0/0&\nodata&M0.4/0\\
346  & 20 54 46.64  &$+$44 12 06.3  &K8.6/0  &\nodata&\nodata&\nodata&K8.6/0\\
347  & 20 54 46.91  &$+$44 48 19.7  &Cont  &\nodata&\nodata&\nodata&Cont\\
348  & 20 54 51.15  &$+$44 11 34.8  &K8.0/0;K7.8/0  &\nodata&\nodata&\nodata&K7.9/0\\
349  & 20 54 51.24  &$+$44 32 30.6  &K7.6/0.44;K7.0/0.46  &\nodata&\nodata&\nodata&K7.3/0.45\\
350  & 20 54 54.30  &$+$44 43 43.4  &\nodata  &M3.8/0.26&M3.4/1.04&\nodata&M3.8/0.26\\
351  & 20 54 55.16  &$+$44 44 30.9  &K4.6/0.16  &\nodata&\nodata&\nodata&K4.6/0.16\\
352  & 20 54 56.92  &$+$44 39 24.4  &M2.4/0  &M2.0/0&M2.4/0&\nodata&M2.4/0\\
353  & 20 55 03.01  &$+$44 10 52.0  &G6.4/0;G6.4/0  &G6.0/0&\nodata&\nodata&G6.4/0\\
354  & 20 55 03.35  &$+$43 30 38.5  &\nodata  &\nodata&\nodata&M3.8/0&M3.8/0\\
355  & 20 55 04.00  &$+$44 44 26.9  &M3.4/0.54  &M2.8/1.34&\nodata&\nodata&M3.4/0.54\\
356  & 20 55 04.57  &$+$44 35 47.3  &Cont  &\nodata&\nodata&\nodata&Cont\\
357  & 20 55 06.95  &$+$43 57 55.6  &\nodata  &Cont&\nodata&\nodata&Cont\\
358  & 20 55 11.11  &$+$43 57 14.8  &\nodata  &M2.0/0&\nodata&\nodata&M2.0/0\\
359  & 20 55 18.22  &$+$44 19 15.5  &\nodata  &Cont&\nodata&\nodata&Cont\\
360  & 20 55 18.24  &$+$44 30 12.7  &\nodata  &K9.6/0&\nodata&\nodata&K9.6/0\\
361  & 20 55 26.15  &$+$44 07 02.9  &\nodata  &Cont&\nodata&Cont&Cont\\
362  & 20 55 28.10  &$+$43 43 11.2  &7250/0  &\nodata&\nodata&7000/0&7250/0\\
363  & 20 55 28.35  &$+$43 51 46.5  &\nodata  &Cont&\nodata&\nodata&Cont\\
364  & 20 55 29.05  &$+$44 22 25.9  &K6.4/0;G6.0/0  &\nodata&\nodata&\nodata&K1.2/0\\
365  & 20 55 31.88  &$+$44 47 00.6  &Cont  &\nodata&\nodata&\nodata&Cont\\
366  & 20 55 41.29  &$+$44 39 07.0  &Cont  &\nodata&\nodata&\nodata&Cont\\
367  & 20 55 42.50  &$+$44 14 12.8  &K7.8/0  &\nodata&\nodata&\nodata&K7.8/0\\
368  & 20 55 48.13  &$+$43 50 36.6  &Cont  &\nodata&\nodata&\nodata&Cont\\
369  & 20 55 57.10  &$+$44 15 35.8  &K6.6/0.46;K7.0/0.40  &\nodata&\nodata&\nodata&K6.8/0.43\\
370  & 20 56 01.44  &$+$43 35 44.0  &11500/0;9000/0  &\nodata&\nodata&\nodata&K6.8/0.43\\
371  & 20 56 02.06  &$+$43 37 18.2  &Cont  &\nodata&\nodata&\nodata&Cont\\
372  & 20 56 04.85  &$+$44 34 56.4  &M3.8/0.14  &M4.0/0.18&\nodata&\nodata&M3.8/0.14\\
373  & 20 56 08.02  &$+$43 26 52.4  &\nodata  &\nodata&\nodata&M3.6/0&M3.6/0\\
374  & 20 56 11.70  &$+$44 10 55.1  &K3.6/0;G6.6/0  &\nodata&\nodata&\nodata&K0.1/0\\
375  & 20 56 12.65  &$+$43 45 32.0  &5800/0;6000/0  &4800/0&\nodata&\nodata&K0.1/0\\
376  & 20 56 15.30  &$+$44 34 52.5  &\nodata  &M2.2/0&\nodata&\nodata&M2.2/0\\
377  & 20 56 19.61  &$+$43 45 38.7  &K7.0/0  &\nodata&\nodata&\nodata&K7.0/0\\
378  & 20 56 20.10  &$+$44 42 27.7  &M5.2/0.10  &\nodata&\nodata&\nodata&M5.2/0.10\\
379  & 20 56 22.01  &$+$44 35 37.4  &9250/0  &\nodata&\nodata&\nodata&9250/0\\
380  & 20 56 23.96  &$+$43 42 58.3  &\nodata  &M3.8/0&\nodata&M3.8/0&M3.8/0\\
381  & 20 56 24.95  &$+$43 43 28.7  &M3.6/0.10  &M3.6/0.20&\nodata&\nodata&M3.6/0.10\\
382  & 20 56 27.20  &$+$43 45 58.2  &K8.8/0  &K9.0/0&\nodata&\nodata&K8.8/0\\
383  & 20 56 29.50  &$+$43 14 53.6  &\nodata  &\nodata&K7.4/0.25&\nodata&K7.4/0.25\\
384  & 20 56 30.10  &$+$43 51 08.5  &K4.4/0  &\nodata&\nodata&\nodata&K4.4/0\\
385  & 20 56 30.28  &$+$43 55 25.8  &Cont  &\nodata&\nodata&\nodata&Cont\\
386  & 20 56 36.18  &$+$43 21 32.7  &\nodata  &M2.6/0.02&M3.6/0.36&\nodata&M2.6/0.02\\
387  & 20 56 38.88  &$+$43 51 20.5  &M0.4/0.28  &M0.0/0.92&\nodata&\nodata&M0.4/0.28\\
388  & 20 56 40.05  &$+$43 59 45.4  &K9.4/0  &\nodata&\nodata&\nodata&K9.4/0\\
389  & 20 56 44.00  &$+$43 46 00.2  &\nodata  &Cont&\nodata&\nodata&Cont\\
390  & 20 56 46.66  &$+$43 46 01.9  &M4.8/0;M4.6/0  &M4.8/0&\nodata&\nodata&M4.7/0\\
391  & 20 56 46.73  &$+$43 46 08.8  &\nodata  &\nodata&\nodata&M1.6/0&M1.6/0\\
392  & 20 56 51.43  &$+$44 35 32.2  &Cont  &\nodata&\nodata&\nodata&Cont\\
393  & 20 56 51.56  &$+$43 22 49.7  &M2.4/0  &M2.2/0&M2.4/0&\nodata&M2.4/0\\
394  & 20 56 52.19  &$+$44 05 51.6  &K9.6/0.60  &\nodata&M1.0/0.23&\nodata&K9.6/0.60\\
395  & 20 56 59.31  &$+$43 47 52.8  &M4.2/0;M4.2/0  &M4.2/0&M4.0/0&\nodata&M4.2/0\\
396  & 20 57 01.63  &$+$43 41 39.0  &\nodata  &\nodata&M5.2/0&\nodata&M5.2/0\\
397  & 20 57 03.32  &$+$43 41 44.3  &M0.0/0.34;M0.8/0.22  &\nodata&M0.8/0.83&K8.6/0.04&M0.4/0.28\\
398  & 20 57 04.07  &$+$44 37 50.8  &K4.4/0  &\nodata&\nodata&\nodata&K4.4/0\\
399  & 20 57 04.28  &$+$43 44 29.2  &M5.6/0  &M5.4/0&\nodata&M6.0/0&M5.6/0\\
400  & 20 57 07.83  &$+$43 41 55.2  &K9.6/0;K9.4/0  &\nodata&\nodata&\nodata&K9.5/0\\
401  & 20 57 12.47  &$+$43 40 56.2  &M7.0/0.80  &\nodata&\nodata&\nodata&M7.0/0.80\\
402  & 20 57 13.11  &$+$43 54 19.9  &M4.2/0  &\nodata&\nodata&\nodata&M4.2/0\\
403  & 20 57 15.86  &$+$43 58 04.7  &M4.6/0  &\nodata&\nodata&\nodata&M4.6/0\\
404  & 20 57 24.85  &$+$44 19 47.0  &7500/0  &\nodata&\nodata&\nodata&7500/0\\
405  & 20 57 26.68  &$+$43 35 30.3  &K7.0/0.26;K8.0/0.42  &K7.0/1.08&\nodata&\nodata&K7.5/0.34\\
406  & 20 57 31.03  &$+$43 37 32.8  &6250/0  &\nodata&\nodata&\nodata&6250/0\\
407  & 20 57 33.77  &$+$44 05 13.4  &\nodata  &M4.6/0&\nodata&\nodata&M4.6/0\\
408  & 20 57 34.52  &$+$43 59 54.7  &Cont  &\nodata&\nodata&\nodata&Cont\\
409  & 20 57 37.29  &$+$44 06 44.0  &\nodata  &Cont&Cont&Cont&Cont\\
410  & 20 57 38.38  &$+$44 06 58.9  &Cont  &\nodata&\nodata&\nodata&Cont\\
411  & 20 57 41.80  &$+$43 49 53.3  &M5.4/0  &M5.4/0&\nodata&\nodata&M5.4/0\\
412  & 20 57 46.54  &$+$44 07 11.7  &M5.8/0.16  &\nodata&\nodata&\nodata&M5.8/0.16\\
413  & 20 57 48.50  &$+$43 29 42.7  &M0.8/0  &\nodata&\nodata&\nodata&M0.8/0\\
414  & 20 57 48.81  &$+$44 05 25.9  &\nodata  &\nodata&\nodata&K7.2/0&K7.2/0\\
415  & 20 57 50.00  &$+$44 08 08.4  &M2.0/0  &\nodata&M1.8/0&M2.2/0&M2.0/0\\
416  & 20 57 55.42  &$+$44 05 25.0  &M5.8/0  &M5.8/0&M5.8/0&\nodata&M5.8/0\\
417  & 20 57 59.85  &$+$43 53 26.6  &K7.8/0.80  &\nodata&\nodata&K6.4/0.60&K7.8/0.80\\
418  & 20 58 01.36  &$+$43 45 20.6  &K6.6/1.14;K7.8/2.42  &\nodata&K7.4/1.22&\nodata&K7.2/1.78\\
419  & 20 58 06.04  &$+$43 49 32.8  &M1.0/0  &M0.4/0&M1.8/0&\nodata&M1.0/0\\
420  & 20 58 06.10  &$+$43 53 01.4  &M1.6/0;M1.6/0  &\nodata&\nodata&M1.6/0;M1.6/0;M2.0/0&M1.6/0\\
421  & 20 58 07.64  &$+$43 52 52.7  &\nodata  &M2.4/0.70&\nodata&\nodata&M2.4/0.70\\
422  & 20 58 08.43  &$+$43 39 00.3  &M5.2/0  &\nodata&\nodata&\nodata&M5.2/0\\
423  & 20 58 08.86  &$+$43 46 59.9  &K9.2/0  &\nodata&K8.8/0&\nodata&K9.2/0\\
424  & 20 58 09.53  &$+$44 11 02.8  &M4.4/0.10  &M4.6/0.02&\nodata&\nodata&M4.4/0.10\\
425  & 20 58 09.99  &$+$43 45 36.1  &M3.8/0.74;M4.0/0.36  &M3.6/0.62&M4.0/0.46&\nodata&M3.9/0.55\\
426  & 20 58 10.82  &$+$43 53 08.2  &K9.2/0  &\nodata&\nodata&K8.6/0&K9.2/0\\
427  & 20 58 11.38  &$+$43 52 57.0  &M4.6/0.90  &\nodata&\nodata&M5.0/1.02&M4.6/0.90\\
428  & 20 58 12.33  &$+$44 20 58.2  &M0.8/0.18  &\nodata&\nodata&\nodata&M0.8/0.18\\
429  & 20 58 14.27  &$+$43 53 04.6  &M5.8/0  &\nodata&\nodata&\nodata&M5.8/0\\
430  & 20 58 17.90  &$+$43 53 44.1  &\nodata  &\nodata&\nodata&Cont&Cont\\
431  & 20 58 18.19  &$+$43 26 13.5  &K5.8/0.56  &\nodata&\nodata&K4.0/0.56&K5.8/0.56\\
432  & 20 58 19.61  &$+$43 53 54.5  &G6.0/0;G6.0/0  &\nodata&\nodata&G6.0/0&G6.0/0\\
433  & 20 58 21.54  &$+$43 53 44.9  &\nodata  &\nodata&\nodata&Cont&Cont\\
434  & 20 58 23.71  &$+$43 52 56.3  &\nodata  &M0.4/0&\nodata&\nodata&M0.4/0\\
435  & 20 58 23.81  &$+$43 53 11.4  &5600/0  &\nodata&\nodata&\nodata&5600/0\\
436  & 20 58 23.99  &$+$43 53 54.6  &K9.2/0.10  &\nodata&\nodata&M0.4/0.14&K9.2/0.10\\
437  & 20 58 25.55  &$+$43 53 28.6  &M3.0/0.46  &\nodata&M3.2/0.76&M2.0/0.02&M3.0/0.46\\
438  & 20 58 26.90  &$+$44 18 06.3  &M5.4/0.26  &\nodata&\nodata&\nodata&M5.4/0.26\\
439  & 20 58 27.02  &$+$43 53 20.1  &\nodata  &Cont&\nodata&\nodata&Cont\\
440  & 20 58 27.25  &$+$43 54 55.8  &M5.8/0  &\nodata&\nodata&\nodata&M5.8/0\\
441  & 20 58 29.09  &$+$44 10 50.5  &\nodata  &M4.2/0&\nodata&\nodata&M4.2/0\\
442  & 20 58 29.41  &$+$43 55 12.5  &M5.6/1.12  &\nodata&\nodata&\nodata&M5.6/1.12\\
443  & 20 58 30.41  &$+$43 53 59.2  &\nodata  &M3.2/0&M3.2/0&\nodata&M3.2/0\\
444  & 20 58 30.47  &$+$43 54 09.6  &M2.6/0  &\nodata&M2.4/0&M2.6/0&M2.6/0\\
445  & 20 58 30.94  &$+$43 45 11.2  &\nodata  &M2.6/0&\nodata&\nodata&M2.6/0\\
446  & 20 58 33.59  &$+$44 03 35.5  &M2.4/0.44  &\nodata&\nodata&\nodata&M2.4/0.44\\
447  & 20 58 35.67  &$+$44 18 44.8  &M3.4/0  &\nodata&\nodata&\nodata&M3.4/0\\
448  & 20 58 39.58  &$+$44 18 28.0  &M3.6/0.34  &\nodata&\nodata&\nodata&M3.6/0.34\\
449  & 20 58 39.65  &$+$43 43 09.1  &\nodata  &\nodata&\nodata&K4.4/0&K4.4/0\\
450  & 20 58 39.74  &$+$44 01 32.8  &K4.6/1.20  &\nodata&\nodata&\nodata&K4.6/1.20\\
451  & 20 58 41.97  &$+$44 16 25.6  &M4.0/0  &\nodata&\nodata&\nodata&M4.0/0\\
452  & 20 58 43.13  &$+$43 46 00.1  &M6.2/0  &\nodata&\nodata&\nodata&M6.2/0\\
453  & 20 58 47.40  &$+$44 01 34.8  &M5.0/0  &M5.0/0&M4.8/0&\nodata&M5.0/0\\
454  & 20 58 53.22  &$+$43 58 32.9  &M4.8/0  &M4.8/0&M4.2/0&\nodata&M4.8/0\\
455  & 20 59 03.47  &$+$44 13 11.6  &M4.8/0  &\nodata&\nodata&\nodata&M4.8/0\\
456  & 20 59 05.82  &$+$43 57 03.2  &5300/0  &5300/0&\nodata&\nodata&5300/0\\
457  & 20 59 06.70  &$+$44 18 23.7  &K9.6/0.26  &\nodata&\nodata&\nodata&K9.6/0.26\\
458  & 20 59 14.86  &$+$44 12 28.5  &Cont  &\nodata&\nodata&\nodata&Cont\\
459  & 20 59 20.20  &$+$44 17 05.1  &M1.6/0  &\nodata&\nodata&\nodata&M1.6/0\\
460  & 20 59 29.57  &$+$44 10 47.7  &M0.6/0  &\nodata&\nodata&\nodata&M0.6/0\\
461  & 20 59 29.74  &$+$44 17 04.2  &M0.0/0.60  &\nodata&\nodata&\nodata&M0.0/0.60\\
462  & 20 59 32.69  &$+$44 08 35.5  &M2.0/0  &\nodata&\nodata&\nodata&M2.0/0\\
463  & 20 59 38.29  &$+$44 10 07.2  &M4.2/0.10  &\nodata&\nodata&\nodata&M4.2/0.10\\
464  & 20 50 53.80  &$+$44 21 18.5  &M3.2/0.52  &M2.8/0.38&\nodata&\nodata&M3.2/0.52\\
465  & 20 53 00.65  &$+$44 36 59.5  &5800/0  &\nodata&\nodata&5600/0&5800/0\\
466  & 20 53 17.47  &$+$44 28 03.1  &K8.2/0;K8.6/0  &\nodata&\nodata&\nodata&K8.4/0\\
467  & 20 53 37.85  &$+$44 24 20.9  &K7.8/0  &\nodata&\nodata&\nodata&K7.8/0\\
468  & 20 55 43.25  &$+$44 03 12.5  &K9.4/0  &\nodata&\nodata&\nodata&K9.4/0\\
469  & 20 54 27.90  &$+$44 00 09.8  &M3.6/0  &\nodata&\nodata&\nodata&M3.6/0\\
470  & 20 52 46.12  &$+$44 10 42.5  &Cont  &\nodata&\nodata&\nodata&Cont\\
471  & 20 52 39.86  &$+$44 05 48.2  &M3.4/0.12  &\nodata&\nodata&\nodata&M3.4/0.12\\
472  & 20 51 05.45  &$+$44 13 59.3  &M4.8/0.08  &M4.8/0.06&\nodata&\nodata&M4.8/0.08\\
473  & 20 52 56.68  &$+$44 29 48.4  &Cont  &\nodata&\nodata&\nodata&Cont\\
474  & 20 51 47.93  &$+$44 38 40.8  &M3.8/0  &\nodata&\nodata&\nodata&M3.8/0\\
475  & 20 52 46.08  &$+$44 39 09.9  &M2.6/0;M2.6/0  &\nodata&\nodata&\nodata&M2.6/0\\
476  & 20 53 08.17  &$+$44 05 14.3  &M3.6/0.44;M3.8/0.28  &M3.2/0.54&M3.2/0.22&\nodata&M3.7/0.36\\
477  & 20 52 14.74  &$+$43 59 47.3  &M6.2/0  &\nodata&\nodata&\nodata&M6.2/0\\
478  & 20 52 51.38  &$+$44 20 35.7  &Cont  &\nodata&\nodata&\nodata&Cont\\
479  & 20 52 41.58  &$+$44 19 27.2  &M4.2/0  &\nodata&\nodata&\nodata&M4.2/0\\
480  & 20 59 19.65  &$+$43 46 00.4  &M7.0/0  &\nodata&\nodata&\nodata&M7.0/0\\
481  & 20 56 39.90  &$+$43 59 45.4  &Cont  &\nodata&\nodata&\nodata&Cont\\
482  & 20 58 19.48  &$+$43 53 44.9  &M1.8/0  &\nodata&\nodata&\nodata&M1.8/0\\
483  & 20 53 34.63  &$+$44 28 51.3  &M2.0/0  &\nodata&\nodata&\nodata&M2.0/0\\
484  & 20 53 58.29  &$+$44 10 21.1  &K4.2/0  &\nodata&\nodata&\nodata&K4.2/0\\
485  & 20 53 35.58  &$+$44 17 43.2  &M2.0/0  &\nodata&\nodata&\nodata&M2.0/0\\
486  & 20 53 55.56  &$+$44 11 06.0  &K9.2/0  &\nodata&\nodata&\nodata&K9.2/0\\
487  & 20 54 05.00  &$+$44 10 24.6  &K7.4/0  &\nodata&\nodata&\nodata&K7.4/0\\
488  & 20 54 06.29  &$+$44 30 24.7  &K6.4/0  &\nodata&\nodata&\nodata&K6.4/0\\
489  & 20 53 54.54  &$+$44 32 28.5  &6500/0  &\nodata&\nodata&\nodata&6500/0\\
490  & 20 53 33.32  &$+$44 25 18.6  &K8.2/0  &\nodata&\nodata&\nodata&K8.2/0\\
491  & 20 53 45.79  &$+$44 28 16.7  &M3.2/0  &\nodata&\nodata&\nodata&M3.2/0\\
492  & 20 53 46.44  &$+$44 27 04.6  &M1.0/0  &\nodata&\nodata&\nodata&M1.0/0\\
493  & 20 53 40.08  &$+$44 25 50.1  &G6.8/0  &\nodata&\nodata&\nodata&G6.8/0\\
494  & 20 53 41.37  &$+$44 24 36.2  &M1.8/0  &\nodata&\nodata&\nodata&M1.8/0\\
495  & 20 54 31.96  &$+$44 20 15.7  &8500/0  &\nodata&\nodata&\nodata&8500/0\\
496  & 20 54 49.16  &$+$44 20 14.6  &K6.8/0  &\nodata&\nodata&\nodata&K6.8/0\\
497  & 20 53 43.61  &$+$44 15 08.6  &K9.8/0  &\nodata&\nodata&\nodata&K9.8/0\\
498  & 20 55 01.18  &$+$44 06 45.8  &8000/0  &\nodata&\nodata&\nodata&8000/0\\
499  & 20 53 58.87  &$+$44 09 41.5  &M0.8/0  &\nodata&\nodata&\nodata&M0.8/0\\
500  & 20 52 26.30  &$+$44 03 26.5  &M2.0/0  &\nodata&\nodata&\nodata&M2.0/0\\
501  & 20 50 48.60  &$+$44 17 03.4  &M3.8/0.70  &\nodata&\nodata&\nodata&M3.8/0.70\\
502  & 20 50 57.49  &$+$44 24 45.4  &K8.6/0.28  &K6.4/0.46&\nodata&\nodata&K8.6/0.28\\
503  & 20 50 37.38  &$+$44 20 53.0  &M1.8/0.10  &\nodata&\nodata&\nodata&M1.8/0.10\\
504  & 20 51 06.63  &$+$44 21 40.7  &Cont  &\nodata&\nodata&\nodata&Cont\\
505  & 20 52 08.95  &$+$44 21 54.6  &M0.6/0  &\nodata&\nodata&\nodata&M0.6/0\\
506  & 20 52 33.58  &$+$44 20 45.9  &M5.4/0.40  &\nodata&\nodata&\nodata&M5.4/0.40\\
507  & 20 52 06.72  &$+$44 29 23.6  &K9.8/0  &\nodata&\nodata&\nodata&K9.8/0\\
508  & 20 52 32.66  &$+$44 26 32.2  &K6.0/0  &\nodata&\nodata&\nodata&K6.0/0\\
509  & 20 52 26.79  &$+$44 37 06.6  &5700/0  &\nodata&\nodata&\nodata&5700/0\\
510  & 20 52 33.95  &$+$44 29 16.8  &K6.4/0  &\nodata&\nodata&\nodata&K6.4/0\\
511  & 20 52 29.41  &$+$44 38 40.4  &K8.4/0  &\nodata&\nodata&\nodata&K8.4/0\\
512  & 20 52 45.03  &$+$44 35 23.7  &K4.4/0  &\nodata&\nodata&\nodata&K4.4/0\\
513  & 20 53 29.92  &$+$44 39 35.1  &M2.6/0  &\nodata&\nodata&\nodata&M2.6/0\\
514  & 20 53 12.22  &$+$44 26 34.9  &M1.8/0  &\nodata&\nodata&\nodata&M1.8/0\\
515  & 20 53 40.53  &$+$44 37 27.3  &6000/0  &\nodata&\nodata&\nodata&6000/0\\
516  & 20 50 55.44  &$+$44 17 45.9  &M2.0/0  &\nodata&\nodata&\nodata&M2.0/0\\
517  & 20 52 05.51  &$+$44 23 37.0  &Cont  &\nodata&\nodata&\nodata&Cont\\
518  & 20 50 59.66  &$+$44 30 15.3  &K8.4/0  &\nodata&\nodata&\nodata&K8.4/0\\
519  & 20 52 24.97  &$+$44 28 15.4  &M2.6/0  &\nodata&\nodata&\nodata&M2.6/0\\
520  & 20 53 02.09  &$+$44 46 14.3  &M2.2/0  &\nodata&\nodata&\nodata&M2.2/0\\
521  & 20 51 47.79  &$+$43 42 38.9  &K6.6/0  &\nodata&\nodata&\nodata&K6.6/0\\
522  & 20 50 54.47  &$+$43 46 23.8  &K8.2/0  &\nodata&\nodata&\nodata&K8.2/0\\
523  & 20 48 57.79  &$+$43 49 55.1  &M4.8/2.50  &\nodata&\nodata&\nodata&M4.8/2.50\\
524  & 20 48 51.69  &$+$43 51 01.4  &K9.0/0  &\nodata&\nodata&\nodata&K9.0/0\\
525  & 20 48 35.46  &$+$43 53 13.4  &K9.6/0.38  &\nodata&\nodata&\nodata&K9.6/0.38\\
526  & 20 48 32.87  &$+$44 11 59.6  &M3.6/0.26  &\nodata&\nodata&\nodata&M3.6/0.26\\
527  & 20 48 33.96  &$+$44 22 28.7  &G6.6/0  &\nodata&\nodata&\nodata&G6.6/0\\
528  & 20 50 06.17  &$+$44 25 05.0  &M4.6/0  &\nodata&\nodata&\nodata&M4.6/0\\
529  & 20 50 44.96  &$+$44 20 58.9  &M3.6/0.42  &\nodata&\nodata&\nodata&M3.6/0.42\\
530  & 20 50 37.95  &$+$44 25 12.4  &K9.0/0  &\nodata&\nodata&\nodata&K9.0/0\\
531  & 20 50 56.70  &$+$44 17 05.4  &M2.8/0  &\nodata&\nodata&\nodata&M2.8/0\\
532  & 20 50 54.86  &$+$44 20 12.5  &M4.0/0.16  &\nodata&\nodata&\nodata&M4.0/0.16\\
533  & 20 50 48.53  &$+$44 33 33.2  &M2.4/0.62  &\nodata&\nodata&\nodata&M2.4/0.62\\
534  & 20 51 12.44  &$+$44 19 43.0  &M4.8/0  &\nodata&\nodata&\nodata&M4.8/0\\
535  & 20 51 20.59  &$+$44 20 32.2  &M3.2/0  &\nodata&\nodata&\nodata&M3.2/0\\
536  & 20 51 12.62  &$+$44 18 45.4  &5300/0  &\nodata&\nodata&\nodata&5300/0\\
537  & 20 52 34.38  &$+$44 26 05.2  &M0.6/0  &\nodata&\nodata&\nodata&M0.6/0\\
538  & 20 52 51.93  &$+$44 28 13.7  &K8.2/0  &\nodata&\nodata&\nodata&K8.2/0\\
539  & 20 52 22.91  &$+$44 22 25.3  &M0.8/0  &\nodata&\nodata&\nodata&M0.8/0\\
540  & 20 53 27.53  &$+$44 06 09.3  &6250/0  &\nodata&\nodata&\nodata&6250/0\\
541  & 20 51 13.74  &$+$44 22 25.2  &M5.4/0  &\nodata&\nodata&\nodata&M5.4/0\\
542  & 20 51 05.91  &$+$44 23 47.1  &M3.6/0.20  &\nodata&\nodata&\nodata&M3.6/0.20\\
543  & 20 52 31.70  &$+$44 29 59.1  &M2.6/0  &\nodata&\nodata&\nodata&M2.6/0\\
544  & 20 54 34.54  &$+$44 33 08.8  &K9.0/0  &\nodata&\nodata&\nodata&K9.0/0\\
545  & 20 55 49.40  &$+$44 34 10.2  &5100/0  &\nodata&\nodata&\nodata&5100/0\\
546  & 20 55 28.51  &$+$44 43 45.0  &M1.8/0  &\nodata&\nodata&\nodata&M1.8/0\\
547  & 20 55 19.40  &$+$44 41 09.6  &M3.0/0  &\nodata&\nodata&\nodata&M3.0/0\\
548  & 20 54 57.36  &$+$44 38 43.6  &K6.6/0  &\nodata&\nodata&\nodata&K6.6/0\\
549  & 20 54 44.66  &$+$44 31 44.2  &5700/0  &\nodata&\nodata&\nodata&5700/0\\
550  & 20 54 45.82  &$+$44 35 48.0  &M2.4/0  &\nodata&\nodata&\nodata&M2.4/0\\
551  & 20 54 06.49  &$+$44 30 24.0  &K7.4/0  &\nodata&\nodata&\nodata&K7.4/0\\
552  & 20 53 57.79  &$+$44 29 43.0  &5300/0  &\nodata&\nodata&\nodata&5300/0\\
553  & 20 53 25.47  &$+$44 27 16.4  &M0.4/0  &\nodata&\nodata&\nodata&M0.4/0\\
554  & 20 53 08.30  &$+$44 50 05.0  &M1.8/0  &\nodata&\nodata&\nodata&M1.8/0\\
555  & 20 53 23.81  &$+$45 06 47.8  &K4.2/0  &\nodata&\nodata&\nodata&K4.2/0\\
556  & 20 59 25.87  &$+$44 14 21.6  &M1.0/0  &\nodata&\nodata&\nodata&M1.0/0\\
557  & 20 59 57.74  &$+$44 47 12.6  &K3.2/0  &\nodata&\nodata&\nodata&K3.2/0\\
558  & 20 53 42.14  &$+$44 26 53.7  &K9.4/0  &\nodata&\nodata&\nodata&K9.4/0\\
559  & 21 00 03.30  &$+$43 04 27.9  &M1.0/0  &\nodata&\nodata&\nodata&M1.0/0\\
560  & 21 01 17.98  &$+$43 40 06.2  &Cont  &\nodata&\nodata&\nodata&Cont\\
561  & 21 01 04.96  &$+$43 19 43.7  &Cont  &\nodata&\nodata&\nodata&Cont\\
\enddata
\end{deluxetable*}


==> cluster.tex <==
\begin{table*}
\renewcommand{\tabcolsep}{0.1cm}

\caption{Luminosity spreads within different temperature bins }\label{Table:Lumspread}
%\tiny
\begin{center}
\begin{tabular}{cccccccccccccccccc}
\hline
&  &\multicolumn{2}{c}{4000$-$5000~K} & & \multicolumn{2}{c}{3000$-$4000~K} & \\
\cline{3-4} \cline{6-7} 
Regions & Age &$\sigma$Log~$L_{\star}/L_{\odot}$ & N  & &$\sigma$Log~$L_{\star}/L_{\odot}$ & N  & References \\
\hline
Trapezium &1~Myr  &0.32  &40 & &0.35 &197 &1 \\
Taurus &1.5~Myr   &0.38  &20 & &0.33 &127 &2 \\
%Taurus &1.5~Myr   &0.58  &13 & &0.29 &36 & &0.34 &65 &2 \\
MGC2068/2071 &1.5~Myr  &0.34  &23 & &0.33 &105  &3 \\
Cha~I &2~Myr  &0.31  &18 & &0.26 &153  &4 \\
IC~348 &2.5~Myr  &0.24  &20 & &0.29 &203  &5 \\
NGC~2264 &3~Myr  &0.20  &181 & &0.25 &298  &6 \\
%$\sigma$~Ori &3~Myr  &0.32  &9 & &0.17 &45 & &0.25 &49 &7 \\
$\sigma$~Ori &3~Myr  &0.24   &20    & &0.24 &122  &7 \\
NGC~2362 &5~Myr  &0.15  &27 & &0.17 &62  &8 \\
Upper~Sco &11~Myr  &0.21  &65 & &0.23 &562  &9 \\
Ori~1b    &5~Myr   &0.23  &63 & &0.30 &412  &10\\
%25~Ori    &7.6~Myr  &0.12  &12 & &0.18 &25 & &0.28 &82 &10\\
25~Ori    &7.6~Myr  &0.12     &16  & &0.22 &172  &10\\
%HD~35762  &8~Myr  &0.13  &4 & &0.31 &15 & &0.26 &35 &10\\
HD~35762  &8~Myr  &    &   & &0.24 &74  &10\\
Ori~1a    &10.8~Myr   &0.20  &68 & &0.30 &653 &10\\
%HR~1833  &12.9~Myr  &0.11  &5 & &0.24 &8 & &0.28 &33 &10\\
HR~1833  &12.9~Myr  &    &   & &0.29  &54   &10\\
\hline
%\diagbox{a}{b}      &3.1, constant  & 3.1, BB7000 &5.5, constant & 5.5, BB7000  \\
%        \hline
% & \multicolumn{4}{c}{The sources in this work}\\
%\hline
%3.1, constant&0   &$-$0.067 dex  & $-$0.110 dex  &$-$0.204 dex    \\  
%\hline
%3.1, BB7000&    & 0 &$-$0.030 dex   &$-$0.127 dex  \\  
%\hline
%5.5, constant&    &   & 0 &$-$0.077 dex   \\ 
%\hline
%5.5, BB7000&    &   &   &0    \\  
%  \hline
% & \multicolumn{4}{c}{The sources in this work and in \cite{2016ApJ...831..169S}}\\
%\hline
%Full disks&24\% (9/38) &39\% (15/38)&29\% (11/38)&63\% (24/38)    %\\  
%TDs &40\% (8/20)       &45\% (8/20) &15\% (3/20) &10\% (2/20)    %\\  
%\hline
\end{tabular}
\end{center}
References--1. This work, 2. \cite{2014ApJ...786...97H}, 2.\cite{2009A&A...497..117A}, \cite{2014ApJ...794...36H}, 4. \cite{2007ApJS..173..104L}, 5. \cite{2003ApJ...593.1093L}, 6. \cite{2018A&A...609A..10V}, 7. \cite{2014ApJ...794...36H}, 8. \cite{2005AJ....130.1805D}, 9. \cite{2018AJ....156...76L}, 10. \cite{2019AJ....157...85B}
\end{table*}
\normalsize


==> model.tex <==
\begin{table}
\caption{Stellar parameters derived from simulated observations \label{tabe-model}}
 \centering
\begin{tabular}{lcccccccccc}
\hline\hline
  &\multicolumn{2}{c}{Simulated observations} & & \multicolumn{2}{c}{Derived parameters}\\
  &\cline{1-2} \cline{4-5}
\hline
\multicolumn{1}{c}{Case} & \multicolumn{1}{c}{Photometry}&\multicolumn{1}{c}{Spectra} & &\multicolumn{1}{c}{Without Veiling}&\multicolumn{1}{c}{With veiling} \\ 
\hline
1 &$r_{7465}=1.6$ &$r_{7465}=0.1$ &$A_{\rm V}$=   & \\
  &               &               &$T_{\rm eff}$= & \\
  &               &               &$L_{\star}$= & \\
\hline
2 &$r_{7465}=0.1$ &$r_{7465}=0.1$ &$A_{\rm V}$=   & \\
  &               &               &$T_{\rm eff}$= & \\
  &               &               &$L_{\star}$= & \\
\hline
\hline
3 &$r_{7465}=0.1$ &$r_{7465}=0.1$ &$A_{\rm V}$=   & \\
  &               &               &$T_{\rm eff}$= & \\
  &               &               &$L_{\star}$= & \\
\hline
\hline
4 &$r_{7465}=0.1$ &$r_{7465}=0.1$ &$A_{\rm V}$=   & \\
  &               &               &$T_{\rm eff}$= & \\
  &               &               &$L_{\star}$= & \\
\hline
\end{tabular}
\end{table}


==> source.tex <==
%\renewcommand{\tabcolsep}{0.02cm}
%\longtab{2}{
%\begin{landscape}
\clearpage
%\begin{longtable}{cccccccccccccccccccccc}
\begin{table*}
\scriptsize
\renewcommand{\tabcolsep}{0.03cm}
\begin{center}
\caption{The parameters for WTTSs \label{Tab:source_Xshooter}}
\begin{tabular}{ccccc|c|c|c|c|c|ccc} 
\hline \hline
    &      &RA      &DEC     & &Pecaut$^{a}$  &Manara$^{b}$  &Luhman$^{c}$      & Others  &       &This work         \\
ID  & Name &(J2000) &(J2000) &Region    & Spt               &Spt     &Spt                         &Spt    & Ref  &Spt \\  
\hline
 %\multicolumn{9}{c}{$\eta$~Cha}\\
%\hline
1 & RECX\,1 &08 36 56.24  &$-$78 56 45.7  &$\eta$~Cha & K5             &           &K6        &K4, K4, K7, K6 &1, 2, 3  &K5 \\


2 & RECX\,3 &08 41 37.03  &$-$79 03 30.4&$\eta$~Cha  & M3.5          &           &M3.25     &M3, M3      &2, 3     &M3.25   \\
3 & RECX\,4 &08 42 23.77  &$-$79 04 03.0&$\eta$~Cha  & M0              &            &M1.75    &K7, M1.5    &2, 3     &M1.75    \\
4 & RECX\,6 &08 42 38.77 &$-$78 54 42.8&$\eta$~Cha  &M3                  &           &M3        &M2, M3       &2, 3     &M3.0  \\
%5 & RECX\,7 &08 43 07.24  &$-$79 04 52.5  & K5              &            &K6       &K4, K3, K7   &1, 2, 3   &K4  \\
5 & RECX\,10&08 44 31.90  &$-$78 46 31.2&$\eta$~Cha   & K9              &            &M1       &K7/M0, K7, M0.5 &1, 2, 3  &M0.5    \\
6 & RECX\,12&08 47 56.77  &$-$78 54 53.2&$\eta$~Cha   &M3.25                 &            &M3.25    &M2, M2, M3  &1, 2, 3     &M3.25    \\
7 &J0836    &08 36 10.73  &$-$79 08 18.4&$\eta$~Cha   &M5.5                 &            &M5.5     &M5.5, M5.5   &3, 4       &M5.5    \\
8 &J0838    &08 38 51.50  &$-$79 16 13.7&$\eta$~Cha   &M5.25                  &          &M5.25    &M5, M5       &3, 4       & M5.25   \\
%\hline
%\multicolumn{9}{c}{TW~Hya Association}\\
%\hline
9 &TWA\,2A&11 09 13.80  &$-$30 01 39.9 &TWA    &M1.5         &M2    &M2.25  &M0.5, M2, M1.5, M2.2 &5, 6, 7, 28     &M2.25 \\
10 &TWA\,3B &11 10 27.81 &$-$37 31 53.2 &TWA&M4       &      &     &   & &M4.0    \\
11 &TWA\,6 &10 18 28.70 &$-$31 50 02.9&TWA    &M0            &K7    &M0.0     &K7, M0,    M0.0    &5, 6, 28           &K7.0   & \\
12 &TWA\,7 &10 42 30.06 &$-$33 40 16.6&TWA    &M3          &M3    &M3.25     &M1, M2, M3.2       &5, 6, 28           & M3.25\\
13 &TWA\,8A &            &       &TWA&M3       &      &     &   & &M3.0    \\
14 &TWA\,8B &            &       &TWA&M5.5       &      &     &   & &M5.25    \\
15 &TWA\,9A&11 48 24.22 &$-$37 28 49.2&TWA    &K7            &K5    &     &K5, K5, K7, K6           &5, 6, 8, 28        &K7.0  \\
16 &TWA\,9B&11 48 23.73  &$-$37 28 48.5&TWA    &M3.5         &M3    &     &M1, M3.5, M3.4           &5, 8, 28         &M3.5 \\
%15 &TWA\,13A&11 21 17.24 &$-$34 46 45.5   &        &M1.1     &M1    &M1     &M2, M1           &9, 6          & M2 \\
%16 &TWA\,13B&11 21 17.24 &$-$34 46 45.5   &        &M1.0     &M1    &     &M1, M1                &9, 6          &M1.75 \\
17 &TWA\,14 &11 13 26.22 &$-$45 23 42.7&TWA    &K8            &M0.5  &     &M0, M0.6, K8, M1.9       &7, 10, 28      &M0.5  \\
18 &TWA\,15A&12 34 20.65 &$-$48 15 13.5&TWA   &               &M3.5  &     &M1.5                &10              &M3.25 \\
19 &TWA\,15B&12 34 20.47  &$-$48 15 19.5&TWA   &                 &M3    &     &M2.2, M2            &7, 10           &M3.25\\
20 &TWA\,25 &12 15 30.72  &$-$39 48 42.6&TWA   &K9       &M0    &M0.75     &M0, M1, M0.5            &11, 6, 28      &M0.5 \\
21 &TWA\,26 &11 39 51.14 &$-$31 59 21.5 &TWA  &M8             &M9    &M8.5      &M8, M8, M9           &12, 13, 14       &M8.5   & \\
22 &TWA\,29 &12 45 14.16  & $-$44 29 07.7&TWA   &M9.5         &M9.5  &M9.25  &M9.5                  &13            &M9.5 \\
%\hline
%\multicolumn{9}{c}{Lupus}\\
%\hline
23 &Sz~94  &16 07 49.60 &$-$39 04 28.8 &Lupus   &            &M4    &     &M4                &15           &M3.5 \\
24 &Sz~107 &16 08 41.80 &$-$39 01 37.0 & Lupus   &            &M5.5  &      &M5.5              &15           &M5.5    \\
25 &Sz\,121&16 10 12.20 &$-$39 21 18.1 & Lupus   &             &M4    &      &M3                &15           &M4.0  \\
26 &Sz\,122&16 10 16.42  &$-$39 08 05.1 & Lupus   &             &M2      &     &M2              &15           & M2.25 \\
27 &Par-Lup3-1 &16 08 16.03 &$-$39 03 04.3 & Lupus  &            &M6.5      &     &M7.5, M6.25    &16, 17          &M6.5 \\
28 &Par-Lup3-2 &16 08 35.78 &$-$39 03 47.9 & Lupus  &          &M5      &     &M6                &16           &M5.0\\
29 &RXJ1526.0-4501 &15 25 59.65 &$-$45 01 15.7 &Lupus  &K0     &G9      &     &G7, G8, G5        &6, 18, 20         &K0.0   \\
30 &RXJ1508.6-4423 &15 08 37.74 &$-$44 23 17.0&Lupus  &G6     &G8      &     &G8, G1.5, G8,      &6, 18, 20            &G6 \\
31 &RXJ1515.8-3331 &15 15 45.36 &$-$33 31 59.8&Lupus  &K0       &K0.5      &   &K0, K0, K1             &6, 19, 20         &K0.0    \\
32 &RXJ1547.7-4018 &15 47 41.76 &$-$40 18 26.8&Lupus  &K1        &K3      &     &K1, K1              &6, 20          &K1.0    \\
33 &RXJ1538.6-3916 &15 38 38.36 &$-$39 16 54.1&Lupus  &K4       &K4      &     &K4                   &20           &K4.0    \\
34 &RXJ1540.7-3756 &15 40 41.17 &$-$37 56 18.5&Lupus  &K6       &K6      &     &K6                   &20           &K6.0    \\
35 &RXJ1543.1-3920 &15 43 06.25 &$-$39 20 19.5&Lupus  &       &K6      &     &K6                   &20           &K6.0    \\
%\hline
%\multicolumn{10}{c}{$\sigma$~Ori}\\
%\hline
36 &SO~879 &05 39 05.42  &$-$02 32 30.3 &$\sigma$~Ori &          &K7      &    &K7, K6.5               &21, 24          &K7.0   \\
37 &SO~925 &05 39 11.41  &$-$02 33 32.8 &$\sigma$~Ori  &              &M5.5    &     &M5, M5.5             &22, 23          &M5.5 \\
38 &SO~999 &05 39 20.25  &$-$02 38 25.8&$\sigma$~Ori  &               &M5.5    &     &M5.5, M4              &23, 24          &M5.25\\
39 &SO~797 &05 38 54.92  &$-$02 28 58.4&$\sigma$~Ori &               &M4.5    &     &M4.5                   &23           &M4.75 \\
40 &SO~641 &05 38 38.58  &$-$02 41 55.9&$\sigma$~Ori  &               &M5    &     &M5, M5.5              &23, 27          &M5.25 \\
%\hline
%\multicolumn{10}{c}{Taurus}\\
%\hline
%41 &RXJ0445.8+1556  &04 45 51.29 &+15 55 49.7 &      &         &G5    &G5     &G3      &25           &G4   & \\
41 &RXJ0438.6+1546  &04 38 39.07 &+15 46 13.6 & Taurus &              &K2    &K1     &G6      &25           &K2.0   & \\
%43 &RXJ0457.5+2014  &04 57 30.66 &+20 14 29.4 &      &         &K1    &       &K3      &25           &K0.5   & \\
%\hline
%\multicolumn{10}{c}{Upper~Sco}\\
%\hline
42 &PZ99J160550.5-253313 &16 05 50.64 &$-$25 33 13.6 &Upper~Sco &G7           &K1        &     &K1, G7              &6, 26          &G7.0    \\
43 &PZ99J160843.4-260216 &16 08 43.41 &$-$26 02 16.8 &Upper~Sco &G7           &K0.5      &     &G9, G7               &6, 26          &G7.0    \\
%\hline
%\multicolumn{10}{c}{Cha~I}\\
%\hline
44 &LM717   &11 08 02.34 &$-$76 40 34.3 &Cha~I &         &M6.5      &M6     &                     &           &M6.5 \\
%47 &LM601   &11 12 30.99 &$-$76 53 34.2 &      &   &M7.5       &M7     &                     &           &   & \\
45 &J11195652-7504529 &11 19 56.52 & $-$75 04 52.9 &Cha~I &    &M7   &M7.25  &                     &           &M6.5   \\
%49 &CHSM17173 &11 10 22.26 &$-$76 25 13.8      &  &    &M8     &M8     &                     &           &   & \\
\hline
\end{tabular}
\end{center}
$^{a}$ Spectral types are from \citet{2013ApJS..208....9P} and \citet{2016MNRAS.461..794P}; $^{b}$ Spectral types are from \citet{2013A&A...551A.107M} and \citet{2017A&A...605A..86M}; $^{c}$ Spectral types are from \citet{2004ApJ...609..917L}, \citet{2017AJ....153...46L}, and \citet{2007ApJS..173..104L};\\
\tablerefs{1. \citet{1997A&A...328..187C}, 2. \citet{1999ApJ...516L..77M}, 3. \citet{2004MNRAS.355..363L}, 4. \citet{2004ApJ...600.1016S}, 5. \citet{1999ApJ...512L..63W},  6. \citet{2006A&A...460..695T}, 7. \citet{2011ApJ...727....6S}, 8. \citet{2004ApJ...616..998W}, 9. \citet{1999A&A...346L..41S}, 10. \citet{2001ApJ...549L.233Z}, 11. \citet{2004ARA&A..42..685Z}, 12. \citet{2002ApJ...575..484G}, 13. \citet{2007ApJ...669L..97L}, 14. \citet{2008AJ....136.1290R}, 15. \citet{1994AJ....108.1071H}, 16. \citet{2003A&A...406.1001C}, 17. \citet{2014ApJ...785..159M}, 18. \citet{2002AJ....124.1670M}, 19. \citet{1997A&A...326..211W}, 20. \citet{1997A&AS..123..329K}, 21. \citet{2002A&A...384..937Z}, 22. \citet{2003A&A...404..171B}, 23. \citet{2012A&A...548A..56R}, 24. \citet{2014ApJ...794...36H}, 25. \citet{2017ApJ...838..150K}, 26. \citet{1998A&A...333..619P}, 27. \citet{2006A&A...445..143C}, 28. \citet{ 2014ApJ...786...97H}.} %\citet{2016MNRAS.461..794P} for TWA 14, RXJ1526.0-4501, RXJ1508.6-4423}
\end{table*}
\normalsize

%\tablefoot{***}
%\end{table*}
%\normalsize


==> tab1.tex <==
%\renewcommand{\tabcolsep}{0.15cm}
\begin{table*}
\caption{Observation logs.}\label{Tab:obs_log}
%\small
\centering
\begin{tabular}{cccccccccccccccccccccccc}
\hline\hline
   %     &          & RA      &DEC     &    &   \\%   &Targets &TO  \\
\cline{5-6}
        &                & RA     & DEC    &Exposure   & Stellar &           &\\
Config. & Obs-date (UT) & (J2000) &(J2000) &(minutes)  & Numbers &Instruments  &PI\\ %&Numbers\\
\hline 
  1  & 2012-05-18   &20:52:50   & 44:19:32   &45   & &MMT/Hectospec  &Fang\\
  2  & 2012-06-14   &20:54:31   & 44:34:32   &45   & &MMT/Hectospec  &Fang \\
  3  & 2012-06-15   &20:57:36   & 43:58:05   &45   & &MMT/Hectospec  &Fang\\
  4  & 2012-11-04   &20:49:23   & 44:39:16   &90   & &MMT/Hectospec  &Hillenbrand\\
  5  & 2012-12-04   &20:56:47   & 43:46:02   &90   & &MMT/Hectospec  &Hillenbrand\\
  6  & 2012-12-06   &20:49:48   & 43:30:23   &90   & &MMT/Hectospec  &Hillenbrand\\
  7  & 2017-06-02   &20:50:51   & 44:08:19   &45   & &MMT/Hectospec  &Fang\\
  8  & 2017-06-04   &20:53:01   & 43:53:15   &45   & &MMT/Hectospec  &Fang\\
  9  & 2017-06-05   &20:55:35   & 44:26:24   &45   & &MMT/Hectospec  &Fang\\
  10 & 2017-06-06   &20:59:09   & 43:30:46   &45   & &MMT/Hectospec  &Fang\\
  \hline
  11 &1998-06-02   &...      & ...        &...   & &WIYN/Hydra \\
  12 &1998-06-05   &...      & ...        &...   & &WIYN/Hydra \\
  13 &1998-07-15   &...      & ...        &...   & &WIYN/Hydra \\
  14 &1998-07-16   &...      & ...        &...   & &WIYN/Hydra \\
  15 &1998-07-16   &...      & ...        &...   & &WIYN/Hydra \\
  16 &1998-07-17   &...      & ...        &...   & &WIYN/Hydra \\
  17 &1998-07-21   &...      & ...        &...   & &WIYN/Hydra \\
  \hline
  F6, 9, 11, 12, 13, 17, 20, 24, 29, 31, 33, 35 &... XXX   &XXX      & XXX        &...   & &Keck/Deimos \\
  \multicolumn{7}{c}{...} \\ 
\hline
\end{tabular}
\end{table*}



==> tab_spt.tex <==
\begin{center}
\startlongtable
\begin{deluxetable*}{rcccrcccccrccccccccccccccccccccccc}
\tablecaption{Young stars in North America Nebula and Pelican}\label{tabe_YSO}
\tablewidth{700pt}
\tablehead{\multicolumn{1}{c}{} &\multicolumn{1}{c}{RA} &\multicolumn{1}{c}{DEC} &\multicolumn{1}{c}{$T_{\rm eff}$}&\multicolumn{1}{c}{Lum} &\multicolumn{1}{c}{Av} &\multicolumn{5}{c}{YSO criteria} \\
\cline{7-11}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{(J2000)} &\multicolumn{1}{c}{(J2000)} &\multicolumn{1}{c}{(K)}&\multicolumn{1}{c}{($L_{\odot}$)} &\multicolumn{1}{c}{(mag)} &\multicolumn{1}{c}{IRE} &\multicolumn{1}{c}{Li}&\multicolumn{1}{c}{Na I}&\multicolumn{1}{c}{X-ray}&\multicolumn{1}{c}{var}}
\startdata
1  & 20 49 11.78  &$+$44 12 33.3  &   3970  &        1.292&  3.7&Y&Y&\nodata&\nodata\\
2  & 20 49 14.46  &$+$44 14 50.3  &   3015  &        0.202&  2.0&Y&Y&\nodata&\nodata\\
3  & 20 49 20.28  &$+$44 35 13.8  &   3437  &        0.362&  2.4&Y&Y&\nodata&\nodata\\
4  & 20 49 24.75  &$+$44 35 22.0  &   2908  &        0.171&  2.0&Y&\nodata&\nodata&\nodata\\
5  & 20 49 32.18  &$+$44 17 03.4  &   3546  &        0.615&  2.6&Y&Y&\nodata&\nodata\\
6  & 20 49 35.85  &$+$44 30 45.3  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
7  & 20 49 53.49  &$+$44 10 17.2  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
8  & 20 50 06.07  &$+$44 17 49.3  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
9  & 20 50 09.89  &$+$44 15 22.0  &   3602  &        0.383&  2.9&Y&Y&\nodata&\nodata\\
10  & 20 50 22.42  &$+$44 19 17.6  &   3360  &        0.738&  4.9&Y&\nodata&\nodata&Y\\
11  & 20 50 27.71  &$+$44 23 29.2  &   5008  &        4.819&  3.3&Y&Y&\nodata&\nodata\\
12  & 20 50 31.96  &$+$44 12 48.7  &   6750  &       17.495&  7.3&N&\nodata&\nodata&\nodata\\
13  & 20 50 32.33  &$+$44 26 17.9  &   4068  &        2.152&  5.3&Y&Y&\nodata&\nodata\\
14  & 20 50 33.06  &$+$44 15 38.9  &   3602  &        0.435&  1.8&Y&Y&\nodata&Y\\
15  & 20 50 36.94  &$+$44 21 40.8  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
16  & 20 50 36.97  &$+$44 20 49.8  &   3964  &        2.333&  1.8&Y&Y&\nodata&Y\\
17  & 20 50 37.02  &$+$44 18 24.6  &   3952  &        4.666&  2.7&Y&Y&\nodata&\nodata\\
18  & 20 50 37.44  &$+$44 21 15.9  &   3279  &        1.121&  3.5&Y&Y&\nodata&\nodata\\
19  & 20 50 39.12  &$+$44 30 38.1  &   3970  &        0.255&  4.2&Y&Y&\nodata&\nodata\\
20  & 20 50 40.27  &$+$44 30 49.2  &   4216  &        2.137&  2.8&Y&Y&\nodata&\nodata\\
21  & 20 50 40.46  &$+$44 20 21.7  &   3160  &        0.380&  1.5&Y&Y&\nodata&\nodata\\
22  & 20 50 40.54  &$+$44 20 51.0  &   3385  &        1.223&  2.7&Y&Y&\nodata&Y\\
23  & 20 50 42.77  &$+$44 21 55.0  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
24  & 20 50 43.53  &$+$44 15 52.0  &   3686  &        0.608&  1.4&Y&Y&\nodata&Y\\
25  & 20 50 43.72  &$+$44 16 49.3  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
26  & 20 50 44.93  &$+$44 15 55.1  &   3372  &        1.411&  1.8&Y&Y&\nodata&Y\\
27  & 20 50 45.74  &$+$44 11 55.3  &*******  &          NaN&  NaN&N&\nodata&\nodata&\nodata\\
28  & 20 50 46.08  &$+$44 19 10.4  &   3503  &        0.775&  1.0&Y&Y&\nodata&Y\\
29  & 20 50 46.40  &$+$44 31 12.4  &   3791  &        0.319&  5.8&Y&\nodata&\nodata&\nodata\\
30  & 20 50 47.00  &$+$44 17 29.5  &   3657  &        1.412&  2.3&Y&Y&\nodata&Y\\
31  & 20 50 48.10  &$+$44 33 37.1  &   3450  &        0.486&  2.2&Y&\nodata&\nodata&\nodata\\
32  & 20 50 48.58  &$+$44 21 04.5  &   3160  &        0.285&  2.0&Y&Y&\nodata&Y\\
33  & 20 50 48.71  &$+$44 20 53.7  &   3858  &        0.941&  2.0&Y&Y&\nodata&Y\\
34  & 20 50 48.80  &$+$44 19 23.7  &   3299  &        0.782&  2.1&Y&Y&\nodata&Y\\
35  & 20 50 50.38  &$+$44 50 11.6  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
36  & 20 50 52.56  &$+$44 16 44.3  &   4506  &        2.632&  1.9&Y&Y&\nodata&\nodata\\
37  & 20 50 53.16  &$+$44 23 53.7  &   3340  &        0.648&  1.5&Y&Y&\nodata&Y\\
38  & 20 50 53.57  &$+$44 21 01.1  &   4010  &        3.321&  2.4&Y&Y&\nodata&\nodata\\
39  & 20 50 53.62  &$+$44 24 29.9  &   5370  &        4.684&  5.6&Y&Y&\nodata&\nodata\\
40  & 20 50 53.87  &$+$44 21 38.8  &   2980  &        0.185&  1.1&Y&\nodata&\nodata&\nodata\\
41  & 20 50 54.18  &$+$44 38 08.3  &   3928  &        0.901&  2.4&Y&Y&\nodata&Y\\
42  & 20 50 54.29  &$+$44 17 52.8  &Cont  &\nodata&\nodata&Y&Y&\nodata&\nodata\\
43  & 20 50 54.88  &$+$44 22 58.4  &   3713  &        0.294&  2.2&Y&Y&\nodata&Y\\
44  & 20 50 55.58  &$+$44 24 24.6  &   3546  &        0.142&  4.6&Y&\nodata&\nodata&\nodata\\
45  & 20 50 55.65  &$+$44 17 50.3  &   3916  &        1.604&  2.5&Y&Y&\nodata&Y\\
46  & 20 50 57.46  &$+$44 24 46.6  &   4292  &        1.719&  5.0&Y&Y&\nodata&\nodata\\
47  & 20 50 58.18  &$+$44 29 59.2  &   3686  &        0.739&  1.5&N&Y&\nodata&Y\\
48  & 20 50 58.34  &$+$44 14 32.5  &   5310  &        2.958&  2.5&Y&Y&\nodata&Y\\
49  & 20 50 58.39  &$+$44 14 44.5  &   3700  &        2.846&  1.4&Y&Y&\nodata&Y\\
50  & 20 50 58.70  &$+$44 17 31.0  &   3928  &        1.113&  1.9&Y&Y&\nodata&\nodata\\
51  & 20 50 58.74  &$+$44 23 17.8  &   3412  &        0.210&  1.0&Y&Y&\nodata&Y\\
52  & 20 50 59.04  &$+$44 19 53.9  &   3299  &        0.409&  1.5&Y&Y&\nodata&\nodata\\
53  & 20 50 59.47  &$+$44 19 39.3  &   3385  &        0.380&  1.7&Y&Y&\nodata&Y\\
54  & 20 50 59.74  &$+$44 40 49.1  &   4253  &        2.216&  4.2&Y&Y&\nodata&\nodata\\
55  & 20 51 00.89  &$+$44 31 49.9  &   4043  &        0.890&  1.6&Y&Y&\nodata&\nodata\\
56  & 20 51 01.44  &$+$44 13 29.7  &*******  &          NaN&  NaN&N&Y&\nodata&Y\\
57  & 20 51 01.46  &$+$44 15 34.7  &   3835  &        0.906&  2.0&Y&Y&\nodata&Y\\
58  & 20 51 01.56  &$+$44 15 42.2  &   3990  &        1.373&  1.6&Y&Y&\nodata&Y\\
59  & 20 51 02.19  &$+$44 20 09.4  &   3052  &        0.229&  1.2&Y&Y&\nodata&Y\\
60  & 20 51 03.18  &$+$44 24 04.1  &   3657  &        0.536&  2.2&Y&Y&\nodata&\nodata\\
61  & 20 51 03.32  &$+$44 24 15.7  &   3657  &        0.486&  1.4&Y&Y&\nodata&Y\\
62  & 20 51 03.35  &$+$44 14 40.4  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
63  & 20 51 04.64  &$+$44 23 50.3  &   5390  &        5.417&  2.6&Y&Y&\nodata&Y\\
64  & 20 51 05.47  &$+$44 14 00.4  &   3160  &        0.780&  2.1&Y&\nodata&\nodata&\nodata\\
65  & 20 51 05.69  &$+$44 16 32.5  &   4550  &        4.915&  2.9&Y&Y&\nodata&Y\\
66  & 20 51 06.25  &$+$44 18 30.9  &*******  &          NaN&  NaN&N&\nodata&\nodata&\nodata\\
67  & 20 51 08.03  &$+$44 31 50.4  &   3643  &        0.556&  2.3&Y&Y&\nodata&\nodata\\
68  & 20 51 08.28  &$+$44 16 51.4  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
69  & 20 51 08.94  &$+$44 16 42.0  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
70  & 20 51 09.49  &$+$44 33 29.7  &   3199  &        0.771&  2.1&Y&Y&\nodata&\nodata\\
71  & 20 51 10.98  &$+$44 36 44.7  &   3260  &        0.314&  1.6&Y&Y&\nodata&\nodata\\
72  & 20 51 12.09  &$+$44 18 47.7  &   3087  &        0.403&  1.5&Y&Y&\nodata&\nodata\\
73  & 20 51 12.52  &$+$44 18 09.4  &   3940  &        0.303&  1.6&N&Y&\nodata&Y\\
74  & 20 51 13.43  &$+$44 26 18.4  &   3412  &        0.217&  2.4&Y&Y&\nodata&\nodata\\
75  & 20 51 13.65  &$+$44 32 22.7  &   3770  &        1.074&  2.1&Y&Y&\nodata&\nodata\\
76  & 20 51 13.79  &$+$44 31 53.2  &   3087  &        0.238&  1.9&Y&\nodata&\nodata&\nodata\\
77  & 20 51 14.55  &$+$44 13 38.1  &   3320  &        0.647&  2.1&Y&Y&\nodata&\nodata\\
78  & 20 51 15.12  &$+$44 18 17.8  &   3946  &        0.785&  2.3&Y&Y&\nodata&Y\\
79  & 20 51 15.61  &$+$44 14 55.3  &   3990  &        1.975&  2.0&Y&Y&\nodata&\nodata\\
80  & 20 51 16.05  &$+$44 15 00.2  &   3990  &        0.719&  2.9&Y&Y&\nodata&\nodata\\
81  & 20 51 16.50  &$+$44 22 58.0  &   5039  &        2.220&  1.8&Y&Y&\nodata&\nodata\\
82  & 20 51 17.70  &$+$44 18 30.2  &   3657  &        0.738&  2.1&Y&Y&\nodata&Y\\
83  & 20 51 18.23  &$+$44 13 08.3  &   3975  &        1.731&  2.0&Y&Y&\nodata&\nodata\\
84  & 20 51 19.44  &$+$44 19 30.7  &   3672  &        0.363&  1.6&Y&Y&\nodata&Y\\
85  & 20 51 19.85  &$+$44 23 06.7  &   3464  &        0.364&  2.4&Y&Y&\nodata&\nodata\\
86  & 20 51 20.97  &$+$44 26 19.7  &   3940  &        2.631&  2.3&Y&Y&\nodata&Y\\
87  & 20 51 22.45  &$+$44 20 47.3  &   2980  &        0.218&  2.4&Y&\nodata&\nodata&\nodata\\
88  & 20 51 22.58  &$+$44 25 15.9  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
89  & 20 51 22.66  &$+$44 21 07.8  &   3952  &        1.116&  2.1&Y&Y&\nodata&Y\\
90  & 20 51 22.80  &$+$44 33 42.8  &   3946  &        0.498&  1.7&Y&Y&\nodata&\nodata\\
91  & 20 51 23.60  &$+$44 15 42.7  &   3517  &        0.420&  2.3&Y&Y&\nodata&Y\\
92  & 20 51 23.64  &$+$44 31 37.1  &   3260  &        0.221&  1.6&Y&Y&\nodata&\nodata\\
93  & 20 51 23.66  &$+$44 35 22.6  &   3657  &        0.090&  1.0&Y&Y&\nodata&\nodata\\
94  & 20 51 24.04  &$+$44 32 57.2  &   3339  &        0.157&  2.0&Y&Y&\nodata&\nodata\\
95  & 20 51 24.14  &$+$44 17 57.0  &   2896  &        0.390&  2.5&Y&Y&\nodata&Y\\
96  & 20 51 24.40  &$+$44 13 04.7  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
97  & 20 51 24.64  &$+$44 17 55.1  &Cont  &\nodata&\nodata&Y&Y&\nodata&\nodata\\
98  & 20 51 24.70  &$+$44 18 18.8  &   3340  &        0.448&  2.1&Y&Y&\nodata&\nodata\\
99  & 20 51 26.20  &$+$44 30 34.6  &Cont  &\nodata&\nodata&Y&Y&\nodata&\nodata\\
100  & 20 51 26.27  &$+$44 16 59.6  &   2689  &        0.077&  3.8&Y&\nodata&\nodata&\nodata\\
101  & 20 51 26.45  &$+$43 53 12.6  &   3958  &        0.912&  2.3&Y&Y&\nodata&\nodata\\
102  & 20 51 26.53  &$+$44 36 28.7  &   3940  &        0.331&  2.6&Y&Y&\nodata&\nodata\\
103  & 20 51 26.75  &$+$44 04 24.7  &   3517  &        0.984&  2.2&Y&Y&\nodata&\nodata\\
104  & 20 51 26.97  &$+$44 13 15.6  &   3946  &        0.890&  2.5&Y&Y&\nodata&\nodata\\
105  & 20 51 28.44  &$+$44 26 01.2  &   3966  &        0.362&  2.7&Y&Y&\nodata&Y\\
106  & 20 51 28.56  &$+$44 15 45.5  &   3412  &        0.354&  1.6&Y&Y&\nodata&Y\\
107  & 20 51 29.67  &$+$44 32 19.7  &   5390  &        4.570&  1.7&Y&\nodata&\nodata&\nodata\\
108  & 20 51 30.56  &$+$44 03 45.1  &   4235  &        2.784&  2.0&Y&Y&\nodata&\nodata\\
109  & 20 51 30.89  &$+$44 06 59.6  &   4528  &        0.802&  1.7&Y&Y&\nodata&\nodata\\
110  & 20 51 31.64  &$+$44 13 01.4  &   3437  &        0.283&  2.3&Y&Y&\nodata&\nodata\\
111  & 20 51 31.87  &$+$44 02 54.3  &   3088  &        0.371&  2.2&Y&Y&\nodata&\nodata\\
112  & 20 51 32.77  &$+$43 11 22.3  &   3835  &        0.366&  1.5&N&Y&\nodata&\nodata\\
113  & 20 51 32.77  &$+$44 23 48.1  &   3835  &        0.685&  2.1&Y&Y&\nodata&\nodata\\
114  & 20 51 33.11  &$+$44 36 59.7  &   3835  &        0.309&  2.5&Y&Y&\nodata&\nodata\\
115  & 20 51 33.37  &$+$44 26 37.0  &   5350  &        9.653&  4.1&Y&Y&\nodata&Y\\
116  & 20 51 33.39  &$+$44 34 54.4  &   4374  &        0.931&  2.5&Y&Y&\nodata&\nodata\\
117  & 20 51 33.69  &$+$44 10 14.6  &   3477  &        0.430&  1.9&Y&Y&\nodata&\nodata\\
118  & 20 51 35.39  &$+$44 30 39.2  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
119  & 20 51 37.60  &$+$44 20 04.6  &   3437  &        0.451&  1.9&N&Y&\nodata&\nodata\\
120  & 20 51 37.95  &$+$43 23 04.6  &   3858  &        1.102&  2.8&Y&Y&\nodata&\nodata\\
121  & 20 51 38.26  &$+$43 57 14.0  &   3320  &        0.084&  1.7&Y&\nodata&\nodata&\nodata\\
122  & 20 51 38.65  &$+$44 03 41.0  &   3464  &        0.829&  2.7&Y&Y&\nodata&\nodata\\
123  & 20 51 39.24  &$+$44 24 28.1  &   5330  &        8.377&  3.8&Y&Y&\nodata&Y\\
124  & 20 51 39.95  &$+$44 33 14.3  &   4000  &        0.760&  2.7&Y&Y&\nodata&\nodata\\
125  & 20 51 40.69  &$+$43 13 14.0  &   2883  &        0.226&  2.9&Y&Y&\nodata&\nodata\\
126  & 20 51 41.25  &$+$43 47 54.9  &   3952  &        2.459&  2.3&N&Y&\nodata&\nodata\\
127  & 20 51 41.40  &$+$44 15 07.2  &Cont  &\nodata&\nodata&Y&Y&\nodata&\nodata\\
128  & 20 51 41.90  &$+$44 16 08.3  &   4020  &        0.888&  2.2&Y&Y&\nodata&Y\\
129  & 20 51 42.09  &$+$44 38 56.7  &   4550  &        5.087&  3.5&Y&Y&\nodata&\nodata\\
130  & 20 51 42.89  &$+$44 07 30.7  &   3904  &        0.209&  3.8&Y&\nodata&\nodata&\nodata\\
131  & 20 51 44.73  &$+$44 08 47.0  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
132  & 20 51 45.20  &$+$43 49 02.4  &   5290  &        2.733&  6.9&Y&Y&\nodata&\nodata\\
133  & 20 51 45.98  &$+$44 28 35.4  &   3437  &        0.384&  2.4&Y&Y&\nodata&Y\\
134  & 20 51 46.12  &$+$44 23 09.1  &   2956  &        0.111&  2.9&Y&\nodata&\nodata&\nodata\\
135  & 20 51 47.41  &$+$44 32 08.2  &   3412  &        0.271&  2.0&Y&Y&\nodata&\nodata\\
136  & 20 51 48.54  &$+$44 05 19.7  &   3464  &        0.672&  1.7&Y&Y&\nodata&\nodata\\
137  & 20 51 48.75  &$+$44 23 40.8  &   3490  &        0.379&  2.2&Y&Y&\nodata&\nodata\\
138  & 20 51 48.85  &$+$44 11 02.8  &   3958  &        0.687&  3.0&Y&Y&\nodata&\nodata\\
139  & 20 51 51.25  &$+$44 15 12.3  &   3385  &        0.127&  5.9&Y&\nodata&\nodata&\nodata\\
140  & 20 51 52.01  &$+$43 10 46.9  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
141  & 20 51 52.24  &$+$44 18 21.4  &   3437  &        0.289&  2.7&Y&Y&\nodata&\nodata\\
142  & 20 51 52.90  &$+$44 15 57.5  &Cont  &\nodata&\nodata&Y&Y&\nodata&\nodata\\
143  & 20 51 55.68  &$+$44 33 52.7  &   5330  &        3.577&  3.8&Y&Y&\nodata&\nodata\\
144  & 20 51 57.21  &$+$44 02 16.1  &   3964  &        0.263&  2.9&Y&Y&\nodata&\nodata\\
145  & 20 51 57.50  &$+$44 27 17.4  &   3240  &        0.324&  1.6&Y&Y&\nodata&\nodata\\
146  & 20 51 58.04  &$+$44 04 21.0  &   3142  &        0.299&  2.3&Y&Y&\nodata&\nodata\\
147  & 20 51 58.47  &$+$44 37 24.2  &   3952  &        1.348&  3.7&Y&Y&\nodata&Y\\
148  & 20 51 58.63  &$+$44 14 56.8  &   3904  &        1.485&  3.9&Y&Y&\nodata&\nodata\\
149  & 20 51 58.67  &$+$44 30 06.3  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
150  & 20 51 58.68  &$+$44 30 27.4  &   3260  &        0.442&  2.5&Y&\nodata&\nodata&\nodata\\
151  & 20 51 59.19  &$+$44 25 43.9  &   3940  &        2.684&  2.3&Y&Y&\nodata&Y\\
152  & 20 51 59.42  &$+$43 50 42.0  &   4461  &        5.466&  2.8&Y&Y&\nodata&\nodata\\
153  & 20 51 59.40  &$+$44 16 22.1  &   4292  &        2.610&  2.3&Y&Y&\nodata&\nodata\\
154  & 20 52 00.16  &$+$44 19 59.0  &   3517  &        0.482&  2.2&Y&Y&\nodata&\nodata\\
155  & 20 52 00.97  &$+$44 28 41.5  &   3517  &        0.522&  2.0&Y&Y&\nodata&\nodata\\
156  & 20 52 01.11  &$+$44 32 39.1  &   4068  &        1.173&  1.9&N&Y&\nodata&Y\\
157  & 20 52 01.61  &$+$44 20 32.6  &   3517  &        0.671&  1.9&Y&Y&\nodata&\nodata\\
158  & 20 52 02.66  &$+$44 27 28.8  &   3490  &        0.350&  1.9&Y&Y&\nodata&\nodata\\
159  & 20 52 02.91  &$+$44 13 51.9  &   3412  &        0.508&  3.4&Y&Y&\nodata&\nodata\\
160  & 20 52 03.64  &$+$44 28 38.0  &   3464  &        0.213&  1.4&Y&Y&\nodata&\nodata\\
161  & 20 52 05.28  &$+$44 17 29.3  &   3630  &        0.607&  2.2&Y&Y&\nodata&\nodata\\
162  & 20 52 06.73  &$+$44 27 55.7  &   3891  &        0.556&  2.0&Y&Y&\nodata&\nodata\\
163  & 20 52 06.74  &$+$44 33 55.0  &   3490  &        0.155&  2.9&Y&\nodata&\nodata&\nodata\\
164  & 20 52 07.96  &$+$43 54 16.2  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
165  & 20 52 08.56  &$+$44 34 15.1  &   3320  &        0.499&  4.5&Y&Y&\nodata&\nodata\\
166  & 20 52 10.99  &$+$44 08 10.2  &   3490  &        0.289&  2.5&Y&Y&\nodata&\nodata\\
167  & 20 52 11.55  &$+$44 17 54.7  &*******  &          NaN&  NaN&N&Y&\nodata&Y\\
168  & 20 52 12.92  &$+$44 20 53.4  &   4330  &        1.262&  4.1&Y&Y&\nodata&Y\\
169  & 20 52 13.58  &$+$44 12 02.0  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
170  & 20 52 13.57  &$+$43 40 38.9  &   3891  &        1.243&  3.9&Y&Y&\nodata&\nodata\\
171  & 20 52 14.91  &$+$44 20 38.2  &   3052  &        0.056&  4.2&Y&\nodata&\nodata&\nodata\\
172  & 20 52 15.12  &$+$44 17 20.5  &   3015  &        0.464&  2.9&Y&\nodata&\nodata&\nodata\\
173  & 20 52 15.14  &$+$43 30 07.5  &   3979  &        2.851&  4.6&Y&Y&\nodata&\nodata\\
174  & 20 52 15.43  &$+$44 28 10.9  &   3869  &        0.821&  2.2&Y&Y&\nodata&\nodata\\
175  & 20 52 17.83  &$+$44 21 15.9  &   3958  &        0.766&  2.5&Y&Y&\nodata&Y\\
176  & 20 52 18.37  &$+$44 25 02.1  &   4330  &        0.086&  2.5&Y&\nodata&\nodata&\nodata\\
177  & 20 52 18.40  &$+$44 16 30.5  &   3825  &        0.829&  3.4&Y&Y&\nodata&\nodata\\
178  & 20 52 18.44  &$+$44 05 15.0  &   3437  &        0.401&  3.4&Y&Y&\nodata&\nodata\\
179  & 20 52 19.68  &$+$44 24 49.2  &   3160  &        0.175&  1.3&Y&Y&\nodata&\nodata\\
180  & 20 52 20.22  &$+$44 30 30.9  &   4000  &        0.217&  3.7&Y&Y&\nodata&Y\\
181  & 20 52 20.31  &$+$43 58 42.7  &   3279  &        0.257&  2.6&Y&\nodata&\nodata&\nodata\\
182  & 20 52 22.51  &$+$44 14 00.2  &   5309  &        2.388&  3.2&Y&Y&\nodata&\nodata\\
183  & 20 52 22.85  &$+$44 27 02.9  &   2760  &        0.034&  1.2&Y&\nodata&\nodata&\nodata\\
184  & 20 52 23.28  &$+$43 04 56.4  &   3464  &        0.483&  1.7&Y&Y&\nodata&\nodata\\
185  & 20 52 24.01  &$+$44 31 55.4  &   3160  &        0.172&  2.5&Y&\nodata&\nodata&\nodata\\
186  & 20 52 24.56  &$+$44 23 55.2  &   3320  &        0.189&  2.2&Y&\nodata&\nodata&\nodata\\
187  & 20 52 25.22  &$+$44 25 55.2  &*******  &          NaN&  NaN&N&Y&\nodata&Y\\
188  & 20 52 25.37  &$+$44 14 32.4  &   3015  &        0.118&  2.3&Y&\nodata&\nodata&\nodata\\
189  & 20 52 25.57  &$+$44 29 11.9  &   3052  &        0.094&  3.6&Y&\nodata&\nodata&\nodata\\
190  & 20 52 25.89  &$+$44 25 22.2  &   3052  &        0.128&  2.8&Y&Y&\nodata&\nodata\\
191  & 20 52 26.19  &$+$44 34 26.2  &*******  &          NaN&  NaN&N&\nodata&\nodata&Y\\
192  & 20 52 26.72  &$+$44 26 33.2  &   3517  &        0.410&  2.9&Y&Y&\nodata&\nodata\\
193  & 20 52 26.75  &$+$44 17 06.5  &   5390  &        8.462&  2.6&Y&\nodata&\nodata&Y\\
194  & 20 52 27.17  &$+$44 04 39.1  &   3199  &        0.604&  3.3&Y&\nodata&\nodata&\nodata\\
195  & 20 52 28.02  &$+$44 03 31.0  &   5370  &        7.657&  4.7&Y&Y&\nodata&\nodata\\
196  & 20 52 28.31  &$+$44 21 14.6  &   3946  &        0.562&  2.0&Y&Y&\nodata&Y\\
197  & 20 52 28.79  &$+$44 18 29.7  &   3425  &        0.303&  1.8&Y&Y&\nodata&\nodata\\
198  & 20 52 29.61  &$+$44 34 18.5  &   3199  &        0.062&  3.1&Y&\nodata&\nodata&\nodata\\
199  & 20 52 29.76  &$+$44 21 04.6  &   3220  &        0.323&  2.5&Y&Y&\nodata&\nodata\\
200  & 20 52 30.80  &$+$44 30 35.1  &   3756  &        0.455&  3.4&Y&\nodata&\nodata&Y\\
201  & 20 52 30.88  &$+$44 20 11.6  &   3946  &        0.676&  2.6&Y&Y&\nodata&\nodata\\
202  & 20 52 32.11  &$+$44 28 24.2  &   3320  &        0.462&  3.7&Y&\nodata&\nodata&\nodata\\
203  & 20 52 33.30  &$+$44 31 40.8  &   3437  &        0.308&  4.5&Y&\nodata&\nodata&\nodata\\
204  & 20 52 33.79  &$+$44 24 26.3  &   3385  &        0.385&  3.2&Y&Y&\nodata&\nodata\\
205  & 20 52 34.35  &$+$44 17 40.2  &   3791  &        0.531&  2.6&Y&Y&\nodata&\nodata\\
206  & 20 52 34.40  &$+$44 38 24.6  &   3755  &        0.617&  3.9&Y&Y&\nodata&\nodata\\
207  & 20 52 35.29  &$+$44 33 19.4  &   4197  &        3.228&  5.1&Y&Y&\nodata&Y\\
208  & 20 52 35.41  &$+$44 37 22.3  &   3160  &        0.191&  4.1&Y&\nodata&\nodata&\nodata\\
209  & 20 52 35.52  &$+$44 19 10.4  &   3742  &        1.130&  1.9&N&Y&\nodata&Y\\
210  & 20 52 36.47  &$+$44 11 46.4  &   3886  &        0.387&  1.8&Y&Y&\nodata&\nodata\\
211  & 20 52 39.50  &$+$43 59 54.2  &   3770  &        0.555&  2.8&Y&Y&\nodata&\nodata\\
212  & 20 52 39.93  &$+$44 05 49.3  &   3385  &        0.169&  1.4&Y&\nodata&\nodata&\nodata\\
213  & 20 52 41.58  &$+$44 37 20.4  &   3124  &        0.500&  3.3&Y&Y&\nodata&\nodata\\
214  & 20 52 41.70  &$+$44 34 07.1  &*******  &          NaN&  NaN&N&Y&\nodata&Y\\
215  & 20 52 41.84  &$+$44 26 55.1  &   3160  &        0.158&  3.4&Y&\nodata&\nodata&\nodata\\
216  & 20 52 42.58  &$+$44 19 21.1  &   3657  &        0.526&  1.8&Y&Y&\nodata&Y\\
217  & 20 52 42.80  &$+$44 19 10.2  &   3814  &        0.549&  5.6&Y&\nodata&\nodata&\nodata\\
218  & 20 52 44.23  &$+$44 17 50.3  &   3088  &        0.118&  1.8&Y&Y&\nodata&\nodata\\
219  & 20 52 46.14  &$+$44 24 57.8  &Cont  &\nodata&\nodata&Y&Y&\nodata&\nodata\\
220  & 20 52 47.47  &$+$44 15 41.9  &   3385  &        0.317&  2.2&Y&Y&\nodata&\nodata\\
221  & 20 52 48.65  &$+$44 19 50.6  &   3791  &        0.528&  2.6&Y&Y&\nodata&\nodata\\
222  & 20 52 49.07  &$+$44 15 20.2  &   3412  &        0.197&  1.9&Y&Y&\nodata&\nodata\\
223  & 20 52 49.81  &$+$44 19 02.0  &   4215  &        1.885&  2.2&Y&Y&\nodata&Y\\
224  & 20 52 50.63  &$+$43 42 55.4  &   3742  &        0.243&  2.1&Y&Y&\nodata&\nodata\\
225  & 20 52 51.90  &$+$44 25 44.3  &   3015  &        0.091&  3.3&Y&\nodata&\nodata&\nodata\\
226  & 20 52 52.48  &$+$44 14 25.1  &   3970  &        0.545&  4.4&Y&Y&\nodata&\nodata\\
227  & 20 52 53.41  &$+$44 19 36.5  &   5330  &        5.406&  6.9&Y&Y&\nodata&\nodata\\
228  & 20 52 53.73  &$+$44 14 57.0  &   3940  &        0.181&  2.5&Y&Y&\nodata&\nodata\\
229  & 20 52 54.30  &$+$43 52 16.6  &   3869  &        0.406&  2.5&Y&Y&\nodata&\nodata\\
230  & 20 52 55.39  &$+$44 16 57.8  &   3320  &        0.179&  1.7&Y&Y&\nodata&\nodata\\
231  & 20 52 55.61  &$+$43 56 43.9  &   3240  &        0.119&  3.4&Y&\nodata&\nodata&\nodata\\
232  & 20 52 56.91  &$+$44 26 00.5  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&Y\\
233  & 20 52 57.26  &$+$44 40 46.4  &   3970  &        2.071&  3.8&Y&Y&\nodata&Y\\
234  & 20 52 58.83  &$+$44 15 03.8  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
235  & 20 53 00.56  &$+$44 36 35.7  &   3770  &        0.584&  5.2&Y&\nodata&\nodata&\nodata\\
236  & 20 53 01.78  &$+$44 19 05.7  &   4010  &        1.443&  4.3&Y&Y&\nodata&Y\\
237  & 20 53 02.35  &$+$44 00 47.3  &   2883  &        0.190&  4.4&Y&\nodata&\nodata&\nodata\\
238  & 20 53 03.27  &$+$44 39 48.9  &   3970  &        1.062&  4.4&Y&Y&\nodata&\nodata\\
239  & 20 53 04.62  &$+$44 39 47.0  &   3814  &        0.578&  4.4&Y&\nodata&\nodata&\nodata\\
240  & 20 53 05.72  &$+$44 42 37.0  &   5330  &       10.615&  5.3&Y&Y&\nodata&\nodata\\
241  & 20 53 05.93  &$+$44 15 38.6  &   3412  &        0.312&  2.8&Y&\nodata&\nodata&\nodata\\
242  & 20 53 07.40  &$+$44 14 37.9  &   3124  &        0.114&  3.6&Y&\nodata&\nodata&\nodata\\
243  & 20 53 08.14  &$+$44 05 13.4  &   3385  &        0.361&  3.1&Y&\nodata&\nodata&\nodata\\
244  & 20 53 09.04  &$+$44 30 10.7  &   3928  &        1.230&  4.6&Y&Y&\nodata&\nodata\\
245  & 20 53 09.14  &$+$44 21 16.6  &   2980  &        0.176&  3.2&Y&\nodata&\nodata&\nodata\\
246  & 20 53 10.28  &$+$44 21 48.9  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
247  & 20 53 12.27  &$+$43 38 28.6  &   4253  &        0.723&  2.2&Y&Y&\nodata&\nodata\\
248  & 20 53 12.50  &$+$44 35 24.6  &   3160  &        0.113&  3.1&Y&\nodata&\nodata&\nodata\\
249  & 20 53 12.49  &$+$44 31 06.7  &   3464  &        0.997&  4.7&Y&\nodata&\nodata&Y\\
250  & 20 53 13.99  &$+$44 12 57.7  &   4010  &        0.743&  2.9&Y&Y&\nodata&\nodata\\
251  & 20 53 14.57  &$+$44 29 06.4  &   4000  &        0.999&  3.5&Y&Y&\nodata&Y\\
252  & 20 53 14.90  &$+$44 34 34.7  &   3464  &        0.334&  4.4&Y&\nodata&\nodata&\nodata\\
253  & 20 53 15.13  &$+$44 38 48.3  &   3949  &        0.793&  4.5&Y&Y&\nodata&\nodata\\
254  & 20 53 15.64  &$+$43 44 22.8  &   3437  &        0.232&  2.2&Y&Y&\nodata&\nodata\\
255  & 20 53 15.88  &$+$44 29 47.5  &   3880  &        0.693&  4.2&Y&\nodata&\nodata&\nodata\\
256  & 20 53 16.52  &$+$44 29 33.8  &   3199  &        0.132&  4.2&Y&\nodata&\nodata&\nodata\\
257  & 20 53 16.68  &$+$44 40 54.1  &   3088  &        0.159&  3.8&Y&\nodata&\nodata&\nodata\\
258  & 20 53 16.83  &$+$44 25 41.8  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
259  & 20 53 17.05  &$+$44 38 34.2  &   3928  &        3.592&  4.7&Y&Y&\nodata&Y\\
260  & 20 53 17.70  &$+$44 03 05.4  &   2860  &        0.090&  2.3&Y&\nodata&\nodata&\nodata\\
261  & 20 53 17.89  &$+$44 18 04.4  &   2931  &        0.069&  2.4&Y&\nodata&\nodata&\nodata\\
262  & 20 53 18.91  &$+$44 14 38.8  &   3791  &        0.387&  3.6&Y&Y&\nodata&\nodata\\
263  & 20 53 21.20  &$+$44 53 21.4  &   2931  &        0.137&  4.8&Y&\nodata&\nodata&\nodata\\
264  & 20 53 22.34  &$+$44 38 52.9  &   5800  &       13.874&  5.3&N&\nodata&\nodata&Y\\
265  & 20 53 23.92  &$+$43 54 18.1  &   5400  &       16.829&  4.1&Y&Y&\nodata&\nodata\\
266  & 20 53 23.93  &$+$44 21 58.2  &   3360  &        0.495&  4.0&Y&\nodata&\nodata&\nodata\\
267  & 20 53 24.67  &$+$44 02 31.0  &   7500  &     1666.129& 18.1&Y&\nodata&\nodata&\nodata\\
268  & 20 53 24.63  &$+$44 20 34.4  &   3990  &        1.340&  2.4&N&Y&\nodata&\nodata\\
269  & 20 53 25.75  &$+$44 10 45.6  &   4020  &        1.260&  2.6&N&Y&\nodata&\nodata\\
270  & 20 53 27.13  &$+$44 58 21.1  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
271  & 20 53 27.15  &$+$44 27 11.0  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
272  & 20 53 27.74  &$+$44 10 34.7  &   3955  &        0.973&  3.6&Y&Y&\nodata&\nodata\\
273  & 20 53 28.21  &$+$44 18 20.7  &   3630  &        0.372&  2.4&N&Y&\nodata&\nodata\\
274  & 20 53 29.33  &$+$44 27 29.7  &   2932  &        0.163&  2.6&Y&\nodata&\nodata&\nodata\\
275  & 20 53 29.69  &$+$44 23 56.9  &   3713  &        0.435&  2.5&Y&Y&\nodata&\nodata\\
276  & 20 53 30.26  &$+$44 29 12.7  &   3898  &        2.470&  5.6&Y&\nodata&\nodata&\nodata\\
277  & 20 53 30.44  &$+$44 26 44.2  &   3803  &        0.893&  4.8&Y&Y&\nodata&\nodata\\
278  & 20 53 30.66  &$+$44 25 42.7  &   3015  &        0.063&  1.6&Y&\nodata&\nodata&\nodata\\
279  & 20 53 31.09  &$+$44 23 26.7  &   5330  &        5.431&  3.4&Y&Y&\nodata&Y\\
280  & 20 53 31.28  &$+$44 19 09.6  &   3464  &        0.313&  2.2&Y&Y&\nodata&\nodata\\
281  & 20 53 31.38  &$+$44 13 34.5  &   4000  &        0.835&  3.4&Y&Y&\nodata&\nodata\\
282  & 20 53 31.49  &$+$44 12 45.8  &   3490  &        0.449&  3.8&Y&\nodata&\nodata&\nodata\\
283  & 20 53 31.96  &$+$44 09 47.0  &   3928  &        0.682&  4.4&Y&Y&\nodata&\nodata\\
284  & 20 53 32.05  &$+$44 29 06.1  &   3951  &        0.761&  4.3&Y&\nodata&\nodata&\nodata\\
285  & 20 53 33.29  &$+$44 23 28.7  &   3791  &        0.425&  2.4&Y&Y&\nodata&\nodata\\
286  & 20 53 34.10  &$+$44 20 18.0  &   3503  &        0.166&  1.3&Y&Y&\nodata&\nodata\\
287  & 20 53 34.77  &$+$44 29 18.1  &   3979  &        2.250&  4.3&Y&Y&\nodata&Y\\
288  & 20 53 35.23  &$+$44 16 52.5  &   3916  &        0.564&  2.8&Y&Y&\nodata&\nodata\\
289  & 20 53 35.44  &$+$44 27 48.3  &Cont  &\nodata&\nodata&Y&Y&\nodata&\nodata\\
290  & 20 53 35.58  &$+$44 27 23.8  &   3160  &        0.379&  3.2&Y&Y&\nodata&\nodata\\
291  & 20 53 35.77  &$+$44 28 40.8  &   3124  &        0.312&  4.7&Y&\nodata&\nodata&\nodata\\
292  & 20 53 36.28  &$+$44 16 26.2  &   3949  &        0.479&  3.1&Y&Y&\nodata&\nodata\\
293  & 20 53 36.51  &$+$44 53 13.7  &   3160  &        0.301&  2.0&Y&Y&\nodata&\nodata\\
294  & 20 53 38.29  &$+$44 14 50.7  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
295  & 20 53 38.54  &$+$44 25 43.5  &   3770  &        0.501&  3.5&Y&Y&\nodata&\nodata\\
296  & 20 53 38.72  &$+$43 56 27.1  &   3160  &        0.145&  2.3&Y&\nodata&\nodata&\nodata\\
297  & 20 53 38.75  &$+$44 26 29.9  &   3124  &        0.138&  4.0&Y&\nodata&\nodata&\nodata\\
298  & 20 53 40.14  &$+$44 10 45.7  &   3891  &        0.817&  4.4&Y&Y&\nodata&\nodata\\
299  & 20 53 41.81  &$+$44 27 03.1  &   3964  &        0.851&  3.9&Y&Y&\nodata&\nodata\\
300  & 20 53 42.61  &$+$43 53 53.7  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
301  & 20 53 42.70  &$+$44 03 48.7  &   3970  &        2.061&  2.8&Y&Y&\nodata&\nodata\\
302  & 20 53 43.23  &$+$44 27 36.8  &   3052  &        0.375&  3.9&Y&\nodata&\nodata&\nodata\\
303  & 20 53 43.42  &$+$44 23 12.8  &   3858  &        0.414&  3.3&Y&Y&\nodata&\nodata\\
304  & 20 53 44.90  &$+$44 01 15.2  &   3437  &        0.211&  2.2&Y&Y&\nodata&\nodata\\
305  & 20 53 45.07  &$+$44 25 17.9  &   3686  &        0.668&  4.0&Y&Y&\nodata&\nodata\\
306  & 20 53 46.42  &$+$44 27 14.7  &   2908  &        0.471&  3.5&Y&\nodata&\nodata&\nodata\\
307  & 20 53 46.55  &$+$44 10 49.4  &   4010  &        1.135&  3.3&Y&Y&\nodata&\nodata\\
308  & 20 53 47.15  &$+$44 18 48.7  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
309  & 20 53 54.73  &$+$44 19 42.1  &   3490  &        0.279&  3.1&Y&Y&\nodata&\nodata\\
310  & 20 53 56.10  &$+$44 11 14.0  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
311  & 20 53 56.91  &$+$44 51 31.9  &   3279  &        0.403&  2.9&Y&Y&\nodata&\nodata\\
312  & 20 53 57.51  &$+$44 20 32.6  &   5330  &        4.166&  5.0&Y&Y&\nodata&\nodata\\
313  & 20 53 57.56  &$+$43 56 47.5  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
314  & 20 53 58.00  &$+$44 18 56.6  &   3160  &        0.250&  3.0&Y&\nodata&\nodata&\nodata\\
315  & 20 53 58.24  &$+$44 25 46.2  &   3990  &        0.381&  4.8&Y&\nodata&\nodata&\nodata\\
316  & 20 53 58.43  &$+$44 32 35.0  &   5800  &       20.684&  5.6&N&\nodata&\nodata&Y\\
317  & 20 53 58.56  &$+$44 25 36.4  &   3900  &        1.459&  5.4&Y&\nodata&\nodata&\nodata\\
318  & 20 54 02.41  &$+$44 08 17.4  &   3545  &        0.280&  4.3&Y&\nodata&\nodata&\nodata\\
319  & 20 54 03.85  &$+$44 01 47.8  &   3952  &        0.702&  3.0&Y&Y&\nodata&\nodata\\
320  & 20 54 05.30  &$+$44 36 29.3  &   3928  &        0.669&  5.5&Y&\nodata&\nodata&\nodata\\
321  & 20 54 06.45  &$+$44 22 25.4  &*******  &          NaN&  NaN&N&\nodata&\nodata&\nodata\\
322  & 20 54 06.71  &$+$44 28 13.1  &   3015  &        0.531&  4.8&Y&\nodata&\nodata&\nodata\\
323  & 20 54 08.76  &$+$44 30 11.5  &   5350  &        2.906&  4.6&Y&Y&\nodata&\nodata\\
324  & 20 54 09.95  &$+$44 10 00.3  &   3239  &        0.304&  4.5&Y&\nodata&\nodata&\nodata\\
325  & 20 54 10.12  &$+$44 31 03.0  &   4506  &        2.299&  5.6&Y&Y&\nodata&\nodata\\
326  & 20 54 10.72  &$+$44 32 44.8  &   3517  &        0.697&  5.5&Y&Y&\nodata&\nodata\\
327  & 20 54 11.22  &$+$44 57 09.8  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
328  & 20 54 11.62  &$+$44 29 56.0  &   3142  &        0.445&  5.2&Y&\nodata&\nodata&\nodata\\
329  & 20 54 13.72  &$+$44 24 32.2  &   4942  &        5.604&  5.5&Y&Y&\nodata&\nodata\\
330  & 20 54 16.07  &$+$44 24 10.5  &   5390  &        6.293&  4.7&Y&Y&\nodata&\nodata\\
331  & 20 54 17.72  &$+$44 48 40.1  &   5330  &       13.122&  3.8&Y&Y&\nodata&\nodata\\
332  & 20 54 20.93  &$+$44 31 57.6  &   3372  &        0.272&  5.4&N&\nodata&\nodata&\nodata\\
333  & 20 54 21.13  &$+$44 15 27.1  &   6250  &       29.752&  6.3&N&\nodata&\nodata&Y\\
334  & 20 54 21.77  &$+$44 20 51.1  &   3437  &        0.276&  4.3&Y&\nodata&\nodata&\nodata\\
335  & 20 54 22.52  &$+$44 37 17.2  &   3630  &        0.494&  3.8&Y&Y&\nodata&\nodata\\
336  & 20 54 22.84  &$+$44 24 24.9  &   3437  &        0.286&  3.2&Y&\nodata&\nodata&\nodata\\
337  & 20 54 24.03  &$+$44 34 28.9  &   6250  &       31.814&  7.1&N&\nodata&\nodata&\nodata\\
338  & 20 54 24.41  &$+$44 48 17.6  &   4010  &        0.984&  3.1&Y&Y&\nodata&\nodata\\
339  & 20 54 24.60  &$+$43 49 56.3  &*******  &          NaN&  NaN&N&\nodata&\nodata&\nodata\\
340  & 20 54 26.92  &$+$44 47 53.0  &   5330  &        6.547&  4.2&Y&Y&\nodata&\nodata\\
341  & 20 54 27.94  &$+$44 25 03.8  &   3105  &        0.105&  1.9&Y&Y&\nodata&\nodata\\
342  & 20 54 29.55  &$+$44 45 27.0  &   3713  &        0.950&  3.5&Y&Y&\nodata&\nodata\\
343  & 20 54 40.99  &$+$44 21 54.9  &   3781  &        0.481&  4.6&Y&Y&\nodata&\nodata\\
344  & 20 54 45.60  &$+$44 31 37.1  &   3951  &        1.007&  3.2&Y&Y&\nodata&\nodata\\
345  & 20 54 45.66  &$+$44 43 41.9  &   3713  &        0.503&  2.4&Y&Y&\nodata&\nodata\\
346  & 20 54 46.64  &$+$44 12 06.3  &   3904  &        2.405&  5.0&Y&Y&\nodata&Y\\
347  & 20 54 46.91  &$+$44 48 19.7  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
348  & 20 54 51.15  &$+$44 11 34.8  &   3943  &        1.249&  4.0&Y&Y&\nodata&Y\\
349  & 20 54 51.24  &$+$44 32 30.6  &   3961  &        0.228&  4.0&Y&\nodata&\nodata&\nodata\\
350  & 20 54 54.30  &$+$44 43 43.4  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
351  & 20 54 55.16  &$+$44 44 30.9  &   4216  &        2.109&  1.6&Y&Y&\nodata&\nodata\\
352  & 20 54 56.92  &$+$44 39 24.4  &   3437  &        0.296&  1.2&Y&Y&\nodata&\nodata\\
353  & 20 55 03.01  &$+$44 10 52.0  &   5350  &        6.329&  5.0&Y&Y&\nodata&\nodata\\
354  & 20 55 03.35  &$+$43 30 38.5  &*******  &          NaN&  NaN&N&\nodata&\nodata&\nodata\\
355  & 20 55 04.00  &$+$44 44 26.9  &   3279  &        0.193&  1.0&Y&Y&\nodata&\nodata\\
356  & 20 55 04.57  &$+$44 35 47.3  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
357  & 20 55 06.95  &$+$43 57 55.6  &*******  &          NaN&  NaN&N&\nodata&\nodata&\nodata\\
358  & 20 55 11.11  &$+$43 57 14.8  &Cont  &\nodata&\nodata&Y&Y&\nodata&Y\\
359  & 20 55 18.22  &$+$44 19 15.5  &*******  &          NaN&  NaN&N&\nodata&\nodata&\nodata\\
360  & 20 55 18.24  &$+$44 30 12.7  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
361  & 20 55 26.15  &$+$44 07 02.9  &*******  &          NaN&  NaN&N&\nodata&\nodata&\nodata\\
362  & 20 55 28.10  &$+$43 43 11.2  &   7250  &       15.356&  6.5&Y&\nodata&\nodata&\nodata\\
363  & 20 55 28.35  &$+$43 51 46.5  &*******  &          NaN&  NaN&N&\nodata&\nodata&\nodata\\
364  & 20 55 29.05  &$+$44 22 25.9  &   4888  &        1.073&  4.9&Y&\nodata&\nodata&\nodata\\
365  & 20 55 31.88  &$+$44 47 00.6  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
366  & 20 55 41.29  &$+$44 39 07.0  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
367  & 20 55 42.50  &$+$44 14 12.8  &   3946  &        0.460&  3.1&Y&Y&\nodata&\nodata\\
368  & 20 55 48.13  &$+$43 50 36.6  &*******  &          NaN&  NaN&N&\nodata&\nodata&\nodata\\
369  & 20 55 57.10  &$+$44 15 35.8  &   3979  &        0.697&  2.7&Y&Y&\nodata&\nodata\\
370  & 20 56 01.44  &$+$43 35 44.0  &  11500  &      120.674&  9.0&Y&\nodata&\nodata&\nodata\\
371  & 20 56 02.06  &$+$43 37 18.2  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
372  & 20 56 04.85  &$+$44 34 56.4  &   3199  &        0.377&  1.2&Y&Y&\nodata&\nodata\\
373  & 20 56 08.02  &$+$43 26 52.4  &*******  &          NaN&  NaN&N&\nodata&\nodata&\nodata\\
374  & 20 56 11.70  &$+$44 10 55.1  &   5019  &        2.507&  2.6&Y&Y&\nodata&\nodata\\
375  & 20 56 12.65  &$+$43 45 32.0  &   5800  &        6.530&  6.9&Y&Y&\nodata&Y\\
376  & 20 56 15.30  &$+$44 34 52.5  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
377  & 20 56 19.61  &$+$43 45 38.7  &   3970  &        0.646&  4.8&Y&\nodata&\nodata&Y\\
378  & 20 56 20.10  &$+$44 42 27.7  &   2956  &        0.115&  0.4&Y&\nodata&\nodata&\nodata\\
379  & 20 56 22.01  &$+$44 35 37.4  &   9250  &       46.929&  2.1&Y&\nodata&\nodata&\nodata\\
380  & 20 56 23.96  &$+$43 42 58.3  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
381  & 20 56 24.95  &$+$43 43 28.7  &   3240  &        0.838&  3.6&Y&Y&\nodata&\nodata\\
382  & 20 56 27.20  &$+$43 45 58.2  &   3891  &        1.130&  5.7&Y&\nodata&\nodata&Y\\
383  & 20 56 29.50  &$+$43 14 53.6  &Cont  &\nodata&\nodata&Y&Y&\nodata&\nodata\\
384  & 20 56 30.10  &$+$43 51 08.5  &   4253  &        0.908&  4.7&Y&\nodata&\nodata&\nodata\\
385  & 20 56 30.28  &$+$43 55 25.8  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
386  & 20 56 36.18  &$+$43 21 32.7  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
387  & 20 56 38.88  &$+$43 51 20.5  &   3713  &        0.352&  3.9&Y&\nodata&\nodata&\nodata\\
388  & 20 56 40.05  &$+$43 59 45.4  &   3835  &        0.078&  0.4&Y&\nodata&\nodata&\nodata\\
389  & 20 56 44.00  &$+$43 46 00.2  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
390  & 20 56 46.66  &$+$43 46 01.9  &   3034  &        0.712&  0.6&Y&Y&\nodata&\nodata\\
391  & 20 56 46.73  &$+$43 46 08.8  &Cont  &\nodata&\nodata&Y&Y&\nodata&\nodata\\
392  & 20 56 51.43  &$+$44 35 32.2  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
393  & 20 56 51.56  &$+$43 22 49.7  &   3437  &        0.650&  1.7&Y&Y&\nodata&\nodata\\
394  & 20 56 52.19  &$+$44 05 51.6  &   3814  &        0.572&  4.5&Y&Y&\nodata&\nodata\\
395  & 20 56 59.31  &$+$43 47 52.8  &   3124  &        0.189&  0.3&Y&Y&\nodata&\nodata\\
396  & 20 57 01.63  &$+$43 41 39.0  &Cont  &\nodata&\nodata&Y&Y&\nodata&\nodata\\
397  & 20 57 03.32  &$+$43 41 44.3  &   3713  &        0.480&  2.9&Y&Y&\nodata&\nodata\\
398  & 20 57 04.07  &$+$44 37 50.8  &   4253  &        0.665&  0.2&Y&Y&\nodata&\nodata\\
399  & 20 57 04.28  &$+$43 44 29.2  &   2908  &        0.276&  1.1&Y&\nodata&\nodata&\nodata\\
400  & 20 57 07.83  &$+$43 41 55.2  &   3825  &        1.582&  1.3&Y&Y&\nodata&\nodata\\
401  & 20 57 12.47  &$+$43 40 56.2  &   2770  &        0.088&  0.5&Y&\nodata&\nodata&\nodata\\
402  & 20 57 13.11  &$+$43 54 19.9  &   3124  &        0.271&  5.9&Y&\nodata&\nodata&\nodata\\
403  & 20 57 15.86  &$+$43 58 04.7  &   3052  &        0.141&  4.6&Y&\nodata&\nodata&\nodata\\
404  & 20 57 24.85  &$+$44 19 47.0  &   7500  &       31.747&  0.7&Y&\nodata&\nodata&\nodata\\
405  & 20 57 26.68  &$+$43 35 30.3  &   3955  &        1.003&  3.4&Y&Y&\nodata&\nodata\\
406  & 20 57 31.03  &$+$43 37 32.8  &   6250  &        5.709&  5.7&N&\nodata&\nodata&\nodata\\
407  & 20 57 33.77  &$+$44 05 13.4  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
408  & 20 57 34.52  &$+$43 59 54.7  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
409  & 20 57 37.29  &$+$44 06 44.0  &Cont  &\nodata&\nodata&Y&Y&\nodata&\nodata\\
410  & 20 57 38.38  &$+$44 06 58.9  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
411  & 20 57 41.80  &$+$43 49 53.3  &   2931  &        0.323&  1.5&Y&\nodata&\nodata&\nodata\\
412  & 20 57 46.54  &$+$44 07 11.7  &   2883  &        0.173&  1.8&Y&\nodata&\nodata&\nodata\\
413  & 20 57 48.50  &$+$43 29 42.7  &   3657  &        0.327&  0.6&N&Y&\nodata&\nodata\\
414  & 20 57 48.81  &$+$44 05 25.9  &*******  &          NaN&  NaN&N&Y&\nodata&Y\\
415  & 20 57 50.00  &$+$44 08 08.4  &   3490  &        0.420&  0.8&Y&Y&\nodata&\nodata\\
416  & 20 57 55.42  &$+$44 05 25.0  &   2883  &        0.456&  1.6&Y&\nodata&\nodata&\nodata\\
417  & 20 57 59.85  &$+$43 53 26.6  &   3946  &        1.843&  1.9&Y&Y&\nodata&Y\\
418  & 20 58 01.36  &$+$43 45 20.6  &   3964  &        0.933&  3.4&Y&Y&\nodata&\nodata\\
419  & 20 58 06.04  &$+$43 49 32.8  &   3630  &        0.318&  0.7&Y&Y&\nodata&Y\\
420  & 20 58 06.10  &$+$43 53 01.4  &   3546  &        0.499&  0.8&Y&Y&\nodata&\nodata\\
421  & 20 58 07.64  &$+$43 52 52.7  &Cont  &\nodata&\nodata&Y&Y&\nodata&\nodata\\
422  & 20 58 08.43  &$+$43 39 00.3  &   2956  &        0.032&  0.4&Y&\nodata&\nodata&\nodata\\
423  & 20 58 08.86  &$+$43 46 59.9  &   3858  &        0.810&  2.7&Y&Y&\nodata&\nodata\\
424  & 20 58 09.53  &$+$44 11 02.8  &   3087  &        0.661&  2.7&Y&\nodata&\nodata&\nodata\\
425  & 20 58 09.99  &$+$43 45 36.1  &   3179  &        0.258&  1.7&Y&Y&\nodata&Y\\
426  & 20 58 10.82  &$+$43 53 08.2  &   3858  &        1.993&  1.9&Y&Y&\nodata&Y\\
427  & 20 58 11.38  &$+$43 52 57.0  &   3052  &        0.840&  4.8&Y&\nodata&\nodata&\nodata\\
428  & 20 58 12.33  &$+$44 20 58.2  &   3657  &        0.549&  2.8&Y&Y&\nodata&\nodata\\
429  & 20 58 14.27  &$+$43 53 04.6  &   2883  &        0.298&  1.6&Y&\nodata&\nodata&Y\\
430  & 20 58 17.90  &$+$43 53 44.1  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&Y\\
431  & 20 58 18.19  &$+$43 26 13.5  &   4043  &        0.535&  1.8&Y&Y&\nodata&\nodata\\
432  & 20 58 19.61  &$+$43 53 54.5  &   5390  &        4.167&  4.4&Y&Y&\nodata&\nodata\\
433  & 20 58 21.54  &$+$43 53 44.9  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&Y\\
434  & 20 58 23.71  &$+$43 52 56.3  &Cont  &\nodata&\nodata&Y&Y&\nodata&\nodata\\
435  & 20 58 23.81  &$+$43 53 11.4  &   5600  &       18.783&  3.2&Y&Y&\nodata&Y\\
436  & 20 58 23.99  &$+$43 53 54.6  &   3858  &        2.161&  2.2&Y&Y&\nodata&\nodata\\
437  & 20 58 25.55  &$+$43 53 28.6  &   3360  &        0.624&  3.2&Y&Y&\nodata&Y\\
438  & 20 58 26.90  &$+$44 18 06.3  &   2931  &        0.120&  1.6&Y&\nodata&\nodata&\nodata\\
439  & 20 58 27.02  &$+$43 53 20.1  &Cont  &\nodata&\nodata&Y&Y&\nodata&Y\\
440  & 20 58 27.25  &$+$43 54 55.8  &   2883  &        0.039&  0.0&Y&\nodata&\nodata&\nodata\\
441  & 20 58 29.09  &$+$44 10 50.5  &Cont  &\nodata&\nodata&Y&Y&\nodata&\nodata\\
442  & 20 58 29.41  &$+$43 55 12.5  &   2908  &        0.480&  7.3&Y&\nodata&\nodata&\nodata\\
443  & 20 58 30.41  &$+$43 53 59.2  &Cont  &\nodata&\nodata&Y&Y&\nodata&Y\\
444  & 20 58 30.47  &$+$43 54 09.6  &   3412  &        0.420&  1.2&Y&Y&\nodata&\nodata\\
445  & 20 58 30.94  &$+$43 45 11.2  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
446  & 20 58 33.59  &$+$44 03 35.5  &   3437  &        0.279&  0.0&Y&Y&\nodata&Y\\
447  & 20 58 35.67  &$+$44 18 44.8  &   3279  &        0.077&  1.8&Y&\nodata&\nodata&\nodata\\
448  & 20 58 39.58  &$+$44 18 28.0  &   3240  &        0.345&  3.0&Y&Y&\nodata&\nodata\\
449  & 20 58 39.65  &$+$43 43 09.1  &*******  &          NaN&  NaN&N&Y&\nodata&Y\\
450  & 20 58 39.74  &$+$44 01 32.8  &   4216  &        0.318&  3.1&Y&Y&\nodata&Y\\
451  & 20 58 41.97  &$+$44 16 25.6  &   3160  &        0.119&  1.7&Y&\nodata&\nodata&\nodata\\
452  & 20 58 43.13  &$+$43 46 00.1  &   2842  &        0.136&  2.6&Y&\nodata&\nodata&\nodata\\
453  & 20 58 47.40  &$+$44 01 34.8  &   2980  &        0.167&  0.7&Y&\nodata&\nodata&\nodata\\
454  & 20 58 53.22  &$+$43 58 32.9  &   3015  &        0.155&  0.4&Y&Y&\nodata&\nodata\\
455  & 20 59 03.47  &$+$44 13 11.6  &   3015  &        0.062&  1.0&Y&\nodata&\nodata&\nodata\\
456  & 20 59 05.82  &$+$43 57 03.2  &   5300  &       20.381&  3.0&Y&Y&\nodata&\nodata\\
457  & 20 59 06.70  &$+$44 18 23.7  &   3814  &        0.243&  1.4&Y&Y&\nodata&Y\\
458  & 20 59 14.86  &$+$44 12 28.5  &Cont  &\nodata&\nodata&Y&Y&\nodata&\nodata\\
459  & 20 59 20.20  &$+$44 17 05.1  &   3546  &        0.063&  3.4&Y&\nodata&\nodata&\nodata\\
460  & 20 59 29.57  &$+$44 10 47.7  &   3686  &        0.208&  2.4&Y&Y&\nodata&\nodata\\
461  & 20 59 29.74  &$+$44 17 04.2  &   3770  &        0.314&  2.9&Y&Y&\nodata&\nodata\\
462  & 20 59 32.69  &$+$44 08 35.5  &   3490  &        0.419&  2.6&Y&Y&\nodata&\nodata\\
463  & 20 59 38.29  &$+$44 10 07.2  &   3124  &        0.368&  2.5&Y&Y&\nodata&\nodata\\
464  & 20 50 53.80  &$+$44 21 18.5  &   3320  &        1.741&  3.0&Y&Y&\nodata&\nodata\\
465  & 20 53 00.65  &$+$44 36 59.5  &   5800  &       27.820&  5.5&N&Y&\nodata&Y\\
466  & 20 53 17.47  &$+$44 28 03.1  &   3916  &        1.529&  3.7&Y&Y&\nodata&Y\\
467  & 20 53 37.85  &$+$44 24 20.9  &   3946  &        0.950&  3.3&Y&Y&\nodata&Y\\
468  & 20 55 43.25  &$+$44 03 12.5  &   3835  &        0.752&  0.0&Y&Y&\nodata&Y\\
469  & 20 54 27.90  &$+$44 00 09.8  &   3240  &        0.328&  7.1&Y&\nodata&\nodata&\nodata\\
470  & 20 52 46.12  &$+$44 10 42.5  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
471  & 20 52 39.86  &$+$44 05 48.2  &   3279  &        0.173&  1.7&Y&Y&\nodata&\nodata\\
472  & 20 51 05.45  &$+$44 13 59.3  &   3015  &        0.669&  1.6&Y&Y&\nodata&Y\\
473  & 20 52 56.68  &$+$44 29 48.4  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
474  & 20 51 47.93  &$+$44 38 40.8  &   3199  &        0.121&  6.1&N&\nodata&\nodata&\nodata\\
475  & 20 52 46.08  &$+$44 39 09.9  &   3412  &        0.230&  8.0&Y&\nodata&\nodata&\nodata\\
476  & 20 53 08.17  &$+$44 05 14.3  &   3220  &        0.320&  2.6&Y&Y&\nodata&\nodata\\
477  & 20 52 14.74  &$+$43 59 47.3  &   2842  &        0.159&  1.7&Y&\nodata&\nodata&\nodata\\
478  & 20 52 51.38  &$+$44 20 35.7  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
479  & 20 52 41.58  &$+$44 19 27.2  &   3124  &        0.075&  2.9&N&\nodata&\nodata&\nodata\\
480  & 20 59 19.65  &$+$43 46 00.4  &   2770  &        0.029&  1.5&Y&\nodata&\nodata&\nodata\\
481  & 20 56 39.90  &$+$43 59 45.4  &Cont  &\nodata&\nodata&Y&\nodata&\nodata&\nodata\\
482  & 20 58 19.48  &$+$43 53 44.9  &   3517  &        1.407&  3.2&Y&Y&\nodata&\nodata\\
483  & 20 53 34.63  &$+$44 28 51.3  &   3490  &        0.400&  3.5&Y&Y&\nodata&\nodata\\
484  & 20 53 58.29  &$+$44 10 21.1  &   4292  &        0.868&  3.6&N&Y&\nodata&\nodata\\
485  & 20 53 35.58  &$+$44 17 43.2  &   3490  &        0.439&  2.9&N&Y&\nodata&\nodata\\
486  & 20 53 55.56  &$+$44 11 06.0  &   3858  &        0.842&  3.9&N&Y&\nodata&Y\\
487  & 20 54 05.00  &$+$44 10 24.6  &   3958  &        1.406&  4.2&N&Y&\nodata&\nodata\\
488  & 20 54 06.29  &$+$44 30 24.7  &   4000  &        2.676&  3.9&N&Y&\nodata&Y\\
489  & 20 53 54.54  &$+$44 32 28.5  &   6500  &       16.329&  5.4&N&\nodata&\nodata&\nodata\\
490  & 20 53 33.32  &$+$44 25 18.6  &   3928  &        0.880&  3.6&N&Y&\nodata&Y\\
491  & 20 53 45.79  &$+$44 28 16.7  &   3320  &        0.546&  3.4&N&\nodata&\nodata&Y\\
492  & 20 53 46.44  &$+$44 27 04.6  &   3630  &        0.770&  3.6&N&\nodata&\nodata&Y\\
493  & 20 53 40.08  &$+$44 25 50.1  &   5310  &       11.526&  5.0&N&Y&\nodata&\nodata\\
494  & 20 53 41.37  &$+$44 24 36.2  &   3517  &        0.740&  3.3&N&Y&\nodata&\nodata\\
495  & 20 54 31.96  &$+$44 20 15.7  &   8500  &       51.565&  9.3&N&\nodata&\nodata&\nodata\\
496  & 20 54 49.16  &$+$44 20 14.6  &   3979  &        2.539&  6.1&N&Y&\nodata&\nodata\\
497  & 20 53 43.61  &$+$44 15 08.6  &   3791  &        0.855&  4.2&N&Y&\nodata&\nodata\\
498  & 20 55 01.18  &$+$44 06 45.8  &   8000  &       47.652&  8.4&N&\nodata&\nodata&\nodata\\
499  & 20 53 58.87  &$+$44 09 41.5  &   3657  &        0.519&  4.0&N&Y&\nodata&\nodata\\
500  & 20 52 26.30  &$+$44 03 26.5  &   3490  &        0.238&  2.3&N&Y&\nodata&\nodata\\
501  & 20 50 48.60  &$+$44 17 03.4  &   3199  &        0.346&  2.6&Y&\nodata&\nodata&Y\\
502  & 20 50 57.49  &$+$44 24 45.4  &   3904  &        1.229&  4.2&Y&\nodata&\nodata&\nodata\\
503  & 20 50 37.38  &$+$44 20 53.0  &   3517  &        2.280&  1.4&N&Y&\nodata&\nodata\\
504  & 20 51 06.63  &$+$44 21 40.7  &*******  &          NaN&  NaN&N&Y&\nodata&\nodata\\
505  & 20 52 08.95  &$+$44 21 54.6  &   3686  &        0.488&  4.0&Y&Y&\nodata&\nodata\\
506  & 20 52 33.58  &$+$44 20 45.9  &   2931  &        0.208&  2.3&Y&\nodata&\nodata&\nodata\\
507  & 20 52 06.72  &$+$44 29 23.6  &   3791  &        0.539&  2.1&N&Y&\nodata&\nodata\\
508  & 20 52 32.66  &$+$44 26 32.2  &   4020  &        1.393&  3.7&N&Y&\nodata&Y\\
509  & 20 52 26.79  &$+$44 37 06.6  &   5700  &       19.144&  7.0&N&Y&\nodata&Y\\
510  & 20 52 33.95  &$+$44 29 16.8  &   4000  &        0.997&  3.3&N&Y&\nodata&Y\\
511  & 20 52 29.41  &$+$44 38 40.4  &   3916  &        1.528&  4.9&N&Y&\nodata&Y\\
512  & 20 52 45.03  &$+$44 35 23.7  &   4253  &        0.808&  4.2&N&Y&\nodata&Y\\
513  & 20 53 29.92  &$+$44 39 35.1  &   3412  &        0.486&  3.2&N&Y&\nodata&Y\\
514  & 20 53 12.22  &$+$44 26 34.9  &   3517  &        1.047&  4.3&N&Y&\nodata&Y\\
515  & 20 53 40.53  &$+$44 37 27.3  &   6000  &       22.606&  8.9&N&\nodata&\nodata&Y\\
516  & 20 50 55.44  &$+$44 17 45.9  &   3490  &        0.322&  1.5&N&Y&\nodata&\nodata\\
517  & 20 52 05.51  &$+$44 23 37.0  &*******  &          NaN&  NaN&N&\nodata&\nodata&Y\\
518  & 20 50 59.66  &$+$44 30 15.3  &   3916  &        0.365&  3.5&N&\nodata&\nodata&Y\\
519  & 20 52 24.97  &$+$44 28 15.4  &   3412  &        0.448&  2.9&N&Y&\nodata&Y\\
520  & 20 53 02.09  &$+$44 46 14.3  &   3464  &        0.254&  2.5&Y&Y&\nodata&\nodata\\
521  & 20 51 47.79  &$+$43 42 38.9  &   3990  &        0.887&  1.2&N&Y&\nodata&\nodata\\
522  & 20 50 54.47  &$+$43 46 23.8  &   3928  &        0.335&  0.8&Y&Y&\nodata&\nodata\\
523  & 20 48 57.79  &$+$43 49 55.1  &   3015  &        0.573&  5.4&Y&\nodata&\nodata&\nodata\\
524  & 20 48 51.69  &$+$43 51 01.4  &   3880  &        0.483&  2.7&Y&\nodata&\nodata&\nodata\\
525  & 20 48 35.46  &$+$43 53 13.4  &   3814  &        0.567&  2.0&Y&Y&\nodata&\nodata\\
526  & 20 48 32.87  &$+$44 11 59.6  &   3240  &        0.297&  1.9&Y&Y&\nodata&\nodata\\
527  & 20 48 33.96  &$+$44 22 28.7  &   5330  &       12.403&  2.9&Y&Y&\nodata&\nodata\\
528  & 20 50 06.17  &$+$44 25 05.0  &   3052  &        0.511&  1.6&N&Y&\nodata&Y\\
529  & 20 50 44.96  &$+$44 20 58.9  &   3240  &        0.108&  1.7&Y&Y&\nodata&\nodata\\
530  & 20 50 37.95  &$+$44 25 12.4  &   3880  &        4.486&  6.6&Y&Y&\nodata&Y\\
531  & 20 50 56.70  &$+$44 17 05.4  &   3385  &        0.242&  1.6&N&Y&\nodata&\nodata\\
532  & 20 50 54.86  &$+$44 20 12.5  &   3160  &        0.209&  2.2&Y&Y&\nodata&\nodata\\
533  & 20 50 48.53  &$+$44 33 33.2  &   3437  &        0.400&  4.3&Y&Y&\nodata&\nodata\\
534  & 20 51 12.44  &$+$44 19 43.0  &   3015  &        0.417&  1.9&N&Y&\nodata&\nodata\\
535  & 20 51 20.59  &$+$44 20 32.2  &   3320  &        0.692&  1.2&N&Y&\nodata&\nodata\\
536  & 20 51 12.62  &$+$44 18 45.4  &   5300  &       12.396&  2.1&N&Y&\nodata&\nodata\\
537  & 20 52 34.38  &$+$44 26 05.2  &   3686  &        0.444&  3.8&N&\nodata&\nodata&\nodata\\
538  & 20 52 51.93  &$+$44 28 13.7  &   3928  &        0.812&  4.1&N&Y&\nodata&Y\\
539  & 20 52 22.91  &$+$44 22 25.3  &   3657  &        0.708&  3.4&N&Y&\nodata&Y\\
540  & 20 53 27.53  &$+$44 06 09.3  &   6250  &        7.406&  2.6&N&Y&\nodata&\nodata\\
541  & 20 51 13.74  &$+$44 22 25.2  &   2931  &        0.325&  1.1&N&Y&\nodata&Y\\
542  & 20 51 05.91  &$+$44 23 47.1  &   3240  &        0.170&  1.4&Y&\nodata&\nodata&\nodata\\
543  & 20 52 31.70  &$+$44 29 59.1  &   3412  &        0.477&  2.9&N&\nodata&\nodata&Y\\
544  & 20 54 34.54  &$+$44 33 08.8  &   3880  &        1.325&  3.3&N&Y&\nodata&Y\\
545  & 20 55 49.40  &$+$44 34 10.2  &   5100  &        2.500&  6.0&N&\nodata&\nodata&\nodata\\
546  & 20 55 28.51  &$+$44 43 45.0  &   3517  &        0.412&  0.8&N&Y&\nodata&\nodata\\
547  & 20 55 19.40  &$+$44 41 09.6  &   3360  &        0.175&  1.8&N&Y&\nodata&\nodata\\
548  & 20 54 57.36  &$+$44 38 43.6  &   3990  &        0.866&  1.2&N&Y&\nodata&\nodata\\
549  & 20 54 44.66  &$+$44 31 44.2  &   5700  &       15.080&  3.6&N&Y&\nodata&Y\\
550  & 20 54 45.82  &$+$44 35 48.0  &   3437  &        0.786&  2.9&N&Y&\nodata&\nodata\\
551  & 20 54 06.49  &$+$44 30 24.0  &   3958  &        2.219&  3.9&N&Y&\nodata&\nodata\\
552  & 20 53 57.79  &$+$44 29 43.0  &   5300  &        7.572&  5.2&N&Y&\nodata&\nodata\\
553  & 20 53 25.47  &$+$44 27 16.4  &   3713  &        2.368&  4.2&N&Y&\nodata&Y\\
554  & 20 53 08.30  &$+$44 50 05.0  &   3517  &        0.311&  1.8&N&Y&\nodata&\nodata\\
555  & 20 53 23.81  &$+$45 06 47.8  &   4292  &        0.606&  2.9&Y&\nodata&\nodata&\nodata\\
556  & 20 59 25.87  &$+$44 14 21.6  &   3630  &        0.310&  2.4&Y&Y&\nodata&Y\\
557  & 20 59 57.74  &$+$44 47 12.6  &   4506  &        0.718&  0.6&N&Y&\nodata&\nodata\\
558  & 20 53 42.14  &$+$44 26 53.7  &   3835  &        1.440&  3.9&N&Y&\nodata&Y\\
559  & 21 00 03.30  &$+$43 04 27.9  &   3630  &        0.104&  2.0&N&\nodata&\nodata&\nodata\\
560  & 21 01 17.98  &$+$43 40 06.2  &*******  &          NaN&  NaN&N&\nodata&\nodata&\nodata\\
561  & 21 01 04.96  &$+$43 19 43.7  &*******  &          NaN&  NaN&N&\nodata&\nodata&\nodata\\
\enddata
\end{deluxetable*}

